A New Deterministic Algorithm for Fully Dynamic All-Pairs Shortest Paths

We study the fully dynamic All-Pairs Shortest Paths (APSP) problem in undirected edge-weighted graphs. Given an $n$-vertex graph $G$ with non-negative edge lengths, that undergoes an online sequence of edge insertions and deletions, the goal is to support approximate distance queries and shortest-path queries. We provide a deterministic algorithm for this problem, that, for a given precision parameter $\epsilon$, achieves approximation factor $(\log\log n)^{2^{O(1/\epsilon^3)}}$, and has amortized update time $O(n^{\epsilon}\log L)$ per operation, where $L$ is the ratio of longest to shortest edge length. Query time for distance-query is $O(2^{O(1/\epsilon)}\cdot \log n\cdot \log\log L)$, and query time for shortest-path query is $O(|E(P)|+2^{O(1/\epsilon)}\cdot \log n\cdot \log\log L)$, where $P$ is the path that the algorithm returns. To the best of our knowledge, even allowing any $o(n)$-approximation factor, no adaptive-update algorithms with better than $\Theta(m)$ amortized update time and better than $\Theta(n)$ query time were known prior to this work. We also note that our guarantees are stronger than the best current guarantees for APSP in decremental graphs in the adaptive-adversary setting.

==> arxiv-version-final/APSP-full-alg.tex <==
\newpage

\section{Algorithm for Fully Dynamic \APSP -- Proof of \Cref{thm: main fully-dynamic APSP single scale}}
\label{sec: fully dynamic alg}

The purpose of this section is to prove Theorem \ref{thm: main fully-dynamic APSP single scale}.

We can assume without loss of generality that the length of every edge in $G$ is at most $D^*$, as edges whose length is greater than $D^*$ can be deleted from $G$.




==> arxiv-version-final/ES-tree.tex <==
\subsection{First Tool: Modified Even-Shiloach Trees}
\label{subsec: ES-trees}

Even-Shiloach Tree (see, e.g. \cite{EvenS,Dinitz,HenzingerKing}) is a classical data structure, that, given a graph $G=(V,E)$ with integral lengths $\ell(e)\geq 1$ on its edges $e\in E$ that undergoes edge deletions, a source $s$, and a distance bound $D\geq 1$, maintains a shortest-path tree from vertex $s$, that includes all vertices $v$ with $\dist(s,v)\leq D$, and, for every vertex $v$ with $\dist(s,v)\leq D$, the distance $\dist(s,v)$. The data structure also supports shortest-path queries: given a vertex $v\in V$, either correctly report that $\dist(s,v)>D$, or return a shortest path connecting $s$ to $v$. We need to slightly generalize this data structure, so that it also supports super-node splitting operations. We do so in the following theorem, whose proof is standard and is deferred to the Appendix.

%Typically, \EST only supports edge deletions (see, e.g. \cite{EvenS,Dinitz,HenzingerKing}). However, as shown in \cite[Lemma 2.4]{BernsteinChechik}, it is easy to extend the data structure to also handle edge insertions in the following two cases: either (i) at least one of the endpoints of the inserted edge is a singleton vertex, or (ii) the distances from the source $s$ to other vertices do not decrease due to the insertion. We denote the corresponding data structure from \cite{BernsteinChechik} by $\EST(G,s,D)$. It was shown in \cite{BernsteinChechik}  that the total update time of $\EST(G,s,D)$, including the initialization and all edge deletions, is $O(m D + U)$, where $U$ is the total number of updates (edge insertions or deletions), and $m$ is the total number of edges that ever appear in $G$.



\begin{theorem}\label{thm: ES-tree}
	There is a deterministic algorithm, that, given a valid input \newline $\iset=\left(H,T,\set{\ell(e)}_{e\in E(H)}, \set{w(v)}_{v\in V(H)}\right )$ to the \recdynnc problem, where graph $H$ undergoes edge-deletion, isolated vertex-deletion, and node-splitting updates, such that vertex weights obey Rules \ref{rule 1: reg vertex weight 0}---\ref{rule 3: weights of split supernodes}, and given additionally a source vertex $s\in V$ (that is a regular vertex), and a distance threshold $D^*>0$, supports $\shortestpath$ queries: given a vertex $v\in V(H)$, either correctly establish, in time $O(\log n)$, that $\dist_H(s,v)>D^*$, or return a shortest $s$-$v$ path $P$, in time $O(|E(P)|)$. The total update time of the algorithm is $\otilde(W\cdot D^*\log W)$, where $W$ is the total weight of all vertices of $H$ at the beginning of the algorithm.
\end{theorem}

\mynote{need to fix the proof so we use $W$ instead of $W(H)$.}
\mynote{Define $W(H)$ and claim it can only decrease? Also that total weight of deleted vertices plus total weight of current vertices only decreases, in observation.}



==> arxiv-version-final/T-emulator.tex <==
\subsection{Maintaining a $T$-Emulator: Proof of \Cref{cor: T-emulator}}
\label{subsec: T-emulator}

In this subsection we prove  \Cref{cor: T-emulator}. 
We assume that\ \Cref{assumption: alg for recdynnc} holds. We also assume that we are given a graph $G$, with integral lengths $\ell(e)\geq 1$ on its edges, that udergoes a sequence $\Sigma$ of edge-deletion and edge-insertion operations, together with a precision parameter $\frac{1}{(\log W)^{1/4}}<\eps<1$, and a distance parameter $0<D^*<W$ that is an integral power of $2$. Denote
$|\Sigma|+|V(G)|+|E(G\attime[0])|=m$, and recall that $m^{1+2\eps}<W/8$.
Additionally, we are given a set $T\subseteq V(G)$ of vertices that we call terminals. We denote by $\tset$ the time horizon that is associated with the update sequence $\Sigma$.

We apply the algorithm from \Cref{thm: main fully-dynamic APSP single scale} to this input, and we denote by $\DS$ the data structure that the algorithm maintains. Recall that the total update time of the algorithm is bounded by $O\left (W^{1+O(\delta)+O(\eps)}\cdot (\Delta(W)\cdot\log W)^{O(1/\eps^2)}\right )$. We will exploit data structure $\DS$, in order to define graph $H$, and we will use the parameters that were defined in the proof of \Cref{thm: main fully-dynamic APSP single scale}. We denote by $\cset=\bigcup_{L=0}^q\cset^L$ the collection of clusters that data structure $\DS$ maintains.

We start by defining the graph $H$, and then provide an algorithm for maintianing it. We then prove that the resulting graph $H$ has all required properties, and provide an algorithm for supporting $\transformpath$ queries.



\input{emulator-def}
\input{emulator-maintain}
\input{stretch-transform-path}


==> arxiv-version-final/appx-reduction.tex <==
\section{Proofs Omitted from \Cref{sec: fully APSP inner main}}
\subsection{Proof of \Cref{obs: coverning chain importance}}
\label{subsec: covering chain importance}
Throughout the proof, whenever we refer to any dynamic objects or data structures, we refer to them at time $\tau$, unless stated otherwise.
Fix an index $1\leq r'<r$. For convenience, we denote $L_{r'}=L$, $C_{r'}=C$, and $i_{r'}=i$. We also denote  $L_{r'+1}=L'$, $C_{r'+1}=C'$, $i_{r'+1}=i'$, and $x_{r'+1}=x'$. Note that, from the definition of a covering chain, supernode $u^{L'}(C)$ must lie in graph $H^{L'}$, so it only remains to prove that $u^{L'}(C)$ is an important supernode for cluster $C'$. From the definition of a covering chain, we are also guaranteed that $i'\geq i+10$, and that $C'=\coveringcluster^{L'}_{i'}(v^{L'}(x'))$. We denote by $\Phi^{L'}_k$ the level-$L'$ phase to which time $\tau$ belongs.

From the definition of a covering chain, $x'\in V^F(C)$ holds, and so edge $(v^{L'}(x'),u^{L'}(C))$ belongs to graph $H^{L'}$. The length of this edge, and the length of every edge incident to supernode $u^{L'}(C)$ in $H^{L'}$ is $2^{\scale(C)}=2^i$. Since $C'=\coveringcluster^{L'}_{i'}(v^{L'}(x'))$, cluster $C'$ contains every vertex in graph $H^{L'}$, whose distance from $v^{L'}(x')$ is at most $2^{i'}$, where $i'\geq {i+10}$. Therefore, both $u^{L'}(C)$, and every vertex that is connected by an edge to $u^{L'}(C)$, lie in cluster $C'$ at time $\tau$. Notice also that $N(u^{L'}(C))\neq \emptyset$ holds at time $\tau$, since $v^{L'}(x')\in N(u^{L'}(C))$. For convenience, denote $u^{L'}(C)$ by $u$.

From Rule \ref{rule2 for importance}, it is now enough to show that, for every time $\tau'<\tau$ during Phase $\Phi^{L'}_k$, if we denote $\tilde C=\anc\attime[\tau'](C')$ and $\tilde u=\anc\attime[\tau'](u)$, then, at time $\tau'$, $N(\tilde u)\subseteq V(\tilde C)$ held.

We now consider any time $\tau'<\tau$ during Phase $\Phi^{L'}_k$, and we denote $\tilde C=\anc\attime[\tau'](C')$ and $\tilde u=\anc\attime[\tau'](u)$. It is now enough to prove that, at time  $\tau'$, $N(\tilde u)\neq \emptyset$ and $N(\tilde u)\subseteq V(\tilde C)$ held.

Observe first that, from the Consistent Covering Property, that is required from the data structures for the \recdynnc problem, at time $\tau'$, $\tilde C=\coveringcluster^{L'}_{i'}(v^{L'}(x'))$ must hold. Therefore, at time $\tau'$, cluster $\tilde C$ contains every vertex of $H^{L'}$ that lies at distance at most $2^{i'}$, where $i'\geq {i+10}$, from vertex $v^{L'}(x)$. We show that this must include every vertex of $N\attime[\tau'](\tilde u)$. Indeed, from \Cref{obs: supernode edge tracking}, since edge $(v^{L'}(x),u)$ is present in graph $H^{L'}$ at time $\tau$, and its length is $2^i$, edge $(v^{L'}(x),\tilde u)$ must be present in graph $H^{L'}$ at time $\tau'$, and its length must also be $2^i$. Since all edges incident to a type-2 supernode have the same length, every edge incident to $\tilde u$ has length $2^i$. Therefore, all vertices of $N\attime[\tau'](\tilde u)$ lie within distance at most $2\cdot 2^i$ from $v^{L'}(x)$ in graph $H^{L'}$ at time $\tau'$, and each such vertex must belong to $C'$. Since vertex $v^{L'}(x')$ belongs to $N(\tilde u)$ at time $\tau'$, we conclude that $N(\tilde u)\neq \emptyset$.


\subsection{Proof of \Cref{obs: another important supernode}}
\label{subsec: obs: another important supernode}


Recall that, at time $\tau$, supernode $u^L(C')$ belongs to $H^L$, and, from the definition of covering chains, $C=\coveringcluster^L_{i'}(v^L(x'))$, and $y'\in V^F(C')$. Moreover,  there is a path $P'$ in graph $H^L$, connecting $v^L(x')$ to  $v^L(y')$, whose length is at most $2^{10L+4}\cdot D_i$.

Therefore, at time $\tau$, cluster $C$ contains all vertices of $H^L$, whose distance from $v^L(x')$ is at most $2^{i'}=2^{i+10L+10}$. At the same time, the distance from $v^L(x')$ to $v^L(y')$ is at most $2^{i+10L+4}$, and every edge that is incident to supernode $u^L(C')$ (inclung the edge that connects it to $v^L(y')$), has length $2^{i''}\leq 2^{i+10L}$. Therefore, at time $\tau$, every vertex in $N(u^L(C'))$ lies at distance at most $2^{i+10L+4}+2\cdot 2^{i+10L}<2^{i+10L+10}$ from vertex $v^L(x')$. We conclude that, at time $\tau$, $u^L(C')\in V(C)$, $N(u^L(C'))\neq \emptyset$, and $N(u^L(C'))\subseteq V(C)$ holds. 
For convenience, we denote $u=u^L(C')$ from now on, and we denote by $\Phi^L_k$ the level-$L$ phase that contains time $\tau$.
Since $\scale(C')=i''<i'=\scale(C)$, from Rule \ref{rule2 for importance}, it is now enough to prove that, for every time $\tau'<\tau$ during Phase $\Phi^L_k$, if we denote $\tilde C=\anc\attime[\tau'](C)$ and $\tilde u=\anc\attime[\tau'](u)$, then, at time $\tau'$, $N(\tilde u)\neq \emptyset$ and $N(\tilde u)\subseteq V(\tilde C)$ held.

From now on, we fix a time $\tau'<\tau$ during Phase $\Phi^L_k$, and we denote $\tilde C=\anc\attime[\tau'](C)$ and $\tilde u=\anc\attime[\tau'](u)$. From the Consistent Covering Poperty of the data structure for the \recdynnc problem, at time $\tau'$, $\tilde C=
\coveringcluster^L_{i'}(v^L(x'))$ held. Therefore, at time $\tau'$, cluster $\tilde C$ contained every vertex of $H^{L}$, whose distance from $v^L(x')$ is at most $2^{i'}=2^{i+10L+10}$. At the same time, from \Cref{obs: no dist increase}, distances between vertices of $H^L$ may only grow over the course of Phase $\Phi^L_k$, so at time $\tau'$, $\dist_{H^L}(v^L(x'),v^L(y'))\leq 2^{i+10L+4}$. Furthermore, since edge $(u,v^L(y'))$ of length $2^{i''}$ lies in graph $H^L$ at time $\tau$, from \Cref{obs: supernode edge tracking}, edge $(\tilde u,v^L(y'))$ of length $2^{i''}$ lies in $H^L$ at time $\tau'$. Thereore, at time $\tau'$, $N(\tilde u)\neq \emptyset$. Lastly, all edges incident to $\tilde u$ must have the same length $2^{i''}\leq 2^{i+10L}$. We conclude that for every vertex $v^L(a)$, that lies in set $N(\tilde u)$ at time $\tau'$, the distance from $v^L(a)$ to $v^L(x')$ at time $\tau'$ is at most $2^{i+10L+4}+2\cdot 2^{i+10L}<2^{i+10L+10}$, and so $N(\tilde u)\subseteq V(\tilde C)$ holds at time $\tau'$.

==> arxiv-version-final/document.tex <==
\subsection{Stage 1: Large Pseudocut Regime}


\begin{lemma}[Simplified version of Lemma 3.12 from \cite{DMG}]\label{lem: path peel}
	There is a deterministic algorithm, called \procpathpeel, that, given a graph $G$, two collections $A,B$ of disjoint subsets of its vertices, and parameters $d,\eta>0$, outputs a routing $\pset$ of vertices of $A$ to vertices of $B$, so that every path in $\pset$ is a simple path of length at most $d$, and the paths in $\pset$ cause congestion at most $\eta$. Moreover, if we denote by $E'$ be the set of all edges $e\in E(G)$, such that exactly $\eta$ paths of $\pset$ use $e$, and we let $A'\subseteq A$, $B'\subseteq B$ be the sets of vertices that do not serve as endpoints of the paths in $\pset$, then $\dist_{G\setminus E'}(A',B')> d$.
 The running time of the algorithm is $O(m\eta+md\log n)$, where $m=|E(G)|$ and $n=V(G)$.
\end{lemma}


==> arxiv-version-final/emulator-def.tex <==
\subsubsection{Definition of Graph $H$}
\label{subsubsec: emulator definition}

We start by defining a dynamic graph $\tilde H$. The dynamic graph $H$ will be obtained from $\tilde H$ by adding a number of isolated vertices to it.
Let $\tau$ be any time during the time horizon $\tset$. We now define the graph $\tH\attime$. Whenever we refer to any dynamic objects and data structures in this definition, we refer to them at time $\tau$. The set $V(\tH)$ of vertices of graph $\tH$ is partitioned into subsets $T,A_0,A_1,\ldots,A_{q}$, that we refer to as \emph{layers}. For $0\leq L\leq q$, set $A_L$ of vertices will contain, for some clusters $C\in \cset^{L}$, a corresponding vertex $z(C)$. We now define the layers $A_0,\ldots,A_q$ one by one. Whenever vertices in each layer are defined, we also define the edges that are incident to them.

\paragraph{Set $A_0$.} For every cluster $C\in \cset^0$, such that there is at least one terminal $t\in T$ with $v^0(t)\in V(C)$, we include vertex $z(C)$ in set $A_0$. For every terminal $t\in T$ with $v^0(t)\in V(C)$, we include an edge connecting $t$ to $z(C)$, whose length is $2^{\scale(C)}$, in graph $\tH$.


\paragraph{Set $A_L$, for $1\leq L\leq q$.}
Consider an index $1\leq L\leq q$, and assume that sets $A_0,\ldots,A_{L-1}$ have been defined already. For a cluster $C\in \cset^L$, we add vertex $z(C)$ to set $A_L$ if at least one of the following hold:

\begin{itemize}
	\item there  is at least one terminal $t\in T$ with $v^L(t)\in V(H^L)$ and  $v^L(t)\in V(C)$; or
	
	\item there is some level $0\leq L'<L$, and vertex $z(C')\in A_{L'}$, such that supernode $u^L(C')$ lies in $H^L$, and it is marked as an important supernode for cluster $C$.
\end{itemize}

If vertex $z(C)$ belongs to set $A_L$, then its incident edges are defined as follows. First, for every terminal $t\in T$, with $v^L(t)\in V(C)$, we add an edge connecting $t$ to $z(C)$, of length $2^{\scale(C)}$ to graph $\tH$. Additionally, for every level $0\leq L'<L$, for every vertex $z(C')\in A_{L'}$, such that supernode $u^L(C')$ lies in $H^L$, and it is marked as an important supernode for cluster $C$, we add an edge $(z(C'),z(C))$ to graph $\tH$, of length $2^{\scale(C)}$.

This completes the definition of graph $\tH$. 
Recall that we have defined a parameter $\Delta'=2\Delta(W)\cdot \log \hat D\leq O\left(\frac{\Delta(W)\log W}{\eps}\right )$.
We need the following observation.

\begin{observation}\label{obs: size of H}
	For all $\tau\in \tset$, $|V(\tH\attime)|\leq 2|T|\cdot (2\Delta')^{2q+2}$. % and $|E(H\attime)|\leq |T|\cdot \left(\Delta(W)\log W\right )^{O(1/\eps)}$.
\end{observation}
\begin{proof}
	Consider some time $\tau\in \tset$, and the corresponding graph $\tH=\tH\attime$. Whenever we refer to dynamic graphs or data structures in this proof, we refer to them at time $\tau$.
	Recall that data structure $\DS$ ensures that, for all $0\leq L\leq q$, every regular vertex of $H^L$ may lie in at most $\Delta'$ clusters of $\cset^L$.
	We prove by induction on $L$, that, for all $0\leq L\leq q$, $|A_L|\leq |T|\cdot (2\Delta')^{2L+2}$ holds. %, and the number of edges connecting vertices of $T\cup A_0\cup\cdots\cup A_{L-1}$ to vertices of $A_L$ is at most $|T|\cdot (2\Delta')^{2L+2}$.
	
	The base of the induction is when $L=0$. Since every regular vertex of $H^0$ may lie in at most $\Delta'$ clusters of $\cset^0$, it is immediate to verify that $|A_0|\leq |T|\cdot \Delta'$ must hold. %Clearly, the number of edges connecting vertices of $T$ to vertices of $A_0$ is at most $|T|\cdot \Delta'$ as well.
	
	Consider now some level $0<L\leq q$, and assume that the inductive claim holds for levels $0,\ldots,L-1$. As before, every regular vertex of $H^L$ may lie in at most $\Delta'$ clusters of $\cset^L$. Additionally, from \Cref{obs: supernode important in few clusters}, for every supernode $u$ of $H^L$, there are at most $\Delta'$ clusters $C\in \cset^L$, such that $u$ is marked as important for $C$. We conclude that $|A_L|\leq \Delta'\cdot (|T|+|A_0|+\cdots+|A_{L-1}|)$. 
	From the induction hypothesis, we then get that:
	
	\[|A_L|\leq \Delta'\cdot |T|\cdot  \left (1+(2\Delta')^2+(2\Delta')^4+\cdots+(2\Delta')^{2L}\right )\leq |T|\cdot (2\Delta')^{2L+2}.  \]
	

	Overall, we get that $|A_q|\leq |T|\cdot (2\Delta')^{2q+2}$, and $|V(H)|\leq 2|A_q|\leq 2|T|\cdot (2\Delta')^{2q+2}$. %From similar arguments, $|E(H)|\leq 2\cdot (2\Delta')^{2q+2}$. Similarly, $|E(H)|\leq |T|\cdot \left(\Delta(W)\log W\right )^{O(1/\eps)}$.
\end{proof}

%Substituting  $\Delta'=2\Delta(W)\cdot \log \hat D\leq O\left(\frac{\Delta(W)\log W}{\eps}\right )$, and recalling that .


We denote $\beta=2|T|\cdot (2\Delta')^{2q+2}$, so for all $\tau\in \tset$, $|V(\tH\attime)|\leq \beta$ holds.
Recalling that $q=\ceil{1/\eps}$, $\Delta' \leq O\left(\frac{\Delta(W)\log W}{\eps}\right )$, and  $\eps>1/(\log W)^{1/4}$, we get that:

\[\beta\leq |T|\cdot \left(\frac{\Delta(W)\log W}{\eps}\right )^{O(1/\eps)}\leq |T|\cdot \left(\Delta(W)\log W\right )^{O(1/\eps)}.\]

We are now ready to define the dynamic graph $H$. For all $\tau\in \tset$, graph $H\attime$ is obtained from graph $\tH\attime$, by inserting a collection $S$ of $\beta-|V(\tH\attime)|$ isolated vertices, that we refer to as \emph{spare vertices}, into it. Clearly, $|V(H)|=\beta\leq \left(\Delta(W)\log W\right )^{O(1/\eps)}$ always holds.



Next, we provide an algorithm that maintains graph $H$ during time horizon $\tset$, while only using edge-deletion, edge-insertion, isolated vertex-deletion, and vertex-splitting updates.

==> arxiv-version-final/emulator-maintain.tex <==
\subsubsection{Maintaining Graph $H$}
\label{subsubsec: maintaining the emulator}

In this subsection we provide an algorithm that correctly maintains the graph $H$ that we defined in Section \ref{subsubsec: emulator definition}, and bound its total update time. 


At the beginning, before any updates from sequence $\Sigma$ are processed, we initialize the data structure $\DS$ that the algorithm from \Cref{thm: main fully-dynamic APSP single scale} maintains. Recall that, for every level $1\leq L\leq q$, the level-$L$ data structure $\DS_L$ maintains, together with each type-2 supernode $u^L(C)\in V(H^L)$, the list of clusters $C'\in \cset^L$, such that $u^L(C)$ is an important supernode for $C'$, together with pointers to all such clusters. 

Using these data structures it is now immediate to construct the initial graph $H\attime[0]$, in time that is asymptotically bounded by  $O(\beta)$ plus the time that is required in order to initialize data structure $\DS$. 

For convenience, for all $1\leq L\leq q$, we denote by $\event_L$ the event that some level-$L$ phase has terminated. Graph $H$ may need to be updated in one of the following five cases: (i) for some level $1\le L\leq q$, event $\event_L$ has happened; or (ii) for some level $0\leq L\leq q$, a type-1 regular vertex $v^L(x)$ is deleted from some cluster $C\in \cset^L$; or (iii) for some level $1\leq L\leq q$, a type-2 supernode $u^L(C)\in V(H^L)$, and cluster $C'\in \cset^L$, supernode $u^L(C)$ that was important for $C'$ stopped being important for $C'$ (this includes the deletion of the supernode from $C'$); or (iv) some cluster $C\in \cset$ just underwent a cluster-splitting update; or (v) for some level $1\leq L\leq q$, a type-2 supernode $u^L(C)\in V(H^L)$ just underwent a supernode-splitting update. We note that the last event may only happen when cluster $C$ just underwent cluster-splitting, so we will address the last two updates together. We first address the last four updates, and then address the first update.



Assume first that, for some level $0\leq L\leq q$, a type-1 regular vertex $v^L(x)$ is deleted from some cluster $C\in \cset$. We check whether $x\in T$ holds. If this is not the case, then no updates to graph $H$ are needed. Otherwise, vertex $z(C)$ must be present in the current graph $H$. We delete edge $(v^L(x),z(C))$ from $H$. If, as the result, vertex $z(C)$ becomes isolated, then we add it to the set $S$ of spare vertices (this does not require updating the graph $H$).

Assume now that, for some level $1\leq L\leq q$, a type-1 supernode $u^L(C)\in V(H^L)$, and cluster $C'\in \cset^L$, supernode $u^L(C)$ that was important for $C'$ stopped being important for $C'$. 
Assume that $C\in \cset^{L'}$, for some $0\leq L'<L$.
In this case, we check whether vertex $z(C)$ lies in set $A_{L'}$. If this is not the case, no further updates are needed. Assume now that $z(C)\in A_{L'}$. Then $z(C')\in A_L$ must hold. We delete the edge $(z(C),z(C'))$ from graph $H$, and, if vertex $z(C')$ becomes isolated in $H$, then we add it to the set $S$ of spare vertices.

Next, assume that, for some level $0\leq L \leq q$, a cluster $C\in \cset^L$ just underwent a cluster-splitting operation, following which a new cluster $C'\subseteq C$ was added to set $\cset^L$. First, we check whether $z(C)\in V(H)$ holds. If this is not the case, then no further updates are needed. Indeed, since $C'\subseteq C$, and since, from Rule  \ref{rule2 for importance}, a type-2 supernode $u^L(\tilde C)$ may only be important for $C'$ if it is important for $C$, if $z(C)\not\in V(H)$, then we do not need to add vertex $z(C')$  to graph $H$. Assume now that $z(C)\in V(H)$. In this case, we may need to apply a vertex-splitting update to vertex $z(C)$ in order to insert $z(C')$ into $H$. We start by constructing a set $E'\subseteq\delta_H(z(C))$ of edges, as follows. Initially, we let $E'=\emptyset$. We then consider every type-1 regular vertex $v^L(x)\in V(C')$ one by one. For each such vertex $v^L(x)$, we check whether $x\in T$ holds. If so, then we add the edge $(x,z(C))$ to $E'$ (since $C'\subseteq C$, this edge must lie in $H$). Next, we consider every type-2 supernode $u^L(\tilde C)\in V(C')$, that is marked as important for $C'$. For each such supernode $u^L(\tilde C)$, we check whether vertex $z(\tilde C)$ lies in graph $H$. If so, then edge $(z(\tilde C),z(C))$ must be present in $H$, and we add this edge to set $E'$. If the resulting set $E'$ that we constucted so far is empty, then no further updats are needed, as vertex $z(C')$ does not need to be inserted into $H$. Assume now that $E'\neq \emptyset$. In this case, we will need to add vertex $z(C')$ to graph $H$ via a vertex-splitting operation applied to vertex $z(C)$, but we may need to expand the set $E'$ of edges first. Note that the splitting of the cluster $C$ at level $L$ may have triggerred the splitting of the corresponding supernode $u^{L'}(C)$ at levels $L'>L$ for which $u^{L'}(C)\in V(H^L)$ holds. For each such level $L'$, supernode $u^{L'}(C')$ was inserted into the graph $H^{L'}$, and the the list of all clusters $C^*\in \cset^{L'}$ for which supernode $u^{L'}(C')$ is marked as important was initialized.
We consider every level $L'>L$, for which supernode $u^{L'}(C')$ was just inserted into $H^{L'}$, and for each such level $L'$, we consider every custer $C^*\in \cset^{L'}$ for which supernode $u^{L'}(C')$ is marked as important one by one. Consider any such level $L'>L$ and supernode $C^*\in \cset^{L'}$. Note that, from Rule \ref{rule2 for importance}, supernode $u^{L'}(C)$ must be important for cluster $C^*$, and so edge $(z(C),z(C^*))$ currently lies in graph $H$. We add this edge to set $E'$. Once we process all levels $L'>L$, for which supernode $u^{L'}(C')$  was just inserted into $H^{L'}$, and every cluster $C^*\in \cset^{L'}$, such that  $u^{L'}(C')$ is marked as important for $C^*$, we obtain the final set $E'\subseteq \delta_H(z(C))$ of edges. We then apply a vertex-splitting update in graph $H$ to vertex $z(C)$, with the set $E'$ of edges, creating a new vertex $z(C')$. Recall that, for every edge $e=(z(C),x)\in E'$, an edge $(z(C'),x)$, whose length is the same as the length of $e$, is inserted into $H$. Note that the time that is required in order to perform this update is asymptotically bounded by the time that data structure $\DS$ spent in order to split cluster $C$, insert the supernodes $u^{L'}(C')$ into graphs $H^{L'}$ with $L'>L$ for which $u^{L'}(C)\in V(H^{L'})$ holds, and to update the list of clusters $C^*\in\cset^{L'}$ for which the newly inserted supernode $u^{L'}(C')$ is marked as important. We also delete an arbitrary vertex $v\in S$ from graph $H$, in order to ensure that $|V(H)|=\beta$ continues to hold.

Lastly, assume that, at some time $\tau\in \tset$, for some level $L$, event $\event_L$ happens. Let $0<L\leq q$ be the smallest integer, for which event $\event_L$ happens at time $\tau$. Then, for all $L'>L$, event $\event_{L'}$ happens at time $\tau$ as well. Moreover, for each such level $L'>L$, graph $H^{L'}$ is computed from scratch at time $\tau$, it is initialized to be empty, and it will remain empty for the duration of the current level-$L'$ phase. Once the level-$L$ data structure is initialized at time $\tau$, we update graph $H$ as follows. First, we delete all edges incident to the vertices of $A_L\cup\cdots\cup A_q$ from it, and then we add all vertices of $A_L\cup\cdots\cup A_q$ to the set $S$ of spare vertices (the latter does not change the graph $H$). 
Next, we consider every cluster $C\in \cset^L$ one by one. When cluster $C$ is considered, we process every type-1 regular vertex $v^L(x)\in C$ one by one. If, for any such vertex $v^L(x)$, $x\in T$ holds, then we select an arbitrary spare vertex $a\in S$, delete it from $S$, and identify it with vertex $z(C)$. We then add this vertex to set $A_L$, and we connect it with an edge of length $2^{\scale(C)}$ to every terminal $t\in T$ with $v^L(t)\in z(C)$. 
We also process every type-2 supernode $u^L(C')\in V(C)$, that is marked as important for $C$, one by one. For each such such supernode, we check whether vertex $z(C')$ lies in graph $H$. If this is the case, and $z(C)$ has not been added to set $A_L$ yet, we select an arbitrary vertex $a\in S$, delete it from $S$, and identify it with vertex $z(C)$. We then add this vertex to set $A_L$. In any case, we add an edge connecting $z(C')$ to $z(C)$, of length $2^{\scale(C)}$ to graph $H$.
It is easy to verify that cluster $C$ can be processed in time $O(|V(C)|)$.

From the above discussion, the total update time that is required in order to maintain graph $H$ is asymptotically bounded by $O(\beta)$ plus the total update time of data structure $\DS$.
Since $\beta \leq |T|\cdot \left(\Delta(W)\log W\right )^{O(1/\eps)}$, and, from \Cref{thm: main fully-dynamic APSP single scale} the total update time of data structure $\DS$, is bounded by $O\left (W^{1+O(\delta)+O(\eps)}\cdot (\Delta(W)\cdot\log W)^{O(1/\eps^2)}\right )$, we conclude that the total update time of the algorithm is bounded by $O\left (W^{1+O(\delta)+O(\eps)}\cdot (\Delta(W)\cdot\log W)^{O(1/\eps^2)}\right )$.

Consider now some time interval $\tset'\subseteq\tset$, such that update sequence $\Sigma$ for graph $G$ was decremental during $\tset'$. Recall that, from the definition of the hierarchical partition of the time horizon $\tset$ into phases, for all $1\leq L\leq q$, event $\event_L$ may only be triggered by the insertion of an edge into $G$. Therefore, during time interval $\tset'$, no such event may happen. It is then immediate to verify that, during the time interval $\tset'$, graph $H$ may only undergo edge-deletion, isolated vertex-deletion, and vertex-splitting updates.
Next, we prove the following observation.

\begin{observation}\label{obs: number of edges decremental interval}
	Let $\tset'\subseteq \tset$ be any time interval during which update sequence $\Sigma$ for graph $G$ is decremental. Then the total number of edges that are ever present in graph $H$ during $\tset'$ is bounded by $|T|\cdot \left(\Delta(W)\log W\right )^{O(1/\eps)}$.
\end{observation}
\begin{proof}
		Let $\tset'\subseteq \tset$ be any time interval during which update sequence $\Sigma$ for graph $G$ is decremental. 
	For all $0\leq L\leq q$, we denote by $E_L$ the collection of edges that are ever present in $H$ during $\tset'$, and connect vertices of $A_L$ to vertices of $T\cup A_0\cup\cdots\cup A_{L-1}$.
	
	Recall that, for all $0\leq L'\leq q$, time interval $\tset'$ is contained in a single level-$L'$ phase. Recall also that data structure $\DS$ guarantees that, over the course of a single level-$L$ phase, a regular vertex may belong to at most $\Delta'$ clusters of $\cset^L$. Moreover, from \Cref{obs: supernode important in few clusters}, for every type-2 supernode $u$ of $H^L$, there may be at most $\Delta'$ clusters $C\in \cset^L$, such that $u$ was ever important for $C$ over the course of a single level-$L$ phase. We conclude that $|E_L|\leq \Delta'\cdot(|T|+|A_0|+\cdots+|A_{L-1}|)\leq \Delta'\cdot \beta$.
	
	Overall, we get that the total number of edges ever present in graph $H$ is bounded by:
	
	\[\sum_{L=0}^q|E_L|\leq (q+1)\cdot \Delta'\cdot \beta\leq  |T|\cdot \left(\Delta(W)\log W\right )^{O(1/\eps)} \]
	
	(we have used the fact that $\beta\leq |T|\cdot \left(\Delta(W)\log W\right )^{O(1/\eps)}$, $q=\ceil{1/\eps}$, $\Delta'\leq O\left(\frac{\Delta(W)\log W}{\eps}\right )$,  and $\eps>1/(\log W)^{1/4}$).
\end{proof}


It now remains to prove that graph $H$ is indeed a valid $D^*$-restricted $T$-emulator, to bound its stretch, and to provide an algorithm for the $\transformpath$ queries. We do all this in the next subsection.

==> arxiv-version-final/intro-backup.tex <==

\section{Introduction}
\label{sec: intro}
We study the fully dynamic All-Pairs Shortest-Paths (\APSP) problem  in weighted undirected graphs. 
In this problem, the input is an undirected $n$-vertex graph $G$ with lengths $\ell(e)\geq 1$ on its edges, that undergoes an online sequence of edge insertions and deletions. The goal is to support (approximate) shortest-path queries $\shortestpathquery(x,y)$: given a pair $x,y$ of vertices of $G$, return a path connecting $x$ to $y$, whose length is within factor $\alpha$ of the length of the shortest $x$-$y$ path in $G$, where $\alpha$ is the \emph{approximation factor} of the algorithm. We also consider approximate distance queries, $\distquery(x,y)$: given a pair $x,y$ of vertices of $G$, return an estimate $\dist'(x,y)$ on the distance $\dist_G(x,y)$ between $x$ and $y$ in $G$, such that $\dist_G(x,y)\leq \dist'(x,y)\leq \alpha\cdot \dist_G(x,y)$. 
Throughout, we denote $|V(G)|=n$, and we denote by $m$ the total number of edges that are ever present in $G$; if an edge is deleted from $G$ and then inserted into $G$ multiple times, we count these as different edges. We also denote by $\Lambda$ the ratio of longest to shortest edge length.

\APSP is one of the most fundamental problems in graph algorithms, both in the dynamic and the static settings. Algorithms for this problem often serve as building blocks for designing algorithms for a range of other graph problems and beyond. Interestingly, algorithms for dynamic \APSP turned out to be extremely useful in the design of fast algorithms for classical cut, flow, and other graph problems in the static setting. 
Not surprisingly, this problem has been the subject of extensive study, from many different angles and in various regimes. 

A central goal in this area is to obtain algorithms with the strongest possible guarantees for the problem. Specifically, we would like the approximation factor $\alpha$ that the algorithm achieves to be low, and its total update time\footnote{In the context of fully dynamic algorithms, it is customary to focus on amortized update time per operation, which, in our case, is simply the total update time divided by $m$. We will use total update time and amortized update time per operation interchangeably, but we will try to clearly distinguish between them to avoid confusion.} -- the time required to maintain its data structures -- as close as possible to linear in $m$. In addition to the approximation factor and the total update time, other important parameter is  \emph{query time} -- the time it takes to process a single query. Ideally, we would like  the query time for $\shortestpathquery$ to be close to $ O(|E(P)|)$, where $P$ is the path that the algorithm returns, which is the best query time we can hope for.   Lastly, we distinguish between the \emph{oblivious-adversary} setting, where the sequence of updates to graph $G$ is constructed in advance and may not depend on the algorithm's behavior, and the \emph{adaptive-adversary} setting, where each update to graph $G$ may  depend arbitrarily on the algorithm's inner state and past behavior, such as responses to queries. While the oblivious-adversary setting appears significantly easier to handle algorithmically, many applications that rely on algorithms for dynamic \APSP require that the algorithm works in the adaptive-adversary setting. It is well known that deterministic algorithms always work against an adaptive adversary. Seeing that the \APSP problem itself is used as a building block in many different other setting,  designing a deterministic algorithm for the problem is especially desirable.

A straightforward algorithm for the fully-dynamic \APSP problem is the following: every time a query $\shortestpathquery(x,y)$ arrives, compute the shortest $x$-$y$ path in $G$ from scratch. This algorithm solves the problem exactly, but it has query time $\Theta(m)$. Another approach is to rely on \emph{spanners}. A spanner of a dynamic graph $G$ is another dynamic graph $H\subseteq G$, with $V(H)=V(G)$, such that the distances between the vertices of $G$ are approximately preserved in $H$; ideally a spanner $H$ should be very sparse. For example, a work of
\cite{BaswanaKS12} provides a randomized algorithm that maintains a spanner of a fully dynamic $n$-vertex graph $G$, that, for any parameter $k\leq O(\log n)$, achieves approximation factor $(2k-1)$, has expected amortized update time $O(k^2\log^2n)$ per update operation, and expected spanner size $O(kn^{1+1/k}\log n)$. Unfortunately, this algorithm only works against an oblivious adversary.
A recent work of
\cite{new-spanner} provides a randomized algorithm for maintaining a spanner of a fully dynamic $n$-vertex graph $G$ that can withstand an adaptive adversary. The algorithm achieves approximation factor $O(\poly\log n)$ and total update time $\Otilde(m)$, and it ensures that the number of edges in the spanner $H$ is always bounded by $O(n\poly\log n)$.  An algorithm for the \APSP problem can naturally build on such  constructions of spanners: given a query $\shortestpathquery(x,y)$ or $\distquery(x,y)$, we simply compute the shortest $x$-$y$ path in the spanner $H$. For example, the algorithm for graph spanners of \cite{new-spanner} implies a randomized $\poly\log n$-approximation algorithm for \APSP that has $O(m\poly\log n)$ total update time.
A recent work of \cite{newest-spanner} provides additional spanner-based algorithms for \APSP. 
Unfortunately, it seems inevitable that this straightforward spanner-based approach to \APSP  must have query time $\Omega(n)$ for both $\shortestpathquery$ and \distquery, and, with current state of the art algorithms, cannot lead to a better than logarithmic approximation. 

In this paper, our focus is on developing algorithms for the \APSP problem, whose query time is $ O(|E(P)|\cdot \poly\log(n\cdot \Lambda))$ for $\shortestpathquery$, where $P$ is the path that the query returns, and $O(\poly\log(n\cdot \Lambda))$ for $\distquery$. %While, in the worst case, it is possible that $P$ contains $\Theta(n)$ edges, this may not be the case typically. 
There are several reasons to strive for these faster query times. First, we typically want responses to the queries to be computed as fast as possible, and the above query times are close to the fastest possible. Second, ensuring that query time for $\shortestpathquery$ is bounded by $ O(|E(P)|\cdot \poly\log(n\cdot \Lambda))$ is often crucial to obtaining fast algorithms for other static graph problems, that use algorithms for \APSP as a subroutine.


%We distinguish between dynamic algorithms that work against an \emph{oblivious adversary}, where the input sequence of edge deletions is fixed in advance and may not depend on the algorithm's past behavior, and algorithms that work against an \emph{adaptive adversary}, where the input update sequence may depend on the algorithm's past responses and inner states arbitrarily. We refer to the former as \emph{oblivious-update} and to the latter as \emph{adaptive-update} algorithms. We note that any deterministic algorithm for the \APSP problem is an adaptive-update algorithm by definition.


As mentioned already, there are several parameters of interest that we would like to optimize in algorithms for \APSP: namely, query time, total update time, and approximation factor. Additionally, we would like the algorithm to withstand an adaptive adversary, and ideally to be deterministic. There is a huge body of work that studies the \APSP problem, in both the dynamic and the static settings, that tries to optimize or achieve various tradeoffs among these different parameters. Some of this work also only focuses on supporting $\distquery$ queries, and not $\shortestpathquery$. We do not attempt to survey all of this work here, partially because this seems impossible, and partially because it may lead to confusion due to the large number of different settings considered. Instead, we will restrict our attention to the adaptive-adversary setting, where the query time for $\shortestpathquery$ is  $ O(|E(P)|\cdot \poly\log(n\cdot \Lambda))$, where $P$ is the returned path, and query time for  $\distquery(x,y)$ is $O(\poly\log(n\cdot \Lambda))$. We will try to survey the most relevant results for this setting, in order to put our results in context with previous work. We will also include some results for \APSP in \emph{decremental} graphs, where only edge-deletion updates are allowed.



{\bf Low-approximation regime.}
One major direction of study is to obtain algorithms for \APSP whose approximation factor  is very close to $1$. 
The classical data structure of Even and Shiloach \cite{EvenS,Dinitz,HenzingerKing}, that we refer to as \EST throughout the paper, implies an exact deterministic
algorithm for decremental unweighted $\APSP$ with $O(mn^{2})$ total update time, and the desired $O(|E(P)|)$ query time for $\shortestpathquery$, where $P$ is the returned path. 
Short of obtaining an exact algorithm for \APSP, the best possible approximation factor one may hope for is $(1+\eps)$, for any $\eps$. A long line of work is dedicated to this direction in the decremental setting \cite{BaswanaHS07,rodittyZ2,henzinger16,bernstein16} 
and in the fully dynamic setting \cite{demetrescu2004new,thorup2004fully,brand2021fast}. In the decremental setting, the fastest algorithms in this line of work, due to \cite{henzinger16} and \cite{bernstein16}, achieve total update time $\tilde{O}(mn/\epsilon)$; the former algorithm is deterministic but only works in unweighted undirected graphs, while the latter algorithm works in directed weighted graphs, with an overhead of $\log \Lambda$ in the total update time, but can only handle an oblivious adversary. In the fully-dynamic setting, all algorithms cited above have amortized update time per operation at least $\Omega(n^2)$. 
A very recent result of \cite{bernstein2022deterministic} obtained a $(2+\eps)$-approximation for fully-dynamic \APSP, with amortized update time $O(m^{1+o(1)})$ per operation.
The high running times of the above mentioned algorithms are perhaps not surprising in view of strong lower bounds that are known for the low-approximation setting.




{\bf Lower Bounds.} 
A number of lower bounds are known for dynamic \APSP with low approximation factor. For example, Dor, Halperin and Zwick \cite{DorHZ00}, and Roddity and Zwick \cite{RodittyZ11} showed that, assuming the Boolean Matrix Multiplication (BMM) conjecture\footnote{The conjecture states that
	there is no ``combinatorial'' algorithm for multiplying two Boolean matrices of size $n\times n$ in time $n^{3-\delta}$ for any constant $\delta>0$.}, for any $\alpha,\beta\geq 1$ with $2\alpha+\beta<4$, no combinatorial algorithm for \APSP achieves a multiplicative $\alpha$ and additive $\beta$ approximation, with total update time
$O(n^{3-\delta})$ and query time $O(n^{1-\delta})$ for \distquery, for any constant $0<\delta<1$. This result was generalized by \cite{HenzingerKNS15}, who showed the same lower bounds for all algorithms and not just combinatorial ones, assuming the Online Boolean Matrix-Vector Multiplication (OMV) conjecture\footnote{The conjecture assumes that there is no $n^{3-\delta}$-time algorithm, for any constant $0<\delta<1$, for the OMV problem, in which the input is a Bollean $(n\times n)$ matrix, with $n$ Boolean dimension-$n$ vectors $v_1,\ldots,v_n$ arriving online. The algorithm needs to output $Mv_i$ immediately after $v_i$ arrives.}. 
The work of Vassilevska Williams and Williams \cite{williams2018subcubic}, combined with the work of  Roddity and Zwick \cite{RodittyZ11}, implies that obtaining such an algorithm would lead to subcubic-time algorithms for a number of important static problems on graphs and matrices.
A very recent result of \cite{abboud2022hardness} provides new lower bounds for the dynamic \APSP problem, in the regime where only \distquery queries need to be supported, under either the 3-SUM conjecture or the APSP conjecture. Let $k\geq 4$ be an integer, let $\eps,\delta>0$ be parameters, and let $c=\frac{4}{3-\omega}$ and $d=\frac{2\omega-2}{3-\omega}$, where $\omega$ is the exponent of matrix multiplication. Then \cite{abboud2022hardness}  show that, assuming either the 3-SUM Conjecture or the APSP Conjecture, there is no $(k-\delta)$-approximation algorithm for decremental \APSP with total update time  $O(m^{1+\frac{1}{ck-d}-\eps})$ and query time for \distquery bounded by $O(m^{\frac{1}{ck-d}-\eps})$. They also show that there is no $(k-\delta)$-approximation algorithm for fully dynamic \APSP that has   $O(n^3)$ preprocessing time, and then supports (fully dynamic) updates and \distquery queries in $O(m^{\frac{1}{ck-d}-\eps})$ time.
Due to these lower bounds, it is natural to focus on somewhat higher approximation factors.

{\bf Higher approximation factor.}
In the regime of higher approximation factors, a long line of work \cite{BernsteinR11,henzinger16,abraham2014fully,HenzingerKN14_focs} focused on the decremental setting with an oblivious adversary. This direction recently culminated with an algorithm of Chechik~\cite{chechik}, that, for any integer $k\ge1$ and parameter $0<\eps<1$, obtains a
$((2+\epsilon)k-1)$-approximation, with total update time $O(mn^{1/k+o(1)}\cdot \log  \Lambda)$, when the input graph is  weighted and undirected. This result is near-optimal, as all its parameters almost match
the best static algorithm of \cite{TZ}. This result was recently slightly improved by \cite{lkacki2020near}, who obtain total update time $O(mn^{1/k}\cdot \log \Lambda)$, and improve query time for $\dquery$.

The best currently known results for the fully dynamic setting with an oblivious adversary are significantly weaker. 
%
%Several algorithms are also known for fully dynamic \APSP in the oblivious setting, that only support approximate \distquery.
For unweighted graphs, the algorithm of \cite{ForsterG19} achieves approximation factor $n^{o(1)}$, with amortized update time $n^{1/2+o(1)}$ per operation  on unweighted graphs, while
the algorithm of \cite{abraham2014fully} achieves a constant approximation factor with expected $o(m)$ amortized update time per operation. In fact the latter paper provides a more general tradeoff between the approximation factor and update time, but in all regimes the expected amortized update time is at least $\Theta(\sqrt m)$ per operation. Lastly, the 
 the algorithm of \cite{ForsterGH20}, based on low-stretch trees, achieves $O(m^{\eps})$ update time per operation, with a factor  $(\log n)^{O(1/\eps)}$-approximation in weighted graphs. All of the above mentioned algorithms for fully-dynamic \APSP with oblivious adversary only support \distquery. We are not aware of algorithms that can additionally support \shortestpathquery.


In contrast, progress in the adaptive-update setting has been much slower. Until very recently, the fastest algorithm for decremental unweighted graphs 
\cite{henzinger16,GutenbergW20} only achieved an $\tilde{O}(mn/\epsilon)$ total update time (for approximation factor $(1+\eps)$), and the work of 
\cite{APSP-old}, for any parameter $1\le k\le o(\log^{1/8}n)$, achieved a multiplicative $3\cdot 2^{k}$ and additive $2^{(O(k\log^{3/4}n)}$ approximation, with query time $O(|E(P)|\cdot n^{o(1)})$ for $\shortestpathquery$, and total update time $n^{2.5+2/k+o(1)}$. Until very recently, the fastest  adaptive-update algorithms for {\bf weighted} graphs had total update time $O\left(\frac{n^{3}\log \Lambda}{\eps}\right )$ and approximation factor $(1+\eps)$ (see \cite{reliable-hubs}), even in the {\bf decremental} setting. 

To summarize, to the best of our knowledge, until very recently, even if we allowed an $o(n)$-approximation factor,
no adaptive-update algorithms with better than $\Theta(n^{3})$ total
update time and better than $\Theta(n)$ query time for $\shortestpathquery$ and $\distquery$ were known for weighted undirected graphs, 
and no adaptive-update algorithms with better than $\Theta(n^{2.5})$ total update time  and better than $\Theta(n)$ query time were known for unweighted undirected graphs, even in the {\bf decremental} setting.

Two very recent results\footnote{To the best of our knowledge, the two results are independent.} provided significantly stronger algorithms for decremental \APSP in weighted graphs: \cite{APSP-previous} designed a deterministic algorithm, that, for any $\Omega(1/\log\log m)<\eps<1$, achieves approximation factor 
$(\log m)^{2^{O(1/\eps)}}$, and has total update time $O\left (m^{1+O(\eps)}\cdot (\log m)^{O(1/\eps^2)}\cdot \log \Lambda\right )$. The query time is  $O(\log m \log\log \Lambda)$ for $\distquery$, and   $O(|E(P)|+\log m \log\log \Lambda)$ for $\shortestpathquery$, where $P$ is the returned path.
The main focus of \cite{bernstein2022deterministic} was mostly on a special case of \APSP called Single Source Shortest Paths (\SSSP), but they also obtained a deterministic algorithm for decremental \APSP with approximation factor $m^{o(1)}$ and total update time $O(m^{1+o(1)})$; unfortunately, the tradeoff between the approximation factor and the total update time is not stated explicitly, though they mention that the approximation factor is super-logarithmic. As mentioned already, they also obtain new results in the low-approximation regime for the fully dynamic setting of \APSP: a $(2+\eps)$-approximation with amortized update time $O(m^{1+o(1)})$ per operation.


In this paper we improve the results of \cite{APSP-previous} in two ways. First, we extend the algorithm to the fully-dynamic setting, and second, we improve the approximation factor to $(\log\log m)^{2^{O(1/\eps^3)}}$.
Altogether, we obtain a deterministic algorithm for fully-dynamic \APSP, that, given  a precision parameter $\frac{2}{(\log n)^{1/200}}<\eps<1/400$, achieves approximation factor $\alpha=(\log\log n)^{2^{O(1/\eps^2)}}$, and has amortized update time $O\left (n^{O(\eps)}\cdot \log \Lambda\right )$ per operation (if starting from an empty graph). Query time for \distquery is $O\left (2^{O(1/\eps)}\cdot \log n\cdot \log \log \Lambda\right )$, and query time for $\shortestpathquery$ is  $O\left (|E(P)|+2^{O(1/\eps)}\cdot \log n\cdot \log\log \Lambda\right )$, where $P$ is the path that the algorithm returns (note that, if we choose $\eps\geq 1/\log\log n$, then query time for $\distquery$ becomes $O(\poly\log(n\cdot \Lambda)$, and query time for $\shortestpathquery$ becomes $\tilde O(|E(P)|)$).
An important intermediate problem that we study is Sparse Neighborhood Cover, and its generalization called Recursive Dynamic Neighborhood Cover (\recdynnc) that we discuss next.

{\bf Sparse Neighborhood Cover and \recdynnc problem.} 
Given a graph $G$ with lengths on edges, a vertex $v\in V(G)$, and a distance parameter $D$, we denote by $B_G(v,D)$ the \emph{ball of radius $D$ around $v$}, that is, the set of all vertices $u$ with $\dist_G(v,u)\leq D$.
Suppose we are given a static graph $G$ with non-negative edge lengths, a distance parameter $D$, and a desired approximation factor $\alpha$. A $(D,\alpha\cdot D)$-\emph{neighborhood cover} for $G$ is a collection $\cset$ of vertex-induced subgraphs of $G$ (that we call \emph{clusters}), such that, for every vertex $v\in V(G)$, there is some cluster $C\in \cset$ with $B_G(v,D)\subseteq V(C)$. Additionally, we require that, for every cluster $C\in \cset$, for every pair $x,y\in V(C)$ of its vertices, $\dist_G(x,y)\leq \alpha\cdot D$; if this property holds, then we say that $\cset$ is a \emph{weak} $(D,\alpha\cdot D)$-neighborhood cover of $G$. If, additionally, the diameter of every cluster $C\in \cset$ is bounded by $\alpha\cdot D$, then we say that  $\cset$ is a \emph{strong} $(D,\alpha\cdot D)$-neighborhood cover of $G$. Ideally, it is also desirable that the neighborhood cover is \emph{sparse}, that is, every edge (or every vertex) of $G$ only lies in a small number of clusters of $\cset$. For this static setting of the problem, the work of \cite{neighborhood-cover2,neighborhood-cover1} provides a deterministic algorithm that produces a strong $(D,O(D\log n))$-neighborhood cover of graph $G$, where every edge lies in at most $O(\log n)$ clusters, with running time $\Otilde(|E(G)|+|V(G)|)$.


In \cite{APSP-previous} a new problem, called Recursive Dynamic Neighborhood Cover (\recdynnc) was introduced. The problem can be viewed as an adaptation of Sparse Neighborhood Covers to the dynamic (decremental) setting, but with additional constraints that make it easy to use as a building block in other dynamic algorithms.
The input to this problem is a bipartite graph $H=(V,U,E)$, with non-negative lengths $\ell(e)$ on edges $e\in E$, and a distance parameter $D$. Vertices in set $V$ are called \emph{regular vertices}, while vertices in set $U$ are called \emph{supernodes}. Graph $H$ undergoes an online sequence $\Sigma$ of updates, each of which must be of one of the following three kinds: (i) edge deletion; or (ii) isolated vertex deletion; or (iii) supernode splitting. In the latter kind of update, we are given a supernode $u\in U$, and a collection $E'\subseteq \delta_H(u)$ of its incident edges. We need to insert a new supernode $u'$ into $H$, and, for every edge $e=(u,v)\in E'$, insert an edge $(u',v)$ into $H$. We note that, while, in general, graph $H$ is decremental, the supernode-splitting update allows us to insert edges into it, in a limited fashion. For conciseness, we will refer to an input $\iset=\left(H=(V,U,E),\set{\ell(e)}_{e\in E},D \right )$  as described above, as \emph{valid input structure}, and to edge-deletion, isolated vertex-deletion, and supernode-splitting updates as \emph{valid update operations}. Note that edges may be inserted into graph $H$ via supernode-splitting updates. In order to control the size of the resulting graph, another parameter called \emph{dynamic degree bound} is used. We say that the dynamic degree bound of valid update structure $\iset$ that undergoes a sequence $\Sigma$ of valid update operations is $\mu$ if, for every regular vertex $v$, the total number of edges that are ever present in $H$ and are incident to $v$, is bounded by $\mu$.

The goal in the \recdynnc problem is to maintain a weak $(D,\alpha\cdot D)$-neighborhood cover $\cset$ of the graph $H$. However, we require that the clusters in $\cset$ are only updated in a specific fashion: once an initial neighborhood cover $\cset$ of $H$  is computed, we can only update clusters via \emph{allowed changes}: for each cluster $C$, we can delete edges or vertices from $C$, and, additionally, if some supernode $u\in V(C)$ just underwent a supernode-splitting update, we can insert the resulting new supernode $u'$ and all edges connecting it to other vertices of $C$, into cluster $C$. A new cluster $C'$ may only be added to $\cset$, if there is a cluster $C\in \cset$ with $C'\subseteq C$. In this case, we say that cluster $C$ underwent a \emph{cluster-splitting} update.  The algorithm must also maintain, for every regular vertex $v$ of $H$, a cluster $C=\coveringcluster(v)\in\cset$, with $B_H(v,D)\subseteq V(C)$. Additionally, we require that the neighborhood cover is \emph{sparse}, namely, for every regular vertex $v$ of $H$, the total number of clusters of $\cset$ to which $v$ may ever belong over the course of the algorithm is small. 
Lastly, we require that the algorithm supports  queries $\spquery(C,v,v')$: given two  vertices $v,v'\in V$, and a cluster $C\in \cset$ with $v,v'\in C$, return a path $P$ in the current graph $H$, of length at most $\alpha\cdot D$ connecting $v$ to $v'$ in $G$, in time $O(|E(P)|)$, where $\alpha$ is the approximation factor of the algorithm.

Given any edge-weighted decremental graph $G$ and a distance bound $D$, it is easy to transform $G$ into a valid input structure: we simply view the vertices of $G$ as supernodes, and we subdivide its edges with new vertices, that become regular vertices in the resulting bipartite graph $H$. An algorithm for solving the \recdynnc problem on the resulting valid input structure $\iset$ (that only undergoes edge-deletion updates) then naturally allows us to maintain a sparse neighborhood cover in the original graph $G$. However, the specific definition of the \recdynnc problem makes it more versatile, and more specifically, we can naturally  compose instances of the problem recursively with one another.

A typical way to exploit this composability property is the following. Suppose we solve the \recdynnc problem on a bipartite graph $H$, with some distance bound $D$. Let $\cset$ be the collection of clusters that the resulting algorithm maintains. Assume now that we would like to solve the same problem on graph $H$, with a larger distance bound $D'>D$. We can then construct another graph $H'$, whose set of regular vertices is the same as that in $H$, and the set of supernodes is $\set{u(C)\mid C\in \cset}$. We add an edge $(v,u(C))$ to the graph if and only if regular vertex $v$ lies in cluster $C\in \cset$, and we set the lengths of the resulting edges to be $D$. As the clusters in $\cset$ evolve, we can maintain graph $H'$ via valid update operations: when some cluster $C\in \cset$ undergoes cluster-splitting, and a new cluster $C'\subseteq C$ is created, we can apply supernode-splitting to supernode $u(C)$ in order to update graph $H'$ accordingly. It is not hard to verify that the resulting graph $H'$ is an emulator for $H$, with respect to distances that are greater than $D$. We can then scale all edge lengths down by factor $D$, and solve the problem on graph $H'$, with a new, significantly smaller, distance parameter $D'/D$. If neighborhood over $\cset$ is sparse, and every regular vertex of $H$ ever belongs to at most $\Delta$ clusters of $\cset$, then the dynamic degree bound for graph $H'$ is bounded by $\Delta$, so graph $H'$ itself is sparse.


We note that, while the \recdynnc problem was first formally defined in \cite{APSP-previous}, the idea of using clustering of a dynamic graph $G$ in order to construct an emulator was exploited before numerous times (see e.g. the constructions of \cite{ForsterG19,chechikLowStretch,ForsterGH20} of dynamic low-stretch spanning trees). In several of these works, a family of clusters of a dynamic graph $G$ is constructed and maintained, and the restrictions on the allowed updates to the cluster family are similar to the ones that we impose; it is also observed in several of these works that with such restrictions one can naturally compose the resulting emulators recursively -- an approach that we follow here as well.
While neither of these algorithms provide neighborhood covers (as can be observed from the fact that one can view the sets of clusters that are maintained for each distance scale as disjoint, something that cannot be achieved in neighborhood covers), a connection between low-diameter decompositions (that often serve as the basis of low-stretch spanning trees) and neighborhood covers has been noticed in prior work. For example, \cite{miller2015improved}, provide a construction of neighborhood covers from low-diameter decompositions.
Additionally, all the above-mentioned algorithms are randomized and assume an oblivious adversary. On the other hand,  \cite{henzinger16,GutenbergW20} implicitly provide a deterministic algorithm for maintaining a neighborhood cover of a dynamic graph. However, these algorithms have a number of drawbacks: first, the running time for maintaining the neighborhood cover is too prohibitive (the total update time is $O(mn)$). Second, the neighborhood cover maintained is not necessarily sparse; in fact a vertex may lie in a very large number of resulting clusters. Lastly, clusters that join the neighborhood cover as the algorithm progresses may be arbitrary. The restriction that, for every cluster $C$ added to the neighborhood cover $\cset$, there must be a cluster $C'$ containing $C$ that already belongs to $\cset$, seems crucial in order to allow an easy recursive composition of emulators obtained from the neighborhood covers, and the requirement that the neighborhood cover is sparse is essential for bounding the sizes of the graphs that arise as the result of such recursive compositions. We also note that
a similar approach of recursive composition of emulators was used in numerous algorithms for \APSP  (see, e.g. \cite{chechik}), and a similar approach to handling cluster-splitting in an emulator that is based on clustering was used before in numerous works, including, e.g., \cite{BernsteinChechik,Bernstein,fast-vertex-sparsest,chechikLowStretch}.



It is not hard to verify that an algorithm for the \recdynnc problem immediately implies an algorithm for {\bf decremental} \APSP with the same approximation factor, and the same total update time (to within $O(\log \Lambda)$-factor). In \cite{APSP-previous}, a deterministic algorithm for the \recdynnc problem  was provided, with approximation factor $\alpha=O\left ((\log m)^{2^{O(1/\eps)}}\right )$, and total update time $O\left (m^{1+O(\eps)}\cdot (\log m)^{O(1/\eps^2)}\right )$. The algorithm ensured that, for every regular vertex $v\in V(H)$, the total number of clusters of $ \cset$ that $v$ ever belongs to is bounded by $m^{O(1/\log\log m)}$. 

In this work, we improve the results of \cite{APSP-previous} in two ways. First, we provide a black-box reduction from the $\recdynnc$ problem to fully dynamic \APSP. Second, we provide an improved algorithm for the \recdynnc problem. The algorithm, given a valid input structure  $\iset=\left(H,\set{\ell(e)}_{e\in E(H)},D \right )$ undergoing a sequence of valid update operations, with dynamic degree bound $\mu$, together with parameters $\hat W$ and  $1/(\log \hat W)^{1/100}\leq \eps<1/400$,  such that, if we denote by $N$ the number of regular vertices in $H$ at the beginning of the algorithm, then $N\cdot \mu= \hat W$ holds, achieves approximation factor $\alpha=(\log\log \hat W)^{2^{O(1/\eps^2)}}$,  with total update time $O(N^{1+O(\eps)}\cdot \mu^{O(1/\eps)})$. The algorithm also ensures that, for every regular vertex $v$, the total number of clusters in the weak neighborhood cover $\cset$ that the algorithm maintains, to which vertex $v$ ever belongs over the course of the algorithm, is bounded by $\hat W^{4\eps^3}$. By combining these two results, we obtain a deterministic algorithm for the fully dynamic \APSP problem, that, given a precision parameter $\frac{2}{(\log n)^{1/200}}<\eps<1/400$, achieves approximation factor $\alpha=(\log\log n)^{2^{O(1/\eps^2)}}$, and has amortized update time $O\left (n^{O(\eps)}\cdot \log \Lambda\right )$ per operation, with query time $O\left (2^{O(1/\eps)}\cdot \log n\cdot \log \log \Lambda\right )$ for \distquery  and query time   $O\left (|E(P)|+2^{O(1/\eps)}\cdot \log n\cdot \log\log \Lambda\right )$ for \pathquery, where $P$ is the path that the algorithm returns.
We now state our results more formally, and discuss the techniques that we employ, while pointing out specific remaining bottlenecks for obtaining a better tradeoff between the approximation factor and the update time of the algorithm.


%\input{old-results-techniques}
\subsection{Our Results}


As mentioned already, a problem that plays a central role in this work is \recdynnc. We do not repeat the definition of the problem from above; a formal (and equivalent) definition can be found in \Cref{sec: valid inputs}. However, the definition that we provided above omitted one technical detail: the Consistent Covering requirement.

Suppose we are given a valid input structure $\iset=\left(H=(V,U,E),\set{\ell(e)}_{e\in E},D \right )$ undergoing an online sequence $\Sigma$ of valid update operations. Let $\tset$ be the time horizon associated with $\Sigma$. In order to define the Consistent Covering property, we first need to define the notion of \emph{ancestor-clusters}. This notion is defined in a natural way. If $C$ is a cluster that is present in $\cset$ at the beginning of the algorithm, then for all $\tau\in \tset$, $\anc\attime(C)=C$, so $C$ is its own ancestor. Assume now that $C'$ is a cluster that was added to set $\cset$ at some time $\tau'>0$, by applying a cluster-splitting update to a cluster $C\in \cset$. Then for all $\tau\in \tset$, if $\tau<\tau'$, $\anc\attime(C')=\anc\attime(C)$, and otherwise $\anc\attime(C')=C'$.

We are now ready to define the Consistent Covering property. Consider an algorithm for the \recdynnc problem on input $(\iset,\Sigma)$, and let $\cset$ be the collection of cluster that it maintains. We say that the algorithm obeys the Consistent Covering property, if, for every regular vertex $v\in V(H)$, for every pair $\tau'<\tau\in \tset$ of time points, if $C=\coveringcluster(v)$ at time $\tau$, and $\anc\attime[\tau'](C)=C'$, then, at time $\tau'$, $B_{H}(v,D)\subseteq V(C')$ held. We require that algorithms for the \recdynnc problem obey the Consistent Covering property.
Our first result is a reduction from \recdynnc to a variant of fully-dynamic \APSP.


\subsubsection{Reduction from \recdynnc to Fully-Dynamic \APSP}

We provide a black-box reduction from \recdynnc to fully-dynamic \APSP.
Our reduction shows that, if there exists an algorithm for the \recdynnc problem with some general set of parameters, then we can convert it into an algorithm for the fully-dynamic \APSP problem. The assumption on the existence of an algorithm for \recdynnc, that serves as the starting point of the reduction, is the following.


\begin{assumption}\label{assumption: alg for recdynnc2}
	There is a deterministic algorithm for the \recdynNC problem, that,  given a valid input structure $\iset=\left(H=(V,U,E),\set{\ell(e)}_{e\in E},D \right )$ undergoing a sequence of valid update operations, with dynamic degree bound $\mu$, together with parameters $\hat W$ and  $1/(\log \hat W)^{1/100}\leq \eps<1/400$,  such that, if we denote by $N$ the number of regular vertices in $H$ at the beginning of the algorithm, then $N\cdot \mu\leq \hat W$ holds, achieves approximation factor $\alpha(\hat W)$,  with total update time $O(N^{1+O(\eps)}\cdot \mu^{O(1/\eps)})$. Moreover, the algorithm ensures that, for every regular vertex $v\in V$, the total number of clusters in the weak neighborhood cover $\cset$ that the algorithm maintains, to which vertex $v$ ever belongs over the course of the algorithm, is bounded by $\hat W^{4\eps^3}$. Here, $\alpha(\cdot)$ is a non-decreasing function.
\end{assumption}

If \Cref{assumption: alg for recdynnc2} holds, then it is quite easy to obtain an algorithm for decremental \APSP (see Section 3.4.2 in the full version \cite{APSP-previous}), that, on an input graph $G$ that initially has $m$ edges, has total update time $O(m^{1+O(\eps)+o(1)} (\log m)^{O(1/\eps)} \log \Lambda)$, and achieves an approximation factor roughly $\alpha(m)$. One of the main contributions of this work is showing that an algorithm for the \RecDynNC problem implies an algorithm for {\bf fully-dynamic} \APSP. 
Specifically, we show that, assuming \Cref{assumption: alg for recdynnc2}, there is an algorithm for a problem that is very similar to, but is slightly different from fully-dynamic \APSP. We call this problem $D^*$-restricted \APSP, and define it next. For a dynamic graph $G$ and time $\tau$, we denote by $G\attime$ the graph $G$ at time $\tau$.

\begin{definition}[$D^*$-restricted \APSP problem]\label{def: bounded APSP}
	The input to the $D^*$-restricted \APSP problem is 
	an $n$-vertex graph $G$ with integral lengths $\ell(e)\geq 1$ on its edges $e\in E(G)$,
	that undergoes an online sequence $\Sigma$ of edge deletions and insertions, together with a precision parameter $\frac{1}{(\log n)^{1/200}}<\eps<1/400$, and a distance parameter $D^*>0$. The goal is to support approximate \shortpath\ queries: given a pair $x,y\in V(G)$ of vertices, the algorithm needs to respond ``YES'' or ''NO'', in time $O\left(2^{O(1/\eps)}\cdot \log n\right )$. If the response is ``NO'', then $\dist_G(x,y)>D^*$ must hold. If the response is ``YES'', then the algorithm should be able, additionally, to compute a path $P$ in the current graph $G$, connecting $x$ to $y$, of length at most $\alpha'\cdot D^*$, in time $O(|E(P)|)$, where $\alpha'$ is the \emph{approximation factor} of the algorithm.
\end{definition}


The following theorem summarizes our reduction from \recdynnc to $D^*$-restricted \APSP.




\begin{theorem}\label{thm: main fully-dynamic APSP single scale}
	Suppose \Cref{assumption: alg for recdynnc2} holds. Then there is a deterministic algorithm for the $D^*$-restricted $\APSP$ problem,  that achieves approximation factor $\alpha'=(\alpha(n^3))^{O(1/\eps)}$, and has amortized update time at most $n^{O(\eps)}$ per operation, if starting from an empty graph.
\end{theorem}



\iffalse
\begin{theorem}\label{thm: reduction main}
	Suppose there exists an algorithm for the \recdynnc problem, that, 
	given a valid input structure $\iset=\left(H=(V,U,E),\set{\ell(e)}_{e\in E},D \right )$ undergoing a sequence of valid update operations with dynamic degree bound $\mu$, such that the number of regular vertices  in the intial graph $H$ is $N$, achieves approximation factor $\alpha(N\cdot \mu)$, has total update time $O(N^{1+\delta}\cdot \mu^{c})$, and ensures that, for every regular vertex $v$ of $H$, the total number of clusters in the neighborhood cover $\cset$ that the algorithm maintains, to which vertex $v$ ever belongs over the course of the algorithm is bounded by $\Delta(N)$; here, $\alpha(\cdot)\geq 2$, $\Delta(\cdot )\geq 2$ are non-decreasing functions, and $\delta,c>0$ are arbitrary parameters.
	Then there is a deterministic algorithm for fully-dynamic \APSP, that, given an instance $G$ of the problem and a precision parameter $\frac{1}{(\log m)^{1/8}}<\eps<1/100$, where $m$ is the total number of edges and vertices ever present in $G$, such that, for all $x>0$, $\Delta(x)\leq x^{\eps^2}$ holds, achieves approximation factor $\alpha'=(\alpha(m^2))^{O(1/\eps)}$, and has total update time at most $O\left (m^{1+O(\delta)+O(\eps)}\cdot (\Delta(m^2)\cdot \log m)^{O(c/\eps)}\cdot \log L\right )$, where $L$ is the ratio of longest to shortest edge length. Query time for \distquery is $O\left (2^{O(1/\eps)}\cdot \log m\cdot \log L\right )$ and query time for \pathquery is  $O\left (|E(P)|+2^{O(1/\eps)}\cdot \log m\cdot \log L\right )$, where $P$ is the path that the algorithm returns.
\end{theorem}
\fi





\subsubsection{New Algorithm for \recdynnc and Fully Dynamic \APSP}
Our next result is an improved algorithm for the \recdynnc problem, that is summarized in the following theorem.

\begin{theorem}\label{thm: main final dynamic NC algorithm}
	There is a deterministic algorithm for the \recdynNC problem, that,  given a valid input structure $\iset=\left(H=(V,U,E),\set{\ell(e)}_{e\in E},D \right )$ undergoing a sequence of valid update operations, with dynamic degree bound $\mu$, together with parameters $\hat W$ and  $1/(\log \hat W)^{1/100}\leq \eps<1/400$,  such that, if we denote by $N$ the number of regular vertices in $H\attime[0]$, then $N\cdot \mu\leq  \hat W$ holds, achieves approximation factor $\alpha=(\log\log \hat W)^{2^{O(1/\eps^2)}}$,  with total update time $O(N^{1+O(\eps)}\cdot \mu^{O(1/\eps)})$. Moreover, the algorithm ensures that, for every regular vertex $v\in V$, the total number of clusters in the weak neighborhood cover $\cset$ that the algorithm maintains, to which vertex $v$ ever belongs over the course of the algorithm, is bounded by $\hat W^{4\eps^3}$.
\end{theorem}



By combining \Cref{thm: main fully-dynamic APSP single scale} and  \Cref{thm: main final dynamic NC algorithm}, we immediately obtain the following corollary. We defer its proof to Section \ref{appx: proof main APSP} of Appendix.

\begin{corollary}\label{cor: fully APSP}
 There is a deterministic algorithm for fully-dynamic \APSP, that, given an $n$-vertex $G$ undergoing an online sequence of edge insertions and deletions, and a precision parameter $\frac{1}{(\log n)^{1/200}}<\eps<1/400$, achieves approximation factor $\alpha'=(\log\log n)^{2^{O(1/\eps^2)}}$, and has amortized update time at most $O\left (n^{O(\eps)}\cdot \log \Lambda\right )$ if starting from an empty graph, where $\Lambda$ is the ratio of longest to shortest edge length. Query time is $O\left (2^{O(1/\eps)}\cdot \log n\cdot \log\log \Lambda\right )$ for \distquery and  $O\left (|E(P)|+2^{O(1/\eps)}\cdot \log n\cdot \log\log \Lambda\right )$ for \pathquery, where $P$ is the path that the algorithm returns.
\end{corollary}





\subsection{Our Techniques}
We provide a brief overview of our techniques, starting with the proof of 
\Cref{thm: main fully-dynamic APSP single scale}.

{\bf Reduction from \recdynnc to $D^*$-restricted \APSP.} 
The description that we provide here is somewhat over-simplified, and is intended for intuition only.
We assume that we are given a fully dynamic graph $G$, that undergoes an online sequence $\Sigma$ of edge-insertions and deletions, such that $|E(G\attime[0])|+|V(G)|+|\Sigma|=m$, together with a distance parameter $D^*$, and a precision parameter $\eps$. At a high level, we use a rather natural approach. This high-level approach was used before in multiple reductions from fully-dynamic to decremental algorithms (see e.g. \cite{henzinger2001maintaining,HenzingerKing,abraham2014fully,ForsterG19,ForsterGH20}), but due to the specific setting of the problem that we consider, the use of this approach in our setting gives rise to a number of new technical challenges that we highlight below. We also provide a brief comparison with previous results where a similar approach was used.  Assume for simplicity that $q=1/\eps$ is an integer, and that so is $M=m^{\eps}$. Assume further that the distance parameter $D^*$ is an integral power of $2$. The data structures that we maintain are partitioned into $q+1$ \emph{levels}. We also define a hierarchical partition of the time horizon $\tset$ into phases.

For level $L=0$, there is a single level-$0$ phase, that spans the entire time horizon $\tset$. We maintain a level-$0$ graph $H^0$, that is constructed as follows. Let $G'$ be the dynamic graph that is obtained from the input graph $G$, by ignoring all edge insertions, and only executing edge-deletion updates. Graph $H^0$ is a bipartite graph, that has a regular vertex $v(x)$ for every vertex $x\in V(G)$, and a regular vertex $v(e)$ for every edge $e\in E(G')$. Additionally, it has a supernode $u(x)$ for every regular vertex $x\in V(G)$, that connects, with an edge of length $1$ to the corresponding regular vertex $v(x)$. For every edge $e=(x,y)\in E(G')$, we also connect $v(e)$ to $u(x)$ and $u(y)$, with edges of length $\ell(e)$. As graph $G'$ undergoes edge-deletions, the corresponding bipartite graph $H^0$ undergoes edge-deletions as well. For every integer $0\leq i\leq \log D^*$, we can view graph $H^0$ as an instance of the \recdynnc problem, with distance bound $D_i=2^i$. We apply the algorithm for the \recdynnc problem from \Cref{assumption: alg for recdynnc2} to this instance, and we denote by $\cset^0_i$ the resulting collection of clusters that it maintains. For every cluster $C\in \cset^0_i$, we say that the \emph{scale} of $C$ is $i$, and we denote $\scale(C)=i$. Let $\cset^0=\bigcup_{i=0}^{\log D^*}$ be the collection of all level-$0$ clusters.

Consider now some level $0<L\leq q$. We partition the time horizon $\tset$ into at most $M^{L}$ \emph{level-$L$ phases}. Each level-$L$ phase $\Phi^L_k$ spans exactly $M^{q-L}$ consecutive edge-insertion updates from the update sequence $\Sigma$ for graph $G$, except for possibly the last phase that may contain fewer edge insertions. We can define this hierarchical partition of the time horizon into phases for different levels so that, for all $0<L\leq q$, every level-$L$ phase is contained in some level-$(L-1)$ phase.

Consider now some level $0<L\leq q$ and a level-$L$ phase $\Phi^L_k$. Let $\Phi^{(L-1)}_{k'}$ be the unique level-$(L-1)$ phase that contains $\Phi^L_k$. We associate, with phase $\Phi^L_k$, a collection $A^L_k$ of edges of $G$, that the level-$L$ data structure will be ``responsible'' for during phase $\Phi^L_k$. These are all the edges that were inserted into $G$ since the beginning of level-$(L-1)$ phase $\Phi^{(L-1)}_{k'}$, but before the beginning of level-$L$ phase $\Phi^L_k$. It is easy that the number of such edges must be bounded by $M^{q-L+1}$. We also denote by $S^L_k$ the collection of vertices of $G$ that serve as endpoints of the edges of $A^L_k$.

We are now guaranteed that, at all times $\tau\in \tset$, for every edge $e\in E(G)$, either $e\in E(G\attime[0])$ (in which we say that it lies at level $0$); or there is some level $0<L\leq q$, such that $e\in A^L_k$ currently holds, where $k$ is the index of the current level-$L$ phase (in which case we say that the level of $e$ is $L$). For every path $P$ in graph $G$, we also define the \emph{level} of path $P$ to be the largest level of any of its edges.

Consider now some level $0<L\leq q$, and recall that there are at most $M^L$ level-$L$ phases. At the beginning of every level-$L$ phase, we construct level-$L$ data structures from scratch. These data structures consist of a dynamic level-$L$ bipartite graph $H^L$, that is viewed as an input to the \recdynnc problem. The set of regular vertices of $H^L$ is $S^L_k$, where $k$ is the index of the current level-$L$ phase. Intuitively, graph $H^L$ will be ``responsible'' for all level-$L$ paths in graph $G$. We describe the sets of supernodes and of edges of $H^L$ below. For all $0\leq i\leq \log D^*$, we view graph $H^L$, together with distance parameter $D_i=2^i$, as an instance of the \recdynnc problem, and we apply the algorithm from \Cref{assumption: alg for recdynnc2} to this instance, denoting the resulting collection of clusters by $\cset^L_i$. We say that all clusters in $\cset^L_i$ have scale $i$, and we denote  $\cset^L=\bigcup_{i=0}^{D^*}\cset^L_i$. The supernodes of graph $H^L$ are vertices $u(C)$ corresponding to some of the clusters  $C\in\bigcup_{L'<L}\cset^{L'}$. As the clusters in set $\bigcup_{L'<L}\cset^{L'}$ evolve, we maintain the corresponding dynamic graph $H^L$ via valid update operations, where, for example, a cluster-splitting update of a cluster $C\in\bigcup_{L'<L}\cset^{L'}$  can be implemented via a supernode-splitting update applied to supernode $u(C)$.

 Notice that, while the number of level-$L$ phase may be as large as $M^L$, the number of regular vertices in the level-$L$ graph $H^L$ is bounded by $2M^{q-L+1}$. Therefore, even though we need to recompute a level-$L$ data structure from scratch at the beginning of each level-$L$ phase, the size of the corresponding graph is sufficiently small that we can afford it. The level-$q$ data structure is computed from scratch after every edge-insertion update, though the number of regular vertices in the corresponding graph $H^q$ is bounded by $M\leq m^{\eps}$.
 
 While the high-level idea described above is quite natural, and was used multiple times in the past (see e.g. \cite{henzinger2001maintaining,HenzingerKing,abraham2014fully,ForsterG19,ForsterGH20}), it poses a number of challenges. The main challenge is the coordination between the different levels that is needed in order to support \shortpath\ queries. Consider, for example, a \shortpath\ query between a pair $x,y$ of vertices of $G$, and assume that there is a path $P$ in $G$ connecting $x$ to $y$, whose length is $D<D^*$. Notice, however, that the edges of $P$ may belong to different levels, and there may not be a single level $L$, such that all vertices of $P$ lie in the graph $H^L$. Assume that the level of path $P$ is $L$. Then we would like the level-$L$ data structure to be ``responsible'' for this query. In other words, we would like some path $P'$, whose length is comparable to $D$, to represent path $P$ in graph $H^L$. But it is possible that the endpoints $x$ and $y$ of $P$ do not even lie in graph $H^L$, so it is not clear which path in $H^L$ we should use as a representative of path $P$.
 

This issue seems especially challenging in the setting of the \APSP with adaptive adversary setting, where it is required that approximate \spquery are supported. For comparison, \cite{abraham2014fully}
and \cite{ForsterGH20} use a very similar high-level idea of a hierarchical partition of the time horizon and the set of edges. In \cite{ForsterGH20}, the algorithm is only required to maintain a low-stretch probabilistic tree embedding of the graph. This allows them to combine the trees maintained at different levels into a single tree that has a relatively low height, thereby circumventing the problem of coordinating between graphs from different levels. In order to respond to \distquery between a pair of vertices, they simply compute the length of the path between the two vertices in the tree that they maintain. Their data structure however cannot support approximate \shortestpathquery. If we tried to similarly combine graphs from different levels in order to overcome the challenge of coordinating between different levels, we would obtain another fully dynamic (non-tree) graph, and it is not clear how to support approximate \shortestpathquery in this graph. A different approach was taken by \cite{abraham2014fully}, whose algorithm exploits specific properties of the distance oracles of \cite{TZ,rodittyZ2}. The latter constructions however are randomized and can only withstand an oblivious adversary.
 
 
 In order to resolve this issue of coordination between levels, we associate, to every cluster $C\in \bigcup_{L=0}^q\cset^L$, a set $V^F(C)\subseteq V(G)$ of vertices, and we think of cluster $C$ as representing this collection of vertices of $G$. For a level $0\le L\leq q$, we include in graph $H^L$ supernodes $u(C)$ for all clusters $C\in \bigcup_{L'<L}\cset^{L'}$ with $S^L_k\cap V^F(C)\neq \emptyset$, where $k$ is the index of the current level-$L$ phase. For every vertex $x\in S^L_k$, and supernode $u(C)$ with $x\in V^F(C)$, we add an edge $(v(x),u(C))$ to graph $H^L$, whose length is $2^{\scale(C)}$. The main challenge in this construction is to define the sets $V^F(C)$ of vertices for clusters $C\in \bigcup_{L=0}^q\cset^L$. On the one hand, we would like to make these sets broad enough, so that the resulting graphs $H^L$ are rich enough in order to allow us to support approximate \shortpath\ queries. On the other hand, in order to ensure that the algorithm is efficient, these sets cannot be too large.
 
 In order to support \shortpath\ queries between pairs of vertices $x,y\in V(G)$, we employ a notion of ``covering chains'' -- structures that span multiple levels. Suppose the shortest path $P$ connecting $x$ to $y$ in $G$ has length $D\leq D^*$, and belongs to level $L$. Using the covering chains, we compute small collections $R(x),R(y)\subseteq S^L_k$ of vertices associated with $x$ and $y$ respectively, such that there exists a vertex $x'\in R(x)$ and a vertex $y'\in R(y)$, together with a path $P'$ in graph $H^L$ connecting $v(x')$ to $v(y')$, whose length is comparable to $D$. Conversely, we show that any such path can be transformed into a path in graph $G$ that connects $x$ to $y$, and has length that is not much larger than $D$.
 
 
 Next, we provide a high-level overview of the proof of \Cref{thm: main final dynamic NC algorithm}. We also  point out the main remaining bottlenecks to obtaining a better approximation.
 
 {\bf Improved algorithm for \recdynnc.}
  The \recdynnc problem can be effectively partitioned into two subproblems. The first subproblem, called \maintaincluster problem, is responsible for maintaining a single cluster. Suppose we are given any such cluster $C\subseteq H$, where $H$ is the current graph, and a distance parameter $D^*>D$. Cluster $C$ will undergo a sequence $\Sigma_C$ of valid update operations that correspond to the updates applied to $H$, possibly with some additional edge-deletions and isolated vertex-deletions. The goal of the \maintaincluster problem is to support \spquery queries: given a pair $x,y$ of regular vertices of $C$, compute a path $P$ of length at most $\alpha\cdot D^*$ connecting them in graph $C$, in time $\tilde O(|E(P)|)$, where $\alpha$ is the approximation factor that the algorithm achieves. Whenever the diameter of cluster $C$ becomes too large, the algorithm may raise a flag $F_C$, and to provide a pair $x,y$ of regular vertices of $C$ (that we call a \emph{witness pair}), such that $\dist_C(x,y)> D^*$. After that, the algorithm will receive, as part of the update sequence $\Sigma_C$, a sequence of edge-deletions and isolated vertex-deletions (that we call a \emph{flag-lowering sequence}), following which at least one of the vertices $x,y$ is deleted from $C$, and flag $F_C$ is lowered. If the diameter of $C$ remains too large, the algorithm can raise the flag again immediately. Queries $\spquery$ may not be asked when flag $F_C$ is up. \maintaincluster problem was defined in \cite{APSP-previous}, and we employ the same definition here.
 
 The second problem is \maintainNC problem. This problem is responsible for managing the neighborhood cover $\cset$ itself. Initially, we start with $\cset$ containing a single cluster - cluster $H$. The clusters in $\cset$ may only undergo allowed operations that are defined exactly like in the \recdynnc problem. The algorithm also needs to maintain, for every regular vertex $v\in V(H)$, a cluster $\coveringcluster(v)\in \cset$, that contains all vertices of $B_H(v,D)$, so that the Consistent Covering property holds. The algorithm does not need to support any queries. But, at any time, it may receive a cluster $C$ and a pair $x,y$ of vertices of $C$, such that $\dist_C(x,y)>D^*$ holds (for a parameter $D^*$ that we specify below). It must then produce a flag-lowering sequence $\Sigma'$ for $C$ (that is, a sequence of edge- and isolated vertex-deletions, after which at least one of $x,y$ is deleted from $C$). All updates from $\Sigma'$ must be then applied to cluster $C$, but they may be interspersed with cluster-splitting operations, when new clusters $C'\subseteq C$ are added to $\cset$. The algorithm must also ensure that every regular vertex of $H$ only belongs to a small number of clusters over the course of the time horizon.
 
 By combining the algorithms for \maintaincluster and \maintainNC problems, it is easy to obtain an algorithm for \recdynnc, whose approximation factor is $\alpha \cdot D^*/D$, where $\alpha$ is the approximation factor of the algorithm for the \maintaincluster problem, and $D^*$ is the threshold parameter for raising the flags $\set{F_C}_{C\in \cset}$.
 
 
 
  While \cite{APSP-previous} did not explicitly define the \maintainNC problem, they effectively provided a simple algorithm for it, that relies on a variation of the standard ball-growing technique, and uses parameter $D^*=\Omega(D\cdot \log N)$, where $N$ is the number of regular vertices in graph $H$. This overhead of $O(\log N)$ factor is one of the reasons for the $(\log N)^{2^{O(1/\eps)}}$-approximation factor that their algorithm achieves, and it is one of the barriers to obtaining a better approximation. We provide a different algorithm for the  \maintainNC problem, that allows us to set $D^*=O(D\cdot \log \log N)$. The overhead of factor  $O(\log\log N)$ in this algorithm is the only remaining barrier to obtaining an improved algorithm for the \recdynnc problem, and for \APSP. For example, if we could ensure that $D^*=O\left (2^{2^{O(1/\poly(\eps))}}\cdot D\right )$ is sufficient, we would obtain an algorithm for \recdynnc and for fully dynamic \APSP with approximation factor $2^{2^{O(1/\poly(\eps))}}$ and the same update time immediately.
  
 
In the remainder of this overview, we focus on the \maintaincluster problem. We first provide a brief overview of the algorithm from \cite{APSP-previous}, and then describe our improvements.

The central concept that \cite{APSP-previous} use in designing an algorithm for the \maintaincluster problem is that of a \emph{balanced pseudocut}, which they also introduced. Let $N$ be the number of regular vertices in $H\attime[0]$, and let $\mu$ be the dynamic degree bound. Recall that, as input to the \maintaincluster problem, we are given a cluster $C$ of $H$, that undergoes a sequence $\Sigma_C$ of valid update operations with dynamic degree bound $\mu$, and a distance parameter $D^*>D$. We use an additional parameter $\rho$; it may be convenient to think of $\rho=N^{\eps}$. Let $\hat D>D^*$ be another distance parameter; its specific value is not important for this technical overview, but it is close to $D^*$. A $(\hat D,\rho)$-pseudocut in graph $C$ is a collection $T$ of regular vertices of $C$, such that, for every regular vertex $v\in V(C)\setminus T$, $B_{C\setminus T}(v,\hat D)$ contains at most $N/\rho$ regular vertices. This notion can be viewed as a generalization of the balanced vertex multicut, that can be defined as a collection $T$ of vertices, such that every connected component of $C\setminus T$ contains at most $N/\rho$ vertices. Intuitively, once the vertices of the pseudocut (or of a balanced multicut) are deleted from $C$, we can break it into significantly smaller clusters, while still maintaining the covering properties of the neighborhood cover $\cset$. However, balanced pseudocuts have one additional crucial property: \cite{APSP-previous} provided an algorithm, that, given a $(\hat D,\rho)$-pseudocut $T$ in cluster $C$, either (i) computes an expander graph $X$, with $V(X)\subseteq T$, such that $|V(X)|$ is comparable to $|T|$, together with an embedding of $X$ into $C$ via short paths that cause a relatively low congestion; or (ii) computes another $(\hat D,\rho)$-pseudocut $T'$ in $C$, with $|T'|\ll |T|$. We denote this algorithm $\alg$. This algorithm is the core technical part in the algorithm of \cite{APSP-previous} for the \maintaincluster problem, and our main technical contribution to the \maintaincluster problem essentially replaces algorithm $\alg$ with a different algorithm. We now provide a very brief description of algorithm $\alg$. 

{\bf Algorithm $\alg$.}
A central observation that is needed for the algorithm is the following: let $T$ be a $(\hat D,\rho)$-pseudocut in graph $C$, and suppose we have computed a relatively small subset $E'$ of edges of $C$, and a collection $T_1,T_2,\ldots,T_{\rho+1}$ of subsets of vertices of $T$, such that each such subset $T_i$ is sufficiently large, and, for all $1\leq i<j\leq \rho+1$, $\dist_{C\setminus E'}(T_i,T_j)>4\hat D$. Then we can compute a pseudocut $T'$ for graph $C$ with $|T'|\ll|T|$. The idea is that there must be some index $1\leq i\leq \rho+1$, such that $B_{C\setminus E'}(T_i,2\hat D)$ contains at most $N/\rho$ regular vertices. By replacing set $T_i$ in the pseudocut $T$ with the endpoints of the edges in $E'$, we obtain a significantly smaller pseudocut $T'$. Algorithm $\alg$ starts with the given pseudocut $T$, and then attempts to compute an expander $X$ over a large subset of vertices of $T$, and to embed it into $C$ via the Cut-Matching Game of \cite{KRV} (in fact, they need to use a weaker variant of the game from \cite{detbalanced}, who provide a deterministic algorithm for the cut player, but unfortunately only ensure a rather weak expansion in the resulting graph $X$, which also contributes to the relatively high approximation factor of \cite{APSP-previous}).
If the Cut-Matching Game fails to construct the expander $X$ and embed it into $C$ as required, then it produces two large subsets $T',T''\subseteq T$ of vertices, and a relatively small subset $E'$ of edges, such that $\dist_{C\setminus E'}(T',T'')>4\hat D$. Then they recursively apply the same algorithm to $T'$ and to $T''$. After $\rho$ such iterations, if the algorithm failed to construct the desired expander $X$ and its embedding, we  obtain large vertex subsets $T_1,\ldots,T_{\rho+1}\subseteq T$, and a subset $E'$ of edges of $C$, that allow us to compute a much smaller pseudocut, as described above. Even though they perform $\rho$ iterations of the algorithm for the Cut-Matching Game, since, in case of a failure, the subsets $T',T''\subseteq T$ of vertices that it produces are very large compared to $|T|$, the resulting subsets $T_1,\ldots,T_{\rho+1}$ of vertices are still sufficiently large to make progress.
We now complete the description of the algorithm of \cite{APSP-previous} for the \maintaincluster problem.

The algorithm is partitioned into phases. Initially, we construct a pseudocut $T$ that contains all regular vertices of $C$. At the beginning of each phase, we use Algorithm $\alg$ (possibly iteratively), in order to compute a pseudocut $T'$, and an expander $X$ defined over a large subset of vertices of $T'$, together with an embedding of $X$ into $C$ via short path that cause a low congestion. Assume first that $|T'|>N^{1-\Theta(\eps)}$. The algorithm of \cite{APSP-previous} employs an algorithm for \APSP in expanders on graph $X$. This algorithm can maintain a large ``core'' $S\subseteq V(X)$, over the course of a large number of edge-deletions from $C$ (the  number that is roughly comparable to $|T'|$). It can also support queries in which, given a pair $x,y\in V(S)$ of vertices, a path of length at most roughly $(\log N)^{O(1/\poly(\eps))}$ connecting $x$ to $y$ in $X$ is returned. This path can then be transformed into a path of comparable length connecting $x$ to $y$ in $C$, using the embedding of $X$ into $C$. Additionally, they maintain an \EST in graph $C$, that is rooted at the vertices of $S$. This tree can be used in order to ensure that all regular vertices of $C$ are sufficiently close to the core $S$, and, whenever this is not the case, flag $F_C$ is raised. Once the algorithm for \APSP in expanders can no longer maintain the core $S$ (after roughly $|T'|$ deletions of edges from $C$), the phase terminates. It is easy to verify that, as long as the cardinality of the pseudocut $T'$ is sufficiently large (say at least $N^{1-\Theta(\eps)}$), the number of phases remains relatively small, and the algorithm can be executed efficiently. Once the cardinality of the pseudocut $T'$ becomes too small, the last phase begins, during which the pseudocut $T'$ remains unchanged. We omit here the description of this phase, since our implementation of this part is essentially identical to that of \cite{APSP-previous}. We only note that this phase solves the \recdynnc problem recursively on two instances, whose sizes are significantly smaller than that of $H$. The two instances are then composed in a natural way, which eventually leads to the doubly-exponential dependence of the approximation factor on $1/\poly(\eps)$.

The algorithm of \cite{APSP-previous} for the \maintaincluster problem loses a super-logarithmic in $N$ approximation factor via this approach, that contributes to the  final $(\log N)^{2^{1/\poly(\eps)}}$-approximation factor for the \recdynnc problem. This loss is largely  due to the use of expander graphs. In addition to the issues that we have mentioned with the implementation of the Cut-Matching game via a deterministic algorithm, all currently known algorithms for \APSP in expanders only achieve a superlogarithmic approximation factor, and even if they are improved, the loss of at least a polylogarithmic approximation factor seems inevitable. It is typical for this issue to arise when relying on expander graphs for distance-based problems, such as \APSP. A recent work of \cite{DMG} suggested a method to overcome this difficulty, by replacing expander graphs with \emph{well-connected} graphs. Intuitively, if $G$ is a graph, and $S$ is large subset of its vertices, we say that $G$ is well-connected with respect to $S$ (or just well-connected) if, for every pair $A,B\subseteq S$ of disjoint equal-cardinality subsets of vertices of $S$, there is a collection $\pset$ of paths in $G$, that connects every vertex of $A$ to a distinct vertex of $B$, such that the paths in $\pset$ are short, and they cause a low congestion. In a typical setting, if $G$ is an $n$-vertex graph, then the lengths of the paths in $\pset$ are bounded by $2^{\poly(1/\eps)}$, and the congestion that they cause is bounded by $n^{O(\eps)}$. \cite{DMG} also developed a toolkit of algorithmic techniques around well-connected graphs, that mirror those known for expanders. For example, they provide an analogue of the Cut-Matching Game, that, given a graph $C$ and a set $T$ of its vertices, either computes a large set $S\subseteq T$ of vertices, and a graph $X$ with $V(X)\subseteq T$, that is well-connected with respect to $S$, together with an embedding of $X$ into $C$ via short paths that cause a low congestion; or it computes two relatively large sets $T',T''\subseteq T$ of vertices, and a small set $E'$ of edges, such  that $\dist_{C\setminus E'}(T',T'')$ is large. Additionally, they provide an algorithm for \APSP in well-connected graphs, that has similar properties to the above mentioned algorithm for \APSP in expanders, but achieves a much better approximation factor of $2^{1/\poly(\eps)}$. By replacing expander graphs with well-connected graphs in the algorithm for \maintaincluster problem of \cite{APSP-previous}, we avoid the superlogarithmic loss in the approximation factor that their algorithm incurred. We note however that replacing expanders with well-connected graphs in algorithm $\alg$ is quite challenging technically, for the following reason. Recall that, in the approach that used the Cut-Matching Game, if the algorithm fails to compute an expander $X$ containing a large number of vertices from the given set $T$ and embed it into $C$, it provides two very large subsets $T',T''\subseteq T$ of vertices, together with a small set $E'$ of edges, such that $\dist_{C\setminus E'}(T',T'')>4\hat D$. Unfortunately, the analogous algorithm of \cite{DMG}, in case of a failure to embed a well-connected graph, provides vertex sets $T',T''$, whose cardinalities are significantly smaller than that of $T$. Specifically, it only ensures that $|T'|,|T''|\geq |T|^{1-4\eps^3}/4$. Since we need to continue applying this algorithm recursively, until $\rho+1$ subsets $T_1,\ldots,T_{\rho+1}$ of vertices of $T$ are constructed, we can no longer guarantee that, for all $i$, $|T_i|$ is sufficiently large. As a result, if our algorithm fails to compute a well-connected graph $X$ and its embedding into $C$, we can no longer compute a new pseudocut whose cardinality is significantly lower than that of $T$. Since the time required to execute this algorithm is super-linear in $|E(C)|$, we cannot afford to execute it many times, so it is critical for us that the cardinality of the pseudocut $T$ decreases significantly with every execution. Our main technical contribution to the algorithm for the \maintaincluster problem is overcoming this hurdle, and designing an analogue of Algorithm $\alg$ that works with well-connected graphs instead of expanders.

\paragraph{Organization.}
We start with preliminaries in \Cref{sec: prelims}. In \Cref{sec: valid inputs}, we formally define valid input structure, valid update operations, and the \recdynnc problem. We also provide the statement our main technical result for the \recdynnc problem -- an algorithm whose guarantees are somewhat weaker than those in \Cref{thm: main final dynamic NC algorithm}, which however allows us to prove \Cref{thm: main final dynamic NC algorithm}. \Cref{sec: fully APSP inner main}  is dedicated to the reduction from \recdynnc to fully dynamic \APSP and the proof of \Cref{thm: main fully-dynamic APSP single scale}.
In \Cref{sec: proof of recdynnc inner} we formally define the \maintainNC and \maintaincluster problems, and state our main results for them. We also complete our algorithm for the \recdynnc problem using these results. We provide our algorithms for the \maintainNC and the \maintaincluster problems in \Cref{sec: alg for maintainNC} and \Cref{sec: balanced pseudocut}, respectively.

==> arxiv-version-final/level-1-DS.tex <==
\newpage

\subsection{Level-$1$ Data Structure}
\label{subsec: level 1}

Recall that we partition the timeline into $M$ level-$1$ phases, each one of which consists of $M^{q-1}$ update operations from the input update sequence $\Sigma$. For all $1\leq k\leq M$, we denote by $\Phi^1_k$ the $k$th level-$1$ phase, and by $E^1_k$ the collection of edges that were inserted into graph $G$ via the update sequence $\Sigma$ over the course of Phase $\Phi^1_k$. 


At the beginning of every level-$1$ phase, we recompute the level-$1$ data structure from scratch. The level-$1$ data structure consists of a valid input 
structure $\iset^1=\left(H^1=(V^1,U^1,\tilde E^1),\set{\ell(e)}_{e\in E^1},D^1 \right )$, that undergoes a sequence of valid update operations, over the course of a single level-$1$ phase, where $D^1=16D^*$. Additionally, for $1\leq i\leq \log D^1$, we maintain data structure $\DS^1_i$, that, intuitively solves the \recdynnc problem on $\iset^1$ for distance parameter $D_i$. We will denote by $\cset^1_i$ the collection of clusters that data structure $\DS^1_i$ maintains.
We now define the data structures more formally.

Consider some level-$1$ phase $\Phi^1_k$, for $1\leq k\leq M$. If $k=1$ (so the current level-$1$ phase is the first one), then we let the graph $H^1$ be an empty graph throughout Phase $\Phi^1_k$, and for  all $1\leq i\leq \log D^1$ the data structure $DS^1_i$ is also empty, and $\cset^1_i=\emptyset$ throughout the phase.

From now on we describe the level-$1$ data structure that is maintained over the course of a level-$1$ phase $\Phi^1_k$, where $1<k\leq M$. We start with the initialization of the data structure, and then describe the updates to it. We then analyze the total update time of the data structure, and provide an algorithm that supports approximate short-path queries in $G$, in some limited cases.



\paragraph{Initialization.}
We start by initializing the graph $H^1=(V^1,U^1,\tilde E^1)$. 
Let $A^1_k=\bigcup_{k'=1}^{k-1}E^1_{k'}$ be the set of all edges that were inserted into $G$ prior to the beginning of Phase $\Phi^1_k$, and let $S^1_k$ be  the set of all vertices of $G$ that serve as endpoints of the edges of $A^1_k$.
Intuitively, throghout Phase $\Phi^1_k$, the level-$1$ data structure is responsible for keeping track of the edges of $A^1_k$.

 At the beginning of the algorithm, we store, together with every vertex $x\in S^1_k$, bi-directional pointers to all edges $e\in A^1_k$ such that $x$ is an endpoint of $e$.

The set $V^1$ of regular vertices of $H^1$ is the union of two subsets: 
set $\set{v^1(x)\mid x\in S^1_k}$ of regular vertices that represent the vertices of $S^1_k$, and 
set $\set{v^1(e)\mid e\in A^1_k}$ of regular vertices that represent the edges of $A^1_k$. 
We refer to the vertices of the former set as \emph{type-1 regular vertices}, and the vertices of the latter  set as \emph{type-2 regular vertices}.


Next, we define the supernodes of $H^1$. Intuitively, the supernodes will correspond to some clusters of $\cset^0$. Specifically, consider any cluster $C\in \cset^0$, and assume that there is some vertex $x\in S^1_k$, such that the corresponding regular vertex $v^0(x)$ of $H^0$ lies in $C$. Then we say that cluster $C$ is \emph{active} at the beginning of Phase $\Phi^1_k$. The set $U^1$ of supernodes of $H^1$ contains a supernode $u^1(C)$ for every cluster $C\in \cset^0$ that is active at the beginning of $\Phi^1_k$. If a cluster $C\in \cset^0$ is active at the beginning of Phase $\Phi^1_k$, then we select an arbitrary vertex $x\in S^1_k$, with $v^0(x)\in V(C)$, and designate vertex $x$ as the \emph{level-$1$ representative of cluster $C$}, denoting $\rep^1(C)=x$.


Lastly, we define the initial set $\tilde E^1$ of edges of $H^1$.
Consider some supernode $u^1(C)\in U^1$, and assume that $C\in \cset^0_i$, for some $1\leq i\leq \log D^0$. For every vertex $x\in S^1_k$ with  $v^0(x)\in V(C)$, we add an edge $(v^1(x),u^1(C))$ to $\tilde E^1$. The length of the edge is $D_i$, and the edge is referred to as a \emph{type-1 edge}. 

Consider now some edge $e=(x,y)\in A^1_k$. For every cluster $C\in \cset^0$ with $v^0(x)\in V(C)$, we add a \emph{type-2 edge} $e'=(v^1(e),u^1(C))$, whose length is $\ell(e)+D_i$,  to set $\tilde E^1$, where $i$ is the index for which $C\in \cset^0_i$. We say that vertex $x$ is \emph{responsible} for edge $e'$, and we store this information together with edge $e'$. Similarly, for every cluster $C\in \cset^0$ with $v^0(y)\in V(C)$, we add a type-2 edge $e''=(v^1(e),u^1(C))$ to set $\tilde E^1$, whose length is $\ell(e)+D_i$, where $i$ is the index for which $C\in \cset^0_i$, and we say that vertex $y$ is responsible for edge $e''$, storing this information together with edge $e''$. If both $v^0(x),v^0(y)\in V(C)$, then we add a single edge $(v^1(e),v^1(C))$ of length $\ell(e)+D_i$, where $i$ is the index for which $C\in \cset^0_i$, and we designate both $x$ and $y$ as being responsible for this edge.

This completes the definition of the initial graph $H^1$. Note that the graph can be constructed in time at most $O(|A^1_k|\cdot \Delta(W)\cdot \log W)$. Indeed, once we construct the set $V^1$ of regular vertices, we can compute, for every vertex $x\in S^1_k$, all clusters $C\in \cset^0$ that contain vertex $v^0(x)$ via the lists $\clusterlist^0_i(v^0(x))$ that data structures $\DS^0_i$ maintain, for $1\leq i\leq \log D^0$. Since, as observed already, every regular vertex of $H^0$ may belong to at most $O(\Delta(W)\cdot \log W)$ clusters of $\cset^0$, the bound follows.


Recall that we have defined $D^1=16D^*$. For all $1\leq i\leq \log D^1$, we define a graph $H^1_i$, that is identical to $H^1$, except that it does not include edges whose length is greater than $D_i$. For all $1\leq i\leq \log D^1$, we have now defined  a valid input structure  $\iset^1_i=\left(H^1_i,\set{\ell(e)}_{e\in \tilde E(H^1_i)},D_i \right )$, that we view as an input to the \recdynnc problem. We will define below a sequence of valid update operations for $\iset^1_i$, based on the sequence $\Sigma$ of updates of graph $G$, over the course of Phase $\Phi^1_k$.  We initialize the data structure for the \recdynnc problem on input $\iset^1_i$, that will be maintained by Algorithm $\aset$, which is assumed to exist in the statement of \Cref{thm: main fully-dynamic APSP single scale}. We denote the corresponding data structure by $\DS^1_i$, and the corresponding collection of clusters that it maintains by $\cset^1_i$. We also denote by $\cset^1=\bigcup_{i=1}^{\log D^1}\cset^1_i$, and we denote by $\DS^1$ all data structures $\DS^1_i$, for $1\leq i\leq \log D^1$.
 
 For convenience, for all $1\leq i\leq \log D^1$, for every regular vertex $v\in V(H^1)$, we denote the cluster $\coveringcluster(v)$ that data structure $\DS^1_i$ maintains by  $\coveringcluster^1_i(v)$. Similarly, we denote the list $\clusterlist(v)$ of all clusters of $\cset^1_i$ containing $v$ that data structure $\DS^1_i$ maintains by $\clusterlist^1_i(v)$. We then let $\clusterlist^1(v)=\bigcup_{i=1}^{\log D^1}\clusterlist^1_i(v)$.
 Lastly, if $C$ is a cluster that currently lies in $\cset^1_i$, for some $1\leq i\leq \log D^1$, and $v,v'$ are two regular vertices of $H^1$ that currently lie in $C$, we denote by $\shortpath^1_i(C,v,v')$ a query $\shortpath(C,v,v')$ to data structure $\DS^1_i$. Recall that the data structure must return a path $P$ of length at most $\alpha(W)\cdot D_1$ connecting $v$ to $v'$ in $H^1_i$, in time $O(|E(P)|)$. Note that $P\subseteq H^1$ must hold. For convenience, we will think of $\shortpath^1_i(C,v,v')$ as a query that is supported by data structure $\DS^1$.



This completes the initialization of the level-$1$ data structure. Next, we define update sequences for valid input structures $\iset^1_i$, for $1\leq i\leq \log D^1$.


\paragraph{Updates.}
We start by defining the input update sequence for valid input structure $\iset^1$. For all $1\leq i\leq \log D^1$, we will then naturally obtain a corresponding update sequence for $\iset^1_i$, by ignoring all edges whose length is greater than $D_i$.

We denote by $\Sigma^1_k\subseteq \Sigma$ the sequence of update operations to graph $G$ that occur over the course of Phase $\Phi^1_k$, where we ignore edge insertions, so $\Sigma^1_k$ only contains edge deletions. For every edge $e\in \Sigma^1_k$ that is deleted from $G$, we will generate a sequence $\hat \Sigma(e)$ of valid update operations to $\iset^1$.
We will ensure that the following invariants always hold throughout the algorithm:

\begin{properties}{I}
	\item If $C$ is a cluster of $\cset^0$, then, at any time in the algorithm's execution, $C$ is active for level $1$ if and only if there is some vertex $x\in S^1_k$ with $v^0(x)\in V(C)$. If $C$ is active for level $1$, then supernode $u^1(C)$ belongs to graph $H^1$, and it is not an isolated vertex in $H^1$. Moreover, some vertex $a\in S^1_k$ with $v^0(a)\in V(C)$ must be assigned as a level-$1$ representative of $C$, so $\rep^1(C)=a$.
	\label{inv: level 1 active clusters}
	
	\item For every vertex $x\in S^1_k$, for every cluster $C\in \cset^0$ that is active for level $1$, edge $(v^1(x),u^1(C))$ is present in $H^1$ if and only if $v^0(x)\in V(C)$. If present, the length of the edge is $D_i$, where $i$ is the index for which $C\in \cset^0_i$. \label{inv: level 1 type 1 regular}
	
	
	\item For every edge $e\in A^1_k$, and cluster $C\in \cset^0$ that is active for level $1$, an edge   $(v^1(e),u^1(C))$ is present in the current graph $H^1$ if and only if (i) edge $e$ is currently present in $G$; and (ii) there is at least one endpoint $z$ of $e$ with $v^0(z)\in V(C)$. If $z$ is the only endpoint of $e$ with $v^0(z)\in V(C)$, then vertex $z$ is responsible for edge $(v^1(e),u^1(C))$, and otherwise, both endpoints of $e$ are responsible for this edge. The length of edge $(v^1(e),u^1(C))$ is $\ell(e)+D_i$, where $i$ is the index for which $C\in \cset^0_i$. \label{inv: level 1 type 2 regular}
\end{properties}

Note that, from the definition of the \recdynnc problem, once a cluster $C$ is added to set $\cset^0$, vertices may be deleted from $C$, but they cannot be added to $C$. Therefore, once $C$ becomes inactive for level $1$, it will remain so for the remainder of the phase.

It is easy to verify that the above invariants hold immediately after the initialization of graph $H^1$. Next, we consider an update operation in $\Sigma^1_k$, in which some edge $e$ is deleted from $G$. We assume that all invariants hold before the deletion of $e$. We provide an algorithm to compute a sequence $\hat \Sigma(e)$ of valid update operations to graph $H^1$, that will ensure that the invariants continue to hold in $H^1$, after $e$ is deleted from $G$, and the updates 
from $\hat \Sigma(e)$ have been processed.

 We consider three cases. First, if $e\in E^1_k$, that is, edge $e$ was inserted into $G$ during the current level-$1$ phase $\Phi^1_k$, then we then we set $\hat\Sigma(e)=\emptyset$.
Assume now that $e\in A^1_k$, that is, edge $e$ was inserted into $G$ during level-$1$ phases $\Phi^1_1,\ldots,\Phi^1_{k-1}$. In this case, we let $\hat \Sigma(e)$ be a sequence of deletions of edges from $H^1$, that includes all edges that are currently incident to vertex $v^1(e)$.

Lastly, assume that $e$ is an original edge of $G$. Note that in this case, vertex $v^0(e)$ is present in the level-$0$ graph $H^0$. We start by updating the level-$0$ data structures with the deletion of $e$ from $G$. As the result, some clusters of $\cset^0$ may undergo allowed changes. We now consider each such change one by one. For each such change, we may add some valid update operations to $\hat \Sigma(e)$.

Let $C\in \cset^0$ be any cluster that underwent a change as the result of the updates to level-0 data structure due to the deletion of $e$ from $G$. 
If the change is the insertion of a supernode into $C$, then we do nothing.


Assume now that the change is the deletion of a vertex from $C$. In this case, we only need to update sequence $\hat \Sigma(e)$, if $C$ is currently an active cluster for level $1$, the deleted vertex is a type-$1$ regular vertex $v^0(x)$ of $H^0$, and $x\in S^1_k$. In this case, we add to $\hat \Sigma(e)$ the following edge deletions from graph $H^1$. First, we delete the edge $(v^1(x),u^1(C))$. Additionally, for every edge $e=(x,y)\in A^1_k$ that has not yet been deleted from $G$, we consider the edge $e'
 =(v^1(e),u^1(C))$ that currently lies in $H^1$. If $x$ is the only endpoint of $e$ that is responsible for $e'$, then  we add the deletion of $e'$ from $H^1$ to $\hat \Sigma(e)$. Otherwise, we make the other endpoint of $e$ be the sole vertex responsible for $e'$, and we do not add any further updates to $\hat \Sigma(e)$.
 If $x$ was the representative of $C$ for level $1$, and there is another type-1 edge $(v^1(z),u^1(C))$ in $H^1$, then we select any such edge and make $z$ the new representative of cluster $C$, so $\rep^1(C)=z$. Otherwise, vertex $u^1(C)$ must now be an isolated vertex in $H^1$. Then cluster $C$ becomes inactive for level $1$, and its representative is undefined. 

% Assume now that $C\in \cset^0$ is a cluster, and that a vertex $z$ is deleted from $C$, via $\delvertex$ operation. 
%We only need to update sequence $\hat \Sigma(e)$ 
%if $C$ is an active level-$1$ cluster, and $z=v(x)$ for some vertex $x\in V(G)$ with $x\in S^1_k$. In this case, we update sequence $\hat \Sigma(e)$ with the deletion of the edge $(v(x),u^1(C))$ from graph $H^1$. Additionally, for every edge $e=(x,y)\in A^1_k$, if vertex $x$ is the only endpoint of the edge $e'=(v(e),u^1(C))$ of $H^1$ that is responsible for $e'$, then we update $\hat \Sigma(e)$ with the deletion of $e'$. Otherwise, we make vertex $y$ the only endpoint of $e'$ that is responsible for this edge, and we do not need to update $\hat \Sigma(e)$. 

% is marked as existing due to vertex $x$ only, we delete $e'$  from $H^1$, and update sequence $\hat \Sigma(e)$ accordingly. If edge $e'$ is marked as existing due to both $x$ and $y$, then we now mark it as existing due to vertex $y$ only. Finally, if $x$ was a level-$1$ representative of $C$, and there is some other vertex $x'\in S^1_k$ with $v(x')\in V(C)$, then we make any such vertex $x'$ a new level-$1$ representative of cluster $C$. If cluster $C$ no longer contains any type-1 regular vertex $v(x')$ with $x'\in S^1_k$, then $C$ becomes inactive for level $1$.


Lastly, we assume that the update operation is  $\csplit$: given a cluster $C\in \cset^0_i$, for some $1\leq i\leq \log D^0$ and a subset $S'\subseteq V(C)$ of its vertices, the data structure $\DS^0_i$ added a new cluster $C'$ to $\cset^0_i$, whose vertex set is $S'$. If cluster $C$ is inactive for level $1$, then no further updates are necessary. Assume now that cluster $C$ is active for level $1$. Let $Z$ be the set of all vertices $x\in S^1_k$, with $v^0(x)\in S'$. If $Z=\emptyset$, then no further updates to $\hat \Sigma(e)$ are necessary, so we assume that $Z\neq \emptyset$ holds. Note that, for each vertex $x\in Z$, $v^0(x)\in V(C)$ must also hold, and edge $(u^1(C),v^1(x))$ must be present in $H^1$. Let $\tilde E'\subseteq A^1_k$ be the set of all edges that still lie in $G$ and have at least one endpoint in $Z$. Notice that, for each such edge $e'$, edge $(v^1(e'),u^1(C))$ lies in $H^1$. We denote $E'=\set{(v^1(x),u^1(C))\mid x\in Z}\cup \set{(v^1(e),u^1(C))\mid e\in \tilde E'}$. We add to $\hat\Sigma(e)$ a supernode splitting operation, that is applied to supernode $u^1(C)$, with the set $E'$ of edges; the operation constructs a new supernode $u^1(C')$ that represents the newly added cluster $C'$. Cluster $C'$ becomes active for level $1$, and we designate an arbitrary vertex $x\in Z$ as its representative for level $1$. %We add the supernode splitting operation described above to $\hat\Sigma(e)$. 
For every edge $e'\in \tilde E'$, if exactly one endpoint of  $e'$ lies in $Z$, then that endpoint becomes responsible for the new edge $(v^1(e),u^1(C'))$; otherwise, both endpoints of $e'$ become responsible for this edge.

Once we process every change in the clusters of $\cset^0$ that was caused by the deletion of edge $e$ from $G$, we obtain the final sequence $\hat \Sigma(e)$ of valid update operations for graph $H^1$. It is immediate to verify that all invariants continue to hold after the updates in $\hat \Sigma(e)$ are applied to $H^1$.

If we denote by $\Sigma^1_k=(e_1,e_2,\ldots,e_r)$ the sequence of edge deletions in graph $G$ that occur during Phase $\Phi^1_k$, then we now obtain an online sequence $\hat \Sigma^1_k=\hat \Sigma(e_1)\circ \hat \Sigma(e_1)\circ\cdots\circ \hat \Sigma(e_k)$ of valid update operations to graph $H^1$. Moreover, the time that is needed in order to produce sequence $\hat \Sigma^1_k$ is subsumed by the time required to maintain data structure $\DS^0$, and by the time required to initialize graph $H^1$. 

We now establish the dynamic degree bound for $\iset^1$ and $\hat \Sigma_1^k$. Consider first a type-1 regular vertex $v^1(x)\in V^1$. Recall that, for a cluster $C\in \cset^0$, an edge $(v^1(x),u^1(C))$ may only be present in $H^1$ if $v^0(x)\in V(C)$. Recall that level-0 data structure guarantees that the total number of clusters of $\cset^0$ to which vertex $v^0(x)$ may belong over the course of the algorithm is bounded by $O(\Delta(W)\cdot \log W)$. Therefore, the number of edges that are ever present in $H^1$ and are incident to $v^1(x)$ is bounded by $O(\Delta(W)\cdot \log W)$. Consider now some type-2 regular vertex $v^1(e)\in V^1$, and assume that $e=(x,y)$. Let $C\in \cset^0$ be any cluster. Then edge $(v^1(e),u^1(C))$ may only be present in $H^1$ if either edge $(v^1(x),u^1(C))$ or edge $(v^1(y),u^1(C))$ belong to $H^1$. Therefore, the total number of edges of $H^1$ that can ever be incident to $v^1(e)$ over the course of the algorithm is also bounded by $O(\Delta(W)\cdot \log W)$, and the dynamic degree bound for $\iset^1$ and $\hat \Sigma^1_k$, that we denote by $\mu_1$, is bounded by $O(\Delta(W)\cdot \log W)$.

Consider now some index $1\leq i\leq \log D^1$, and recall that the initial graph $H^1_i$ is obtained from graph $H^1$ by deleting all edges whose length is greater than $D_i$. Online update sequence $\hat \Sigma^1_k$ for graph $H^1$ naturally defines an online update sequence $\Sigma^1_{k,i}$ for graph $H^1_i$, where we simply ignore all edges whose length is greater than $D_i$: such edges do not need to be deleted from $H^1$, and they may not be inserted via supernode splitting operations. Therefore, we now obtain a sequence of valid update operations for the valid update structure $\iset^1_i$. As the algorithm progresses, we update data structure $\DS^1_i$ with the updates from $\Sigma^1_{k,i}$. Note that, from the assumptions in the statement of \Cref{thm: main fully-dynamic APSP single scale}, every regular vertex of $H^1$ may belong to at most $\Delta(W)$ clusters of $\cset^1_i$ over the course of the algorithm. Since $D^1\leq O(W)$, we get that every regular vertex of $H^1$ may belong to at most $O(\Delta(W)\cdot \log W)$ clusters of $\cset^1$ over the course of the algorithm. 

This completes the description of the algorithm for initializing and maintaining level-$1$ data structures. We now describe our algorithm for supporting short-path queries in some limited cases.



\paragraph{Supporting Approximate Short-Path Queries.}
Let $x$ and $y$ be a pair of vertices in graph $G$. Our level-$0$ and level-$1$ data structures allow us to support approximate short-path queries between $x$ and $y$, provided that there exists a short path $P$ in graph $G$ connecting $x$ to $y$, such that every edge of $P$ is either an original edge of $G$, or it belongs to set $A^1_k$. Notice that, if every edge of $P$ is an original edge of $G$, then support for such queries is provided by the level-$0$ data structure. Therefore, we can assume that at least one edge of $P$ belongs to set $A^1_k$. Notice however that vertices $x$ and $y$ may not lie in set $S^1_k$, so we may not be able to query the level-$1$ data structures with these two vertices directly. Instead, we will define, for each distance scale $1\leq i\leq \log D^0$ ``proxy'' vertices $\sigma_i(x)$ and $\sigma_i(y)$ (which may be undefined for some distance scales), and we will then send a query between a pair of such proxy vertices to $\DS^1$.
We now define such proxy vertices.

Let $z\in V(G)$ be any vertex. 
For all $1\leq i\leq \log D^0$, we define a vertex $\sigma_i(z)\in V(G)$, as follows. Let $C_i=\coveringcluster^0_i(v(z))$ -- the cluster covering $z$ that is maintained by data structure $\DS^0_i$. If $C_i$ is an active level-$1$ cluster, then we set $\sigma_i(z)=\rep^1(C_i)$ -- the level-$1$ representative of $C_i$. Otherwise, $\sigma_i(z)$ is undefined. We do not maintain the proxy vertices $\sigma_i(z)$ explicitly, they are only computed as needed, in oder to respond to short-path queries.
We need the following immediate observation.
Clearly, given a vertex $z\in V(G)$ and a distance scale $1\leq i\leq \log D^0$, the corresponding proxy vertex $\sigma_i(z)$ can be computed in time $O(1)$.%
%
%We then set $R(z)=\set{\sigma_i(z)\mid 1\leq i\leq \log D^1}$. Clearly, $|R(z)|\leq \log D^0$, and it is possible that $R(z)=\emptyset$. Notice also that, as the algorithm progresses, set $R(z)$ of vertices may change (since, e.g., some clusters may become inactive, their representatives may change). We do not maintain the sets $R(z)$ of vertices over the course of the algorithm. Each such set is only computed as needed in order to respond to approximate short-path queries. We need the following immediate observation.

%\begin{observation}\label{obs: covering sets}
%	There is an algorithm that, at any time, given a vertex $z\in V(G)$, computes the current set $R(z)$ of vertices, in time $O(\log D^0)$.
%\end{observation}

The following observation will be crucial for supporting approximate short-path queries. 

\begin{observation}\label{obs: level-1 approx short path queries}
	Consider graph $G$ at any time during Phase $\Phi^1_k$, and let $x,y\in V(G)$ be a pair of vertices of $G$. Assume that the current graph $G$ contains a path $P$ connecting $x$ to $y$ of length at most $D_i$, where $1\leq i\leq \log D^0$, such that every edge of $P$ is either an original edge, or it belongs to $A^1_k$. Assume further that at least one edge of $P$ belongs to $A^1_k$. Then  there is a path $P'$ of length at most $32D_i$ in the current graph $H^1$, connecting vertices $v^1(x')$ to $v^1(y')$, where $x'=\sigma_{i+2}(x)$ and $y'=\sigma_{i+2}(y)$. In particular, both $\sigma_{i+2}(x)$ and $\sigma_{i+2}(y)$ are defined.
\end{observation}

\begin{proof}
Let $e_1,\ldots,e_r$ denote the edges of $P$ that belong to set $A^1_k$. For all $1\leq a\le r$, denote $e_a=(x_a,y_a)$, and assume that vertices $x,x_1,y_1,x_2,y_2,\ldots,x_r,y_r,y$ appear on path $P$ in this order. Let $Q_1,\ldots,Q_{r+1}$ be the collection of subpaths of $P$ that are obtained once the edges $e_1,\ldots,e_{r}$ are deleted from $P$, where for all $1\leq a\leq r$, path $Q_a$ contains vertex $x_a$ as its last endpoint, and path $Q_{r+1}$ connects $y_r$ to $y$. For all $1\leq a\leq r+1$, we denote by $L_a$ the length of path $P_a$ in $G$. Notice that it is possible that path $P_a$ consists of a single vertex $x_a$, in which case its length is $0$. 

Consider first some index $1<a\leq r$, and recall that $Q_a$ is a path of $G$ connecting vertex $y_{a-1}$ to vertex $x_{a}$. The length of the path is $L_a$, and it contains no edges of $A^1_k$. In other words, all edges on path $P_a$ are original edges of $G$. Notice that it is possible that $y_{a-1}=x_{a}$, and the path contains no edges. From \Cref{claim: responding to queries level-0}, there is a path $P'_a$ in graph $H^0$ connecting $v^0(y_{a-1})$ to $v^0(x_{a})$, whose length is at most $2L_a+2$. Let $i_a$ be the smallest integer for which $2L_a+2\leq D_{i_a}$ holds. Clearly, $D_{i_a}\leq 4L_a+4\leq 4D^*+4\leq D^0$.
\mynote{need to increase $D^0$ to $8D^*$, and then increase $D^1$ too}
 Consider now cluster $C_a=\coveringcluster^0_{i_a}(v^0(x_{a}))$ that is maintained by data structure $\DS^1_{i_a}$. Recall that cluster $C_a$ must contain all vertices of $H^1_{i_a}$, whose distance from $v^0(x_{a})$ in graph $H^1_{i_a}$ is at most $D_{i_a}$. In particular, it must contain vertex $v^0(y_a)$. From Invariant \ref{inv: level 1 active clusters}, cluster $C_a$ is currently active at level $1$, and so supernode $u^1(C_a)$ must lie in $H^1$. From Invariant \ref{inv: level 1 type 1 regular}, an edge connecting $v^1(x_{a})$ to $u^1(C_a)$, and an edge connecting $v^1(y_{a-1})$ to $u^1(C_a)$  are both present in graph $H^1$. Moreover, from Invariant \ref{inv: level 1 type 2 regular}, graph $H^1$ contains edges $(v^1(e_{a-1}),u^1(C_a))$ and $(v^1(e_{a}),u^1(C_a))$. The length of the former edge is $\ell(e_{a-1})+D_{i_a}\leq \ell(e_{a-1})+4L_a+4$, while the length of the latter edge is $\ell(e_{a})+D_{i_a}\leq \ell(e_{a})+4L_a+4$. Consider a sequence of vertices $(v^1(e_{a-1}),u^1(C_a),v^1(e_{a}))$ of $H^1$. From the above discussion, this sequence of vertices defines a path in $H^1$ that we denote by $Q'_a$. The length of the path is bounded by $\ell(e_{a-1})+\ell(e_{a})+8L_a+8\leq \ell(e_{a-1})+\ell(e_{a})+16L_a$.


Next, we consider path $Q_1$, that connects $x$ to $x_1$ in graph $G$, whose length is $L_1$. As before, either $x=x_1$ and the path contains no edges; or every edge on path $Q_1$ is original edge of $G$. As before,  from \Cref{claim: responding to queries level-0}, there is a path $P'_1$ in graph $H^0$ connecting $v^0(x)$ to $v^0(x_{1})$, whose length is at most $2L_1+2\leq 2D_i+2\leq 4D_i$. Consider now cluster $C_1=\coveringcluster^0_{i+2}(v^0(x))$ that is maintained by data structure $\DS^1_{i+2}$. Using the same arguments as before, $v^0(x_1)\in V(C_1)$ must hold. As before, cluster $C_1$ must be currently active at level $1$, and so supernode $u^1(C_1)$ must lie in $H^1$. We let $x'=\rep^1(C_1)$ be the current representative vertex of cluster $C_1$ at level $1$. Notice that $x'=\sigma_{i+2}(x)$. From Invariant \ref{inv: level 1 type 1 regular}, there is edge $(v^1(x'),u^1(C_1))$, and edge $(v^1(x_1),u^1(C_1))$ in graph $H^1$. Both these edges have length $D_{i+2}=4D_i$. From Invariant \ref{inv: level 1 type 2 regular}, graph $H^1$ contains edges $(v^1(e_1),u^1(C_1))$ of length at most $\ell(e_1)+D_{i+2}= \ell(e_1)+4D_i$. Consider the sequence $(v^1(x'),u^1(C_1),v_{e_{1}})$ of vertices of $H^1$. From the above discussion, this sequence of vertices defines a path in $H^1$ that we denote by $Q'_1$. The length of the path is bounded by $\ell(e_1)+8D_i$.
	
Lastly, we consider path $Q_{r+1}$, that connects $y_r$ to $y$ in graph $G$, whose length is $L_{r+1}$. This path is processed exactly like $Q_1$, with vertex $y$ playing the role of $x$, and vertex $y_r$ playing the role of $x_1$, so that 	we obtain a path $Q'_{r+1}$ in graph $H^1$, that connects vertex $v^1(y_r)$ to vertex $v^1(y')$, where $y'=\sigma_{i+2}(y)$, and the length of the path is bounded by $\ell(e_r)+8D_i$.

By concatenating the paths $Q_1',Q_2',\ldots,Q_{r+1}'$, we obtain a path $Q^*$ in graph $H^1$, that connects $x'$ to $y'$. The length of the path is bounded by $\sum_{a=1}^{r+1}\left (2\ell(e_a)+16L_a\right )+16D_i\leq 32D_i$.
\end{proof}



The next observation will allow us to transform paths in graph $H^1$ to paths in graph $G$, while approximately preserving their lengths.



 
\begin{observation}\label{obs: back trans}
	There is a deterministic algorithm, that, given a path $P$ in graph $H^1$ of length $D$, connecting a pair of type-$1$ regular vertices $v^1(x)$ and $v^1(y)$, computes a path $P'$ in graph $G$, connecting $x$ to $y$, so that the length of $P'$ is at most $D\cdot \alpha(W)$. The running time of the algorithm is $O(|E(P')|)$.
\end{observation}

\begin{proof}
	The proof is by induction on the number of edges on path $P$; since $H^1$ is a bipartite graph, this number must be even.
	
	The base case is when $P$ contains two edges, so $P=(v^1(x),u^1(C),v^1(y))$, where $C$ is some cluster of $\cset^0$. Let $1\leq i\leq \log D^0$ be the index for which $C\in \cset^1_i$. We are then guaranteed from Invariant \ref{inv: level 1 type 1 regular}, that $v^0(x)\in V(C)$ and $v^0(y)\in V(C)$. Moreover, the lengths of the edges $(v^1(x),u^1(C))$ and $(v^1(y),u^1(C))$ in $H^1$ are both $D_i$, so $D=2D_i$.  We perform query $\shortestpathquery^0_i(C,v(x),v(y))$  in data structure $\DS^0$, obtaining a path $P'$ of length at most $\alpha(W)\cdot D_i$ connecting $v^0(x)$ to $v^0(y)$ in $H^0$, in time $O(|E(P')|)$. Since every type-1 regular vertex $v^0(z)\in V^0$ has degree $1$ in $H^0$, and the only vertex to which it is connected with an edge is the corresponding supernode $u^1(z)$, we can delete all type-1 regular vertices from $P'$ obtaining a valid path in $H^0$ connecting $u^0(x)$ to $u^0(y)$; the number of edges on $P'$ decreases by at most a constant factor. We then suppress all type-2 regular vertices on $P'$, and replace every supernode $u^0(z)$ on $P'$ with the corresponding vertex $z$ of $G$, obtaining a path $P''$ in graph $G$, that connects $x$ to $y$. The length of the path is bounded by $2\alpha(W)\cdot D_i\leq \alpha(W)\cdot D$ (we have used the fact that, for every type-2 regular vertex $v^0(e)$ in $H^0$, every edge incident to $v(e)$ in $H^0$ has length $\ell(e)$).
	
	
	Assume now that we are given a path $P$ in graph $H^1$, that contains more than two edges. The path connects type-1 regular vertices $v^1(x)$ and $v^1(y)$, and has length $D$. Assume first that there is at least one additional vertex $z\in V(G)$, with $z\not\in\set{x,y}$ such that $v^1(z)\in V(P)$. In this case, vertex $v^1(z)$ partitions path $P$ into two subpaths: path $P_1$ connecting $v^1(x)$ to $v^1(z)$, and path $P_2$ connecting $v^1(z)$ to $v^1(y)$. Denote the length of $P_1$ by $L_2$, and the length of $P_2$ by $L_2$. Using the induction hypothesis, we can compute a path $P'_1$, connecting $x$ to $z$ in graph $G$, whose length is at most $L_1\cdot \alpha(W)$, in time $O(|E(P'_1)|)$. Similarly, we can compute a path $P'_2$, connecting $z$ to $y$ in graph $G$, whose length is at most $L_2\cdot \alpha(W)$, in time $O(|E(P'_2)|)$. By concatenating the two paths, we obtain a path $P'$, connecting $x$ to $y$ in $G$, of length at most $L_1\cdot \alpha(W)+L_2\cdot \alpha(W)\leq D\cdot \alpha(W)$. Clearly, the running time of the algorithm is $O(|E(P')|)$.
	
	From now on we assume that every internal vertex of $P$ that is not a supernode is a type-2 regular vertex. Since path $P$ contains more than two edges, it must contain at least one such vertex. We let $v^1(e)$ be an arbitrary type-2 regular vertex that lies on path $P$. We denote by $u^1(C)$ and $u^1(C')$ the supernodes preceding and following $v^1(e)$ on path $P$, respectively. We let $z$ be the endpoint of $e$ that is responsible for edge $e'=(v^1(e),u^1(C))$ (if both endpoints of $e$ are responsible for this edge, we let $z$ be any endpoint of $e$). We define endpoint $z'$ of $e$ with respect to the edge $e''=(v^1(e),u^1(C'))$ similarly. Note that it is possible that $z=z'$. Assume that $C\in \cset^0_i$ and $C'\in \cset^0_{i'}$, so edge $e'$ has length $\ell(e)+D_i$, and edge $e''$ has length $\ell(e)+D_{i'}$. Note that, from Invariants \ref{inv: level 1 type 1 regular} and \ref{inv: level 1 type 2 regular}, edge $\hat e'=(v^1(z),u^1(C))$ is present in graph $H^1$, and its length is $D_i$, and similarly edge $\hat e''=(v^1(z'),u^1(C'))$ is present in $H_1$, and its length is $D_{i'}$.
	
	
	Vertex $v^1(e)$ partitions path $P$ into two subpaths: path $P_1$ connecting $v^1(x)$ to $v^1(e)$, and path $P_2$ connecting $v^1(e)$ to $v^1(z)$. We denote the length of $P_1$ by $L_1$ and the length of $P_2$ by $L_2$, so $L_1+L_2=D$. Let $P'_1$ be the path obtained from $P_1$, by replacing its last edge $e'$ with $\hat e'$. Now path $P_1'$ connects $v^1(x)$ to $v^1(z)$ in $H^1$, and its length is $L_1-\ell(e)$. Similarly, we let $P'_2$ be the path obtained from $P_2$, by replacing its first edge $e''$ with $\hat e''$. Now path $P_2'$ connects $v^1(z')$ to $v^1(y)$ in $H^1$, and its length is $L_2-\ell(e)$. From the induction hypothesis, we can compute a path $Q_1$ in graph $G$, connecting $x$ to $z$, so that the length of $Q_1$ is at most $\alpha(W)\cdot (L_1-\ell(e))$, in time $O(|E(Q_1)|)$. Similarly, we can compute a path $Q_2$ in graph $G$, connecting $z'$ to $y$, so that the length of $Q_2$ is at most $\alpha(W)\cdot (L_2-\ell(e))$, in time $O(|E(Q_2)|)$. Recall that $z$ and $z'$ are both endpoints of edge $e$. If $z=z'$, then we obtain the final path $P'$ in graph $G$, connecting $x$ to $y$, by concatenating the paths $Q_1$ and $Q_2$. Otherwise, path $P'$ is obtained by concatenating $Q_1,e$ and $Q_2$. In either case, the resulting path $P$ connects $x$ to $y$ in $G$, and its length is bounded by $\alpha(W)\cdot (L_1-\ell(e))+\alpha(W)\cdot (L_2-\ell(e))+\ell(e)\leq \alpha(W)\cdot (L_1+L_2)\leq \alpha(W)\cdot D$. The running time of the algorithm is $O(|E(P')|)$.
\end{proof}



We now prove the following claim, that can be viewed as an extension of \Cref{cor: level 0 queries}, and allows us to respond to approximate short path queries between pairs of vertices, provided that there is a short path connecting them in $G$ that only contains edges that are original edges of $G$ and edges of $A^1_k$.

\begin{claim}\label{cor: level 1 queries}
	There is a deterministic algorithm, that, for all $1\leq k\leq M$, at any time during the level-$1$ phase $\Phi^1_k$, given a pair $x,y$ of vertices of $G$, and a distance parameter $D'\leq D^*$ that is an integral power of $2$, responds "YES" or "NO", in time $O(\log W)$. If the algorithm responds "NO", then every path connecting $x$ to $y$ in the current graph $G$ either has length greater than $D'$, or contains at least one edge of $E^1_k$. If the algorithm responds "YES", then it can, additionally, return a path $P'$ in graph $G$, connecting $x$ to $y$, whose length is at most $100(\alpha(W))^2\cdot D$, in time $O(|E(P')|)$.
\end{claim}

\begin{proof}
We start by executing the algorithm from \Cref{cor: level 0 queries}, with the same pair $x,y$ of vertices. If the algorithm responds ``YES'', then we respond ``YES'' as well, and terminate the algorithm. In this case, the algorithm from \Cref{cor: level 0 queries} can also compute a path $P'$ in graph $G$, connecting $x$ to $y$, whose length is at most $4D'\cdot \alpha(W)$, in time $O(|E(P')|)$. We assume from now on that the algorithm from \Cref{cor: level 0 queries} responded ``NO''. Therefore, either there is no path connecting $x$ to $y$ in $G$ whose length is at most $D'$, or each such path contains some inserted edge.



Let $i=\log D'$, so that $D'=D_i$. 
In time $O(1)$, we compute vertices $x'=\sigma_{i+2}(x)$ and $y'=\sigma_{i+2}(y)$. If either of these vertices is undefined, then, from \Cref{obs: level-1 approx short path queries}, every path in graph $G$ connecting $x$ to $y$, whose length is at most $D$ contains an edge of $E^1_k$. We then terminate the algorithm and respond ``NO''. We assume from now on that both $x'$ and $y'$ are defined. Let $C=\coveringcluster^1_{i+5}(v^1(x'))$, that is maintained by data structure $\DS^1_{i+5}$. Note that, from \Cref{obs: level-1 approx short path queries}, if there is a path $P$ connecting $x$ to $y$ in $G$, whose length is at most $D_i$, that only contains original edges of $G$ and edges of $A^1_i$, then there must be a path $P'$ in the current graph $H^1$, of length at most $32D_i$ connecting $v^1(x')$ to $v^1(y')$, and so cluster $C$ must contain $v^1(y')$. 
We check, in time $O(\log W)$, whether $v^1(y')\in V(C)$. If this is not the case, then we return ``NO'', and otherwise we return ``YES''. 

From the above discussion, if our algorithm returned ``NO'', then  every path connecting $x$ to $y$ in the current graph $G$ either has length greater than $D'$, or contains at least one edge of $E^1_k$. We assume from now on that our algorithm returned ``YES'', and in particular that 
 $v^1(y')\in V(C)$ holds.
We can then obtain the desired path connecting $x$ to $y$ in $G$, as follows. 

First, we run query $\shortpath^1_{i+5}(C,v^1(x'),v^1(y'))$ in data structure $\DS^1_{i+5}$, to obtain a path $Q$ in graph $H^1$, connecting $v^1(x')$ to $v^1(y')$, whose length is at most $\alpha(W)\cdot D_{i+5}\leq 32\alpha(W)\cdot D'$, in time $O(|E(Q)|)$.  
Then we apply the algorithm from \Cref{obs: back trans} to path $Q$, to obtain a path $Q'$ in $G$, connecting $x'$ to $y'$, so that the length of $Q'$ is at most $32(\alpha(W))^2\cdot D'$. The running time of the algorithm is $O(|E(Q')|)$. 

Since $x'=\sigma_{i+2}(x)$, vertex $v^0(x')$ must belong to cluster $C'=\coveringcluster^0_{i+2}(x)$ in $\cset^0$. We perform query $\shortpath^0_{i+2}(C',v^0(x),v^0(x'))$ in data structure $\DS^0_{i+2}$, to obtain a path $Q_1$ in graph $H^0$, conncting $v^0(x)$ to $v^0(x')$, so that the length of the path is at most $\alpha(W)\cdot D_{i+2}\leq 4\alpha(W)\cdot D'$. As before, by deleting all type-1 regular vertices from the path, suppressing type-2 regular vertices, and substituting each supenode $u^1(z)$ with the corresponding vertex $z\in V(G)$, we obtain a path $Q_1'$ in graph $G$ that connects vertices $x$ and $x'$. It is easy to verify that $|E(Q_1')|\geq \Omega(|E(Q_1|))$, and so the time needed to compute path $Q_1'$ is bounded by $O(|E(Q_1')|)$. Furthermore, the length of path $Q_1'$ in $G$ is bounded by the length of path $Q_1$ in $H^0$, which is in turn bounded by $4\alpha(W)\cdot D'$.

We similarly compute a path $Q_2'$ in graph $G$, connecting vertices $y$ and $y'$, so that the length of $Q_2'$ is at most $4\alpha(W)\cdot D$, in time $O(|E(Q_2')|)$. By combining paths $Q_1',Q'$ and $Q_2'$, we obtain the final path $P'$ in graph $G$, connecting $x$ to $y$. From the above discussion, the length of the path is bounded by $32(\alpha(W))^2\cdot D'+8\alpha(W)\cdot D'\leq 64(\alpha(W))^2\cdot D'$, and the running time of the algorithm is $O(|E(P')|)$.
\end{proof}


\paragraph{Analysis of total update time.}
We start by bounding the total update time required for maintaining the level-$1$ data structure over the course of a single level-$1$ phase $\Phi^1_k$. As shown already, the time required to initialize graph $H^1$ is $O(|A^1_k|\cdot \Delta(W)\cdot \log W)\leq O(m \cdot \Delta(W)\cdot \log W)\leq O(W'\cdot \mu \cdot \Delta(W)\cdot \log W)$. 
Since $D^1\leq O(W)$, the time required to initialize all graphs $H^1_i$, for $1\leq i\leq \log D^1$, is bouned by $O(W'\cdot \mu \cdot \Delta(W)\cdot \log^2 W)$.

The time that is required in order to compute the update sequence $\hat \Sigma^1_k$ is bounded by the total update time of the level-$0$ data structure over the course of Phase $\Phi^1_k$.

From our assumption in the statement of \Cref{thm: main fully-dynamic APSP single scale}, for all $1\le i\leq \log D^1$, the total update time required for maintaining data structure $\DS^1_i$ is bounded by $|S^1_k|^{1+\delta}\cdot (\mu_1\cdot \log W)^c$, where
$\mu_1\leq O(\Delta(W)\cdot \log W)$ is the dynamic degree bound for $\iset^1$ and $\hat \Sigma^1$. Since $|S^1_k|\leq M^q$, we get that the total update time that is required in order to maintain data structure $\DS^1_i$ over the course of a single level-$1$ phase is bounded by $O\left (M^{q(1+\delta)}\cdot (\Delta(W))^c\cdot (\log W)^{2c}\right )$, and the total update time required for maintaining all data structures $\DS^1_i$, for $1\leq i\leq \log D^1$, is bounded by 
$O\left (M^{q(1+\delta)}\cdot (\Delta(W))^c\cdot (\log W)^{2c+1}\right )$. Since the number of level-$1$ phases is bounded by $M$, the total update time required to maintain all level-1 data structures over the course of the entire algorithm is bounded by:

\[\begin{split} 
T^1&\leq T^0+O(M\cdot W'\cdot \mu \cdot \Delta(W)\cdot \log^2 W)+O\left (M^{(q+1)(1+\delta)}\cdot (\Delta(W))^c\cdot (\log W)^{2c+1}\right )  \\
&\leq c'\cdot (W')^{1+\delta}\cdot \mu^c(\log W)^{c+1}+O\left (M^{(q+1)(1+\delta)}\cdot\mu\cdot (\Delta(W))^c\cdot (\log W)^{2c+1}\right )\\
&\leq c'\cdot M^{(q+1)(1+\delta)}\cdot\mu^c\cdot (\Delta(W))^c\cdot (\log W)^{2c+1},
\end{split}
\]
where, as before, $c'$ is a large enough constant.




==> arxiv-version-final/level-L-inner.tex <==
\subsection{Level $L$ Graph}



==> arxiv-version-final/manage-cluster.tex <==
\newpage

\subsection{Managing a Single Cluster - Algorithm \algmanagecluster}
\label{subsec: manage one cluster}

In this subsection we describe Algorithm \algmanagecluster. 
The input to the algorithm is a valid input structure $\iset=\left(C,\set{\ell(e)}_{e\in E(C)},D \right )$, that undergoes a sequence of valid update operations with dynamic degree bound $\mu$. We denote by $N=N^0(C)$ the number of regular vertices in $C$ at the beginning of the algorithm, and we assume that $N\leq \hat W$. Intuitively, $C$ is a cluster (vertex-induced subgraph) of the graph $H$, on which we are trying to solve the \recdynnc problem. When cluster $C$ is added to the collection $\cset$ of clusters that the algorithm for the \recdynnc problem on graph $H$ maintains, we will immediately initialize Algorithm \algmanagecluster on it. 

Intuitively, algorithm \algmanagecluster runs Algorithm \algmaintaincluster on cluster $C$, as it undergoes a sequence of valid update operations. Recall that Algorithm \algmaintaincluster supports queries $\spquery(C,v,v')$ betwween pairs $v,v'$ of regular vertices of $C$. Whenever Algorithm \algmaintaincluster raises a flag $F_C$, and supplies a pair $x,y$ of regular vertices of $C$ with $\dist_C(x,y)\geq\Delta(\hat W)\cdot D$, our algorithm will perform a \emph{cluster splitting} operation. The Cluster Splitting operation, that we implement via a procedure that we call $\pcsplit$, is the most crucial ingredient of Algorithm \algmanagecluster. 


More formally,
at the beginning of Procedure \pcsplit, we are given the current cluster $C$, and two regular vertices $x,y\in V(C)$, for which $\dist_C(x,y)\geq\Delta(\hat W)\cdot D$ holds. The output of the procedure is a pair $C',C''\subseteq C$ of clusters of $C$, for which the following properties hold:

\begin{properties}{P}
	\item $N(C')\leq N(C'')$, and $N(C')\leq N(C)/2$, where $N(C')$ and $N(C'')$ are the number of regular vertices in $C'$ and $C''$ respectively; \label{prop: csplit: C; is smaller}
	
	\item for every regular vertex $v\in V(C)$, either $B_C(v,D)\subseteq V(C')$, or $B_C(v,D)\subseteq V(C'')$ holds; and \label{prop: csplit: ncover}
	
	\item either (i) $x\in V(C')\setminus V(C'')$ and $y\in V(C'')\setminus V(C')$ holds; or (ii) the opposite holds:  $x\in V(C'')\setminus V(C')$ and $y\in V(C')\setminus V(C'')$; \label{proc: csplit: one of x,y in each cluster}
	
	\item either (i) $B_C(x,\Delta(\hat W)\cdot D/2)\subseteq V(C')$ and $B_C(y,\Delta(\hat W)\cdot D/2)\subseteq V(C'')$; or (ii) the opposite holds: $B_C(x,\Delta(\hat W)\cdot D/2)\subseteq V(C'')$ and $B_C(y,\Delta(\hat W)\cdot D/2)\subseteq V(C')$. \label{prop: csplit: one ball unchanged}
\end{properties}

Consider now the output $(C',C'')$ of procedure $\pcsplit$. We add cluster $C'$ to the collection $\cset$ of the clusters that the algorithm for the \recdynnc problem maintains on graph $H$, and immidiately initialize Algorithm \algmanagecluster on $C'$. Additionally, we let $\Sigma'$ be a sequence of update operations for cluster $C$, that is defined as follows: first, for every edge $e\in E(C)\setminus E(C'')$, we add to $\Sigma'$ edge-deletion operation of edge $e$. Next, for every vertex $z\in V(C)\setminus V(C'')$ (which must now be an isolated vertex of $C$), we add to $\Sigma'$ isolated vertex-deletion operation of vertex $z$. Cluster $C$ in $\cset$ is update via the update sequence $\Sigma'$. Additionally, $\Sigma'$ becomes a flag-lowering update sequence for algorithm $\algmaintaincluster$ on cluster $C$. 

Assume w.l.o.g. that $x\in V(C')\setminus V(C'')$ and $y\in V(C'')\setminus V(C')$ holds. In this case, from Property \ref{prop: csplit: one ball unchanged}, $B_C(x,\Delta(\hat W)\cdot D/2)\subseteq V(C')$ and $B_C(y,\Delta(\hat W)\cdot D/2)\subseteq V(C'')$ hold. Clearly, vertex $x$ is deleted from cluster $C$ as the result of the update sequence $\Sigma'$, and moreover, none of the edges and vertices of $B_C(y,\Delta(\hat W)\cdot D/2)$ are deleted from $C$ via sequence $\Sigma'$. Therefore, $\Sigma'$ is a valid flag-lowering sequence.

When, as the result of Procedure \pcsplit, cluster $C'$ is added to $\cset$, and cluster $C$ is replaced with $C''$ via the flag-lowering sequence $\Sigma'$ of update operations, we say that cluster $C'$ was \emph{split off from cluster $C$}, and we say that $C'$ is a \emph{child-cluster} of cluster $C$. We denote by $N^0(C')$ the total number of regular vertices that lie in cluster $C'$ when it is first created. %For convenience, we also denote by $N=N^0(C)$ the number of regular vertices in cluster $C$, when it was first added to set $\cset$. 
Recall that $N=N^0(C)$ is the number of regular vertices in the initial cluster $C$, and $N\leq \hat W$ holds. Let $q=\ceil{\log \log N}$.

Throughout the algorithm, let $\dset(C)$ denote the collection of all child-clusters of cluster $C$ that have been constructed so far. We partition the collection $\dset(C)$ of clusters into $q+1$ classes $\dset_0,\ldots,\dset_q$. Let $C'\in \cset$ be any such cluster. For an integer $0\leq i\leq q$, we say that $C'$ belongs to class $\dset_i$, if:


\[N^{1-1/2^i}\leq N^0(C')<N^{1-1/2^{i+1}} \].


Let $q'=\ceil{\log(1/\eps)}$. The goal of Procedure \pcsplit is to ensure the following additional property:

\begin{properties}[4]{P}
	\item for every regular vertex $x$ that belonged to $V(C)$ initially,  $x$ may ever belong to at most one cluster of $\dset_0\cup\cdots\cup \dset_{q'}$; additionally, for all $q'< i\leq q$, the total number of clusters in class $\dset_i$ to which $x$ ever belongs is at most $\frac{2N^{\eps/ 2^i}}{\eps}$.\label{prop: csplit: few clusters}
\end{properties}

Let $r=\ceil{1/\eps}$.
Throughout the algorithm, 
for every regular vertex $x\in V(C)$, and every index $q'<i\leq q$, we
maintain a counter $n_i(x)$, that denotes the total number of clusters $C'\in \dset_i$, to which $x$ ever belonged. We also
 maintan a partition $(T_0^i,T_1^i,\ldots,T_{r+2}^i)$ of the regular vertices of $V(C)$. A regular vertex $x\in V(C)$ belongs to set $T_j^i$, for $0\leq j\leq r+1$, if and only if:
 
 
 \[  j\cdot N^{\eps/ 2^i}\leq n_i(x)<(j+1)\cdot N^{\eps/ 2^i}.\]


If $n_i(x)\geq (r+1)\cdot N^{\eps\cdot 2^i}$, then $x$ belongs to set $T^i_{r+2}$. In fact, we will later show that our algorithm ensures that $T^i_{r+2}=\emptyset$ holds.

In order to execute Procedure \pcsplit, we use Procedure \proccut, which is a variant of the standard Ball-Growing technique of ..., and is somewhat similar to a procedure that was used in \cite{APSP-previous}.

==> arxiv-version-final/old-results-techniques.tex <==

\iffalse
From the paper: Even in unweighted graphs, all previously adaptive algorithms for decremental APSP (for any approximation) had total update time at least $\Omega(n^2)$ [HKN16, GWN20, CS20, EFGW20]; for weighted graphs they were even slower. 

\paragraph{Fully dynamic APSP, low approximation factor regime:}

\cite{demetrescu2004new,thorup2004fully} exact algorithm for fully dynamic \APSP, with $\tilde O(n^2)$ amortized update time (per update)

\cite{bernstein2009fully}: 
Fully dynamic 
maintains $(2+\eps)$-approximate distances between all pairs of vertices, with update time $m^{1+o(1)}$ per update. fully dynamic. randomized.

\cite{brand2021fast}
maintains $(1+\eps)$-approximate distances between all pairs of vertices, deterministically in a fully dynamic graph, with update time per operation: $O\left (n^2\cdot (1/\eps)^{\sqrt{2\log_{1/\eps}n}}\right )$, preprocessing time $O(n^{\omega}\cdot(1/\eps)^{\sqrt{2\log_{1/\eps}n}} )$



From the paper: Even in unweighted graphs, all previously adaptive algorithms for decremental APSP (for any approximation) had total update time at least $\Omega(n^2)$ [HKN16, GWN20, CS20, EFGW20]; for weighted graphs they were even slower. 




To summarize, ideally we would like an algorithm for decremental \APSP in weighted undirected graphs that achieves the following properties:

\begin{itemize}
	\item it can withstand an adaptive adversary (and is ideally deterministic);
	\item it has query time $\tilde O(|E(P)|)$ for $\shortestpathquery$, where $P$ is the returned path, and query time $\tilde O(1)$ for \distquery;
	\item it has near-linear in $m$ total update time; and
	\item it has a reasonably low approximation factor (ideally, polylogarithmic or constant).
\end{itemize}

Our main result comes close to achieving all these properties. Specifically, we provide a \emph{deterministic} algorithm for \APSP in weighted undirected graphs. For any precision parameter $\Omega(1/\log\log m)<\eps<1$, the algorithm achieves approximation factor 
$(\log m)^{2^{O(1/\eps)}}$, with total update time: $$O\left (m^{1+O(\eps)}\cdot (\log m)^{O(1/\eps^2)}\cdot \log L\right ).$$ The query time for processing $\distquery$ is $O(\log m \log\log L)$, and the query time for $\shortestpathquery$ is $O(|E(P)|)+O(\log m \log\log L)$, where $P$ is the returned path.
In particular, by letting $\eps$ be a small enough constant, we obtain a $O(\poly\log m)$-approximation with total update time time $O(m^{1+\delta})$, for any constant $0<\delta<1$, and by letting $1/\eps$ be a slowly growing function of $m$ (for example, $1/\eps=O(\log(\log^*m))$), we obtain an approximation factor $(\log m)^{O(\log^* m)}$, and total update time $O(m^{1+o(1)})$.
\fi




\subsection{Our Results and Techniques}

Our main result is a deterministic algorithm for decremental \APSP, that is summarized in the following theorem.
\begin{theorem}\label{thm: main}
	There is a deterministic algorithm, that, given an $m$-edge graph $G$ with length $\ell(e)\geq 1$ on its edges, that undergoes an online sequence of edge deletions, together with a parameter $c/\log\log m<\eps<1$ for some large enough constant $c$, supports approximate $\shortestpathquery$ queries and $\distquery$ queries with approximation factor $O\left ((\log m)^{2^{O(1/\eps)}}\right )$.  The query time for processing $\distquery$ is $O(\log m \log\log L)$, and the query time for processing $\shortestpathquery$ is $O(|E(P)|)+O(\log m \log\log L)$, where $P$ is the returned path, and $L$ is the ratio of longest to shortest edge length. The total update time of the algorithm is bounded by: $$O\left (m^{1+O(\eps)}\cdot (\log m)^{O(1/\eps^2)}\cdot \log L\right ).$$
\end{theorem}

Our proof exploits the decremental Sparse Neighborhood Cover problem, for which we provide the following algorithm:


\begin{theorem}\label{thm: NC}
	There is a deterministic algorithm, that, given an $m$-edge graph $G$ with integral lengths $\ell(e)\geq 1$ on its edges, that undergoes an online sequence of edge deletions, together with parameters $c/\log\log m<\eps<1$ for some large enough constant $c$, and $D\geq 1$, maintains a weak $(D,\alpha\cdot D)$-neighborhood cover $\cset$ of $G$, for $\alpha=O\left ((\log m)^{2^{O(1/\eps)}}\right )$, and  supports  queries $\spquery(C,v,v')$: given a cluster $C\in \cset$, and two  vertices $v,v'\in V(C)$, return a path $P$ connecting $v$ to $v'$ in $G$, of length at most $\alpha\cdot D$, in time $O(|E(P)|)$.
	Additionally, for every vertex $v\in V(G)$, the algorithm maintains a cluster $C=\coveringcluster(v)$ in $\cset$, with $B_G(v,D)\subseteq V(C)$.
	The algorithm starts with $\cset=\set{G}$, and the only allowed changes to the clusters in $\cset$ are: (i) delete an edge from a cluster $C\in \cset$; (ii) delete an isolated vertex from a cluster $C\in \cset$; and (iii) add a new cluster $C'$ to $\cset$, where $C'\subseteq C$ for some cluster $C\in \cset$. The algorithm has total update time $O\left (m^{1+O(\eps)}\cdot (\log m)^{O(1/\eps^2)}\right )$ and ensures that, for every vertex $v\in V(G)$, the total number of clusters $C\in \cset$ to which $v$ ever belongs over the course of the algorithm is at most  $m^{O(1/\log\log m)}$. 
\end{theorem}

We remark that the above theorem requires that we initially set $\cset=\set{G}$. Clearly, this initial cluster set $\cset$ may not be a valid neighborhood cover of $G$. Therefore, before the algorithm processes any updates of graph $G$, it may update this initial cluster set $\cset$, via changes of the types that are allowed by the theorem, until it becomes a valid neighborhood cover. We also note that we allow graphs to have parallel edges, so $m$ may be much larger than $|V(G)|$.


@@@

\paragraph{Recursive Dynamic Neighborhood Cover.}
As mentioned already, one advantage of considering the \NC problem is that its solution naturally provides an emulator for the input graph $G$, which in turn can be used in order to compose algorithms for \NC recursively.
In fact, we initially prove a weaker version of \Cref{thm: NC}, by providing an algorithm (that we denote here for brevity by $\alg'$), that achieves a similar approximation factor, but a slower running time of: $$O\left (m^{1+O(\eps)}\cdot \poly(D)\cdot (\log m)^{O(1/\eps^2)}\right )$$ (on the positive side, the algorithm maintains a {\bf strong} neighborhood cover of the graph $G$). Recall that we call the parameter $D$ the \emph{target distance threshold} for the \NC problem instance.
We use the recursive composability of \NC in order to obtain the desired running time, as follows\footnote{A similar approach of recursive composition of emulators was used in numerous algorithms for \APSP; see, e.g. \cite{chechik}.}. Using standard rescaling techniques, we can assume that $1\leq D\leq \Theta(m)$. For all $1\leq i\leq O(1/\eps)$, let $D_i=m^{\eps i}$. We obtain an algorithm for the Sparse \NC problem for each target distance threshold $D_i$ recursively. For the base of the recursion, when $i=1$, we simply run Algorithm $\alg'$, to obtain the desired running time of $O\left (m^{1+O(\eps)}\cdot (\log m)^{O(1/\eps^2)}\right )$. Assume now that we have obtained an algorithm for target distance threshold $D_i$, that maintains a neighborhood cover $\cset_i$ of graph $G$. In order to obtain an algorithm for target distance threshold $D_{i+1}$, we construct a new graph $H$, by starting with $H=G$, deleting all edges of length greater than $D_{i+1}$, and rounding the lengths of all remaining edges up to the next integral multiple of $D_i$. Additionally, for every cluster $C\in \cset_i$, we add a vertex $u(C)$ (called a supernode), that connects, with an edge of length $D_i$, to every vertex $v\in V(C)\cap V(G)$. It is not hard to show that this new graph $H$ approximately preserves all distances between the vertices of $G$, that are in the range $(D_i,D_{i+1}]$. Since the length of every edge in $H$ is an integral multiple of $D_i$, scaling all edge lengths down by factor $D_i$ does not change the problem. It is then sufficient to solve the \NC problem in the resulting dynamic graph $H$, with target distance threshold $D_{i+1}/D_i=m^{\eps}$, which can again be done via Algorithm $\alg'$, with total update time $O\left (m^{1+O(\eps)}\cdot (\log m)^{O(1/\eps^2)}\right )$. The final algorithm for \Cref{thm: NC} is then obtained by recursively composing Algorithm $\alg'$ with itself $O(1/\eps)$ times. %Throughout, given a graph $H$, a vertex $v\in V(H)$, and a distance bound $D$, we denote by $B_H(v,D)$ the \emph{ball of radius $D$ around $v$}, which is the set of all vertices of $H$ that lie within distance $D$ from $v$.

In order to be able to compose algorithms for the \NC problem using the above approach, we define the problem slightly differently, and we call the resulting variation of the problem Recursive Dynamic Neighborhood Cover, or \recdynnc. We assume that the input is a bipartite graph $H=(V,U,E)$, with non-negative edge lengths. Intuitively, the vertices in set $V$, that we refer to as \emph{regular vertices}, correspond to vertices of the original graph $G$, while the vertices in set $U$, that we call \emph{supernodes}, represent some neighborhood cover $\cset$ of the graph $G$ that is possibly maintained recursively: $U=\set{u(C)\mid C\in \cset}$. (In order to obtain the initial graph $H$, we subdivide every edge of $G$ by a new regular vertex; we view the original vertices of $G$ as supernodes; and for every vertex $v\in V(G)$, we add a new regular vertex $v'$ that connects to $v$ with a length-$1$ edge.) In addition to supporting standard edge-deletion and isolated vertex-deletion updates, we require that the algorithm for the \recdynnc problem supports a new update operation, that we call \emph{supernode splitting}\footnote{We note that a similar approach to handling cluster-splitting in an emulator that is based on clustering was used before in numerous works, including, e.g., \cite{BernsteinChechik,Bernstein,fast-vertex-sparsest,chechikLowStretch}.}. In this operation, we are given a supernode $u\in V(H)$, and a subset $E'$ of edges that are incident to $u$ in graph $H$. The update creates a new supernode $u'$ in graph $H$, and, for every edge $e=(u,v)\in E'$, adds a new edge $(u',v)$ of length $\ell(e)$ to $H$. 
The purpose of this update operation is to mimic the addition of a new cluster $C$ to $\cset$, where $C\subseteq C'$ for some existing cluster $C'\in \cset$. The supernode-splitting operation is applied to supernode $u(C')$, with edge set $E'$ containing all edges $(v,u(C'))$ with $v\in V(C)$, and the operation creates a new supernode $u(C)$.
Supernode-splitting operation, however, may insert some new edges into the graph $H$.
This creates several difficulties, especially in bounding total update times in terms of number of edges. We get around this problem as follows. Recall that the supernodes in set $U$ generally correspond to clusters in some dynamic neighborhood cover $\cset$, that we maintain recursively. We ensure that this neighborhood cover is sparse, that is, every regular vertex may only belong to a small number of such clusters (typically, at most $m^{1/O(\log\log m)}$). This in turn ensures that, in graph $H$, for every regular vertex $v\in V(H)$, the total number of edges incident to $v$ that ever belong to $H$ is also bounded by $m^{1/O(\log\log m)}$. We refer to this bound as the \emph{dynamic degree bound}, and denote it by $\mu$. Therefore, if we denote by $N(H)$ the number of regular vertices that belong to the initial graph $H$, then the total number of edges that ever belong to $H$ is bounded by $N(H)\cdot \mu$. This allows us to use the number of regular vertices of $H$ as a proxy to bounding the number of edges in $H$.

To summarize, the definition of the \recdynnc problem is almost identical to that of the Sparse \NC problem. The main difference is that the input graph now has a specific structure (that is, it is a bipartite graph), and, in addition to edge-deletions, we also need to support isolated vertex deletions and supernode-splitting updates. Additional minor difference is that we only require that the covering properties of the neighborhood cover hold for the regular vertices of $H$ (and not necessarily the supernodes), and we only bound the number of clusters ever containing a vertex for regular vertices (and not supernodes). These are minor technical details that are immaterial to this high-level overview. 

%In the remainder of this overview, for a subgraph $C$ of the input graph $H$, we denote by $N(C)$ the number of regular vertices in $C$, and we denote by $N$ the number of regular vertices in the initial graph $H$.

\paragraph{Procedure $\proccut$ and reduction to the \maintaincluster problem.}
One of the main building blocks of our algorithm is Procedure \proccut. Suppose our goal is to design an algorithm for the \recdynnc problem on input graph $H$, with target distance threshold $D$, and let $\cset$ be the neighborhood cover that we maintain. 
We denote by $N$ the number of regular vertices in the initial graph $H$, and, for each subgraph $H'\subseteq H$, we denote by $N(H')$ the number of regular vertices in $H'$.
Given a cluster $C\in \cset$, and two vertices $x,y\in C$, such that $\dist_C(x,y)> \Omega(D\poly\log N)$, procedure $\proccut$ produces two vertex-induced subgraphs $C',C''\subseteq C$, such that $N(C')\leq N(C'')$, $\diam(C')\leq O(D\poly\log N)$, and each of $C',C''$ contains exactly one of the two vertices $x,y$. Moreover, it guarantees that, for every vertex $v\in V(C)$, either $B_C(v,D)\subseteq C'$, or $B_C(v,D)\subseteq C''$ holds. We then add $C'$ to $\cset$, and update $C$ by deleting edges and vertices from it, until $C=C''$ holds. This procedure is exploited by our algorithm in two ways: first, we compute an initial strong $(D,D\cdot \poly\log N)$-neighborhood cover $\cset$ of the input graph $H$, before it undergoes any updates, by repeatedly invoking this procedure. Later, as the algorithm progresses, and update operations are applied to $H$, the diameters of some clusters $C\in \cset$ may grow. Whenever we identify such a situation, we use Procedure $\proccut$ in order to cut the cluster $C$ into smaller subclusters. We note that, if $C'$ and $C''$ are the outcome of applying Procedure \proccut to cluster $C$, then we cannot guarantee that the two clusters are disjoint, so they may share edges and vertices. Therefore, a vertex of $H$ may belong to a number of clusters in $\cset$. The main challenge in designing Procedure \proccut is to ensure that every vertex of $H$ only belongs to a small number of clusters (at most $N^{O(1/\log\log N)}$) over the course of the entire algorithm. The procedure uses a carefully designed modification of the ball-growing technique  of \cite{LR} that allows us to ensure this property. 
We note that several previous works used the ball-growing technique in order to compute and maintain a clustering of a graph. For example, \cite{chechikLowStretch} employ this technique in order to maintain clustering at every distance scale. However, the clusters that they maintain at each distance scale are disjoint, and so they can use the standard ball-growing procedure of \cite{LR} in order to ensure that relatively few edges have endpoints in different clusters. In contrast, in order to maintain a neighborhood cover, we need to allow clusters at each distance scale to overlap. While one can easily adapt the standard ball-growing procedure of \cite{LR} to still ensure that the total number of edges in the resulting clusters is sufficiently small, this would only ensure that every vertex belongs to relatively few clusters {\bf on average}. It is the strict requirement that {\bf every} vertex may only ever belong to few clusters in the neighborhood cover that makes the design of Procedure \proccut challenging. We are not aware of any other work that adapted the ball-growing technique to this type of requirement, except for the algorithm of \cite{neighborhood-cover2,neighborhood-cover1}, who did so in the static setting. It is unclear though how to adapt their techniques to the dynamic setting.

We also use Procedure \proccut to reduce the \recdynnc problem to a new problem, that we call \maintaincluster. In this problem, we are given some cluster $C$ that was just added to the neighborhood cover $\cset$. The goal is to support  queries $\spquery(C,v,v')$: given a pair $v,v'\in V(C)$ of vertices of $C$, return a path $P$ connecting $v$ to $v'$ in $C$, of length at most $\alpha\cdot D$, in time $O(|E(P)|)$. However, the algorithm may, at any time, raise a flag $F_C$, to indicate that the diameter of $C$ has become too large. When flag $F_C$ is raised, the algorithm must provide two vertices $x,y\in C$, with $\dist_C{(x,y)}>\Omega(D\poly\log N)$. The algorithm then obtains a sequence of update operations (that we call a \emph{flag-lowering sequence}), at the end of which either $x$ or $y$ are deleted from $C$, and flag $F_C$ is lowered. Queries $\spquery$ may only be asked when the flag $F_C$ is down. Once flag $F_C$ is lowered, the algorithm may raise it again immediately, as long as it supplies a new pair $x',y'\in V(C)$ of vertices with $\dist_C{(x',y')}>\Omega(D\poly\log N)$. Intuitively, once flag $F_C$ is raised, we will simply run Procedure \proccut on cluster $C$, with the vertices $x,y$ supplied by the algorithm, and obtain two new clusters $C'$, $C''$. Assume that $C'$ contains fewer regular vertices than $C''$. We then add $C'$ to $\cset$, and delete edges and vertices from $C$ until $C=C''$ holds, thus creating a flag-lowering update sequence for it. In order to obtain an algorithm for the \recdynnc problem, it is then enough to obtain an algorithm for the \maintaincluster problem. We focus on this problem in the remainder of this exposition.

\paragraph{Pseudocuts, expanders, and their embeddings.}

The next central tool that we introduce is balanced pseudocuts. Consider a cluster $C$, for which we would like to solve the \maintaincluster problem, as $C$ undergoes a sequence of online updates, with  target distance threshold $D$. 
For a given balance parameter $\rho$, a standard balanced multicut for $C$ can be defined as a set $E'\subseteq E(C)$ of edges, such that every connected component of $C\setminus E'$ contains at most $N(C)/\rho$ regular vertices. We weaken this notion of balanced multicut, and use instead \emph{balanced pseudocuts}. Let $D'=\Theta(D\poly\log N)$. A $(D',\rho)$-pseudocut in cluster $C$ is a collection $E'$ of its edges, such that, in graph $C\setminus E'$, for every vertex $v\in V(C)$, the ball $B_{C\setminus E'}(v,D')$ contains at most $N(C)/\rho$ regular vertices. In particular, once all edges of $E'$ are deleted from $C$, if we compute a strong $(D,D')$-neighborhood cover $\cset'$ of $C$, then we are guaranteed that for all $C'\in \cset'$, $N(C')\leq N(C)/\rho$. We note that standard balanced multicuts also achieve this useful property. An advantage of using pseudocuts is that we can design a near-linear time algorithm that computes a $(D',\rho)$-pseudocut $E'$ in graph $C$, for $\rho=N^{\eps}$, and additionally it computes an expander $X$, whose vertex set is $\set{v_e\mid e\in E''}$, where $E''\subseteq E'$ is a large subset of the edges of $E'$, together with an embedding of $X$ into $C$, via short embedding paths, that causes a low edge-congestion  (see \Cref{thm: compute pseudocut and expander} for details).
This allows us to build on known expander-based techniques in order to design an efficient algorithm for the \maintaincluster problem. Consider the following algorithm, that consists of a number of phases. In every phase, we start by computing a $(D',\rho)$-pseudocut $E'$ of $C$, the corresponding expander $X$, and its embedding into $C$. Let $E''\subseteq E'$ be the set of edges $e$, whose corresponding vertex $v_e$ lies in the expander $X$, so $V(X)=\set{v_e\mid e\in E''}$. We then use two data structures. The first data structure is an \EST $\tau$, whose root $s$ is a new vertex, that connects to each endpoint of every edge in $E''$, and has depth $O(D\poly\log N)$. This data structure allows us to ensure that every vertex of $C$ is close enough to some edge of $E''$, and to identify when this is no longer the case, so that flag $F_C$ is raised. Additionally, we use known algorithms for \APSP on expanders, together with the algorithm of  \cite{expander-pruning} for expander pruning, in order to maintain the expander $X$ (under update operations performed on the cluster $C$), and its embedding into $C$. This allows us to ensure that all edges in $E''$ remain sufficiently close to each other. These two data structures are sufficient in order to support the $\spquery(C,v,v')$ queries. If the initial pseudocut $E'$ was sufficiently large, then these data structures can be maintained over a long enough sequence of update operations to cluster $C$. Once a large enough number of edges are deleted from $C$, expander $X$ can no longer be maintained, and we recompute the whole data structure from scratch. Therefore, as long as the pseudocut $E'$ that our algorithm computes is sufficiently large (for example, its cardinality is at least $(N(C))^{1-\eps}$), we can support the $\spquery(C,v,v')$ queries as needed, with a very efficient algorithm. 

It now remains to deal with the situation where the size of the pseudocut $E'$ is small. One simple way to handle it is to maintain $2|E'|$ \EST data structures, each of which is rooted at an  endpoint of a distinct edge of $E'$, and has depth threshold $\Theta(D\poly\log N)$.
As long as the root vertex of an \EST $\tau$ remains in the current cluster $C$, we say that the tree $\tau$ \emph{survives}. As long as at least one of the \ESTs rooted at the endpoints of the edges in $E'$ survives, we can support the $\spquery(C,v,v')$ queries using any such tree. We can also use such a tree in order to detect when the diameter of the cluster becomes too large, and, when this happens, to identify a pair $x,y$ of vertices of $C$ with $\dist_C(x,y)$ sufficiently large. Once every \EST that we maintain is destroyed, we are guaranteed that all edges of $E'$ are deleted from $C$. We can then iteratively apply Procedure \proccut in order to further decompose $C$ into a collection of low-diameter clusters (that is, we compute a collection $\cset'$ of subgraphs of $C$, such that $\cset'$ is a $(D,D')$-neighborhood cover for $C$). Since $E'$ was a $(D',\rho)$-pseudocut for the original cluster $C$, we are then guaranteed that every cluster in $\cset'$ is significantly smaller than $C$, and contains at most $N(C)/\rho$ regular vertices. We can then initialize the algorithm for solving the \maintaincluster problem on each cluster of $\cset'$.
This approach already gives non-trivial guarantees (though in order to optimize it, we should choose a different  threshold for the cardinality of $E'$: if $|E'|>\sqrt{N(C)}$, we should use the expander-based approach, and otherwise we should maintain the \EST's). 
Our rough estimate is that such an algorithm would result in total update time $O\left (m^{1.5+O(\eps)}\cdot (\log m)^{O(1/\eps^2)}\right )$, but it is still much higher than our desired update time.

In order to achieve our desired near-linear total update time, % of $O\left (m^{1+O(\eps)}\cdot \poly(D)\cdot (\log m)^{O(1/\eps^2)}\right )$, 
we exploit again the recursive composability properties of the \recdynnc problem. 
Specifically, consider the situation where the pseudocut $E'$ that we have computed is small, that is, $|E'|<(N(C))^{1-\eps}$, and consider the graph $H'=C\setminus E'$. For all $1\leq i\leq \ceil{\log D}$, we solve the \recdynnc problem in graph $H'$ with target distance threshold $D_i=2^i$ recursively. Fix some index $1\leq i\leq \ceil{\log D}$, and let $\cset_i$ be the initial strong $(D_i,D_i\cdot \poly\log N)$-neighborhood cover that this algorithm computes. The properties of the balanced pseudocut ensure that each cluster $C'\in \cset_i$ is significantly smaller that $C$: namely, $N(C')\leq N(C)/\rho\leq (N(C))^{1-\eps}$. Therefore, we can solve the \maintaincluster problem on each such cluster recursively, and we also do so for every cluster that is later added to $\cset_i$. Let $\tilde\cset=\bigcup_i\cset_i$ be the dynamic collection of clusters that we maintain.

We use the set $\tilde\cset$ of clusters in order to construct a \emph{contracted graph} $\hat H$. The vertex set of $\hat H$ consists of the set $S$ of regular vertices -- all regular vertices that serve as endpoints of the edges of $E'$ (the edges of the pseudo-cut); and the set $U'=\set{u(C')\mid C'\in \tilde\cset}$ of supernodes. For every edge $e=(u,v)\in E'$, where $v\in S$ is a regular vertex, we add an edge connecting $v$ to every supernode $u(C')$, such that cluster $C'$ contains either $v$ or $u$. The length of the edge is $D_i$, where $i$ is the index for which $C'\in \cset_i$ holds.
It is not hard to show that the distances between the vertices of $S$ are approximately preserved in graph $\hat H$. As cluster $C$ undergoes a sequence of update operations, the neighborhood covers $\cset_i$ evolve, which in turn leads to changes in the contracted graph $\hat H$. However, we ensure that all changes to the neighborhood covers $\cset_i$ are only of the types allowed by
\Cref{thm: NC}, namely: (i) delete an edge from a cluster of $\cset_i$; (ii) delete an isolated vertex from a cluster  of $\cset_i$; or (iii) add a new cluster $C''$ to $\cset_i$, where $C''\subseteq C'$ for some cluster $C'\in \cset_i$. We are then guaranteed that all resulting changes to graph $\hat H$ can be implemented via allowed update operations: namely edge deletions, isolated vertex deletions, and supernode splitting.

We construct two data structures. First, an \EST $\tau$, in the graph obtained from $C$ by adding a new source vertex $s^*$, that connects to every vertex in $S$ with a length-$1$ edge. The depth of the tree is $O(D\poly\log N)$. This data structure allows us to ensure that every vertex of $C$ is sufficiently close to some vertex of $S$, and, when this is no longer the case, to raise the flag $F_C$, and to supply two vertices $x,y\in V(C)$ that are sufficiently far from each other.

The second data structure is obtained by applying the algorithm for the \maintaincluster problem recursively to the contracted graph $\hat H$. This data structure allows us to ensure that all vertices of $S$ are sufficiently close to each other, and, when this is no longer the case, it supplies a pair of vertices $s,s'\in S$, that are sufficiently far from each other in $\hat H$, and hence in $C$. Since we only use this algorithm in the scenario where $|E'|\leq (N(C))^{1-\eps}$, we are guaranteed that $|S|\leq (N(C))^{1-\eps}$, so graph $\hat H$ is significantly smaller than $C$.

To summarize, in order to solve the \maintaincluster problem in graph $C$, we use an expander-based approach, as long as the size of the pseudocut $E'$ that our algorithm computes is above $(N(C))^{1-\eps}$. Once this is no longer the case, we recursively solve the problem on clusters that are added to the neighborhood covers $\cset_i$ of graph $H=C\setminus E'$, for $1\leq i\leq \ceil{\log D}$. 
This allows us to maintain the neighborhood covers $\set{\cset_i}$, which, in turn, allow us to maintain the contracted graph $\hat H$. We then solve the \maintaincluster problem recursively on the contracted graph $\hat H$.
Once all edges of $E'$ are deleted from $C$, we start the whole algorithm from scratch. Since we ensure that the diameter of $C$ is bounded by $D'$, from the definition of a balanced pseudocut, we are guaranteed that $N(C)$ has decreased by at least a factor $N^{\eps}$.

\paragraph{Directions for future improvements.}
A major remaining open question is whether we can obtain an algorithm for decremental \APSP with a significantly better approximation factor, while preserving the near-linear total update time and the near-optimal query time. 
While it seems plausible that the new tools presented in this paper may lead to an improved $(\log m)^{\poly(1/\eps)}$-approximation algorithm with similar running time guarantees, 
%the same total update time  and query time. The fast growth in the approximation factor that we incur occurs due to the algorithm for the \maintaincluster problem, that recursively solves the same problem in the contracted graph $\hat H$, and also recursively solves the \recdynnc problem on graph $C\setminus E'$, where $E'$ is the pseudocut that the algorithm computes. The latter essentially boils down to recursively solving the \maintaincluster problem on smaller and smaller subgraphs. It is this part that we believe can be improved. Intuitively, when recursively solving the \recdynnc problem in graph $C\setminus E'$, the main loss in the approximation factor occurs because, in each one of the $O(1/\eps)$ resulting recursive levels, we construct and recursively solve the \maintaincluster problem on a new contracted graph $\hat H$ (in fact we obtain a number of such disjoint contracted graphs, but we can view their union as a single graph; all of these graphs are significantly smaller than $C$). We believe that ``unrolling'' this part of the recursion, and maintaining a single contracted graph over all recursive levels may lead to a $(\log m)^{\poly(1/\eps)}$-approximation, though this seems to be technically challenging. 
improving the approximation factor beyond the $(\log m)^{\poly(1/\eps)}$ barrier seems quite challenging. A necessary first step toward such an improvement is to obtain better approximation algorithms for the decremental \APSP problem on expanders. 
We believe that this is a very interesting problem in its own right, and it is likely that better algorithms for this problem will lead to better deterministic algorithms for basic cut and flow problems, including Minimum Balanced Cut and Sparsest Cut, via the techniques of \cite{detbalanced}. This, however, is not the only barrier to obtaining an  approximation factor below $(\log m)^{\poly(1/\eps)}$ for decremental \APSP in near-linear time. In order to bring the running time of the algorithm for the \recdynnc problem down from $O\left (m^{1+O(\eps)}\cdot \poly(D)\cdot (\log m)^{O(1/\eps^2)}\right )$  to the desired running time of $O\left (m^{1+O(\eps)}\cdot (\log m)^{O(1/\eps^2)}\right )$, we recursively compose instances of \recdynnc with each other. This leads to recursion depth $O(1/\eps)$, and unfortunately the approximation factor accumulates with each recursive level. If the running time of our basic algorithm for \recdynnc (see \Cref{thm: main dynamic NC algorithm}) can be improved to depend linearly instead of cubically on $D$, it seems conceivable that one could use the approach of \cite{BernsteinChechik,Bernstein}, together with Layered Core Decomposition of \cite{APSP-old} in order to avoid this recursion (though it is likely that, in the running time of the resulting algorithm, term $m^{1+O(\eps)}$ will be replaced with $n^{2+O(\eps)}$). 
Lastly, our algorithm for the \maintaincluster problem needs to call to itself recursively on the contracted graph $\hat H$, which again leads to a recursion of depth $O(1/\eps)$, with the approximation factor accumulating at each recursive level. One possible direction for reducing the number of the recursive levels is designing an algorithm for computing a pseudocut $E'$, its corresponding expander $X$, and an embedding of $X$ into the cluster $C$ with a better balance parameter $\rho$  (see \Cref{thm: compute pseudocut and expander}). We believe that obtaining an analogue of \Cref{thm: compute pseudocut and expander} with stronger parameters and faster running time is a problem of independent interest. 



==> arxiv-version-final/prelims-backup.tex <==


\section{Preliminaries}\label{sec: prelims}

\mynote{this is copied from \cite{APSP-previous}, except the "Dynamic Graphs" part that was updated. I'll update the rest of prelims later.}
All logarithms in this paper are to the base of $2$. 
All graphs in this paper are undirected. Graphs may have parallel edges, except for simple graphs, that cannot have them.
Throughout the paper, we use a $\tilde O(\cdot)$ notation to hide multiplicative factors that are polynomial in $\log m$ and $\log n$, where $m$ and $n$ are the number of edges and vertices, respectively, in the initial input graph.

We follow standard graph-theoretic notation.   Given a graph $G=(V,E)$ and two disjoint subsets $A,B$ of its vertices, we denote by $E_G(A,B)$ the set of all edges with one endpoint in $A$ and another in $B$, and by $E_G(A)$ the set of all edges with both endpoints in $A$. We also denote by $\delta_G(A)$ the set of all edges with exactly one endpoint in $A$. For a vertex $v\in V(G)$, we denote by $\delta_G(v)$ the set of all edges incident to $v$ in $G$, and by $\deg_G(v)$ the degree of $v$ in $G$.
We may omit the subscript $G$ when clear from context. Given a subset $S\subseteq V$ of vertices of $G$, we denote by $G[S]$ the subgraph of $G$ induced by $S$.

Given a graph $G$ and a weight function $w: V(G)\rightarrow \reals$ on its vertices, for a subset $V'\subseteq V(G)$ of its vertices, we denote by $W(V')=\sum_{v\in V'}w(v')$ the total weight of all vertices in $V'$. Abusing the notation, for a subgraph $C\subseteq G$, we denote the weight of the subgraph $W(C)=\sum_{v\in V(C)}w(v)$.


Given a graph $G$ with lengths $\ell(e)\geq 0$ on edges $e\in E(G)$, for a pair of vertices $u,v\in V(G)$, we denote by $\dist_G(u,v)$ the \emph{distance} between $u$ and $v$ in $G$, that is, the length of the shortest path between $u$ and $v$ with respect to the edge lengths $\ell(e)$.  For a pair $S,T$ of subsets of vertices of $G$, we define the distance between $S$ and $T$ to be $\dist_G(S,T)=\min_{s\in S,t\in T}\dist_G(s,t)$.
For a vertex $v\in V(G)$, and a vertex subset $S\subseteq V(G)$, we also define the distance between $v$ and $S$ as $\dist_G(v,S)=\min_{u\in S}\dist_G(v,u)$.
 The \emph{diameter} of the graph $G$, denoted by $\diam(G)$, is the maximum distance between any pair of vertices in $G$. For a path $P$ in $G$, we denote its length by $\ell_G(P)=\sum_{e\in E(P)}\ell(e)$.
 For a vertex $v\in V(G)$ and a distance parameter $D\geq 0$, we denote by $B_G(v,D)=\set{u\in V(G)\mid \dist_G(u,v)\leq D}$ the \emph{ball of radius $D$ around $v$}.
Similarly, for a vertex subset $S\subseteq V(G)$, we let the ball of radius $D$ around $S$ be $B_G(S,D)=\set{u\in V(G)\mid \dist_G(u,S)\leq D}$.
 We will sometimes omit the subscript $G$ when clear from context.

Given a graph $G$ with length $\ell(e)$ on its edges $e\in E(G)$, we may sometimes consider subgraphs $H\subseteq G$, or graphs that are derived from $G$ in some fashion, that also have lengths $\ell(e)$ on edges. In such cases, for clarity of exposition, we will sometimes denote by $\ell_G(e)$ the length of edge $e$ in graph $G$, and by $\ell_H(G)$ the length of edge $e$ in graph $H$. When the graph we are discussing is unambiguously clear, we will omit the corresponding subscripts.


\paragraph{Neighborhood Covers.}
Neighborhood Cover is a central notion that we use throughout the paper. We use both a strong and a weak notion of neighborhood covers, that are defined as follows.

\begin{definition}[Neighborhood Cover]
	Let $G$ be a graph with lengths $\ell(e)>0$ on edges $e\in E(G)$, let $S\subseteq V(G)$ be a subset of its vertices, and let $D\leq D'$ be two distance parameters. A \emph{weak $(D,D')$-neighborhood cover} for vertex set $S$ in $G$ is a collection $\cset=\set{C_1,\ldots,C_r}$ of vertex-induced subgraphs of $G$ called \emph{clusters}, such that:
	
	\begin{itemize}
%		\item for all $1\leq i\leq r$, $C_i$ is a vertex-induced subgraph of $H$;
		\item for every vertex $v\in S$, there is some index $1\leq i\leq r$ with $B_G(v,D)\subseteq V(C_i)$; and
		\item for all $1\leq i\leq r$, for every pair $s,s'\in S\cap V(C_i)$ of vertices, $\dist_{G}(s,s')\leq D'$.
	\end{itemize} 
	A set $\cset$ of subgraphs of $G$ is a \emph{strong $(D,D')$-neighborhood cover} for vertex set $S$ if it is a weak $(D,D')$-neighborhood cover for $S$, and, additionally, for every cluster $C\in \cset$, for every pair $s,s'\in S\cap V(C)$ of vertices, $\dist_{C}(s,s')\leq D'$.
	
	If the vertex set $S$ is not specified, then we assume that $S=V(G)$.
\end{definition}



\iffalse
\mynote{probably not needed}
\paragraph{Decremental Connectivity/Spanning Forest.}
We use the results of~\cite{dynamic-connectivity}, who provide a deterministic data structure, that we denote by $\CONNSF(G)$, that, given an $n$-vertex unweighted undirected graph $G$, that is subject to edge deletions, maintains a spanning forest of $G$, with total update time $O((m+n)\log^2n)$, where $m$ is the number of edges in the initial graph $G$. Moreover, the data structure supports connectivity queries $\conn(G,u,v)$: given a pair  $u,v$ of vertices of $G$, return ``yes'' if $u$ and $v$ are connected in $G$, and ``no'' otherwise. The running time to respond to each such query is  $O(\log n/\log\log n)$. 
%Since the data structure maintains a spanning forest of $G$, we can also use it to respond to a query $\path(G,u,v)$: given two vertices $u$ and $v$ in $G$, return any simple path connecting $u$ to $v$ in $G$ if such a path exists, and return $\emptyset$ otherwise. If $u$ and $v$ belong to the same connected component $C$ of $G$, then the running time of the query is $O(|V(C)|)$.
\fi

\paragraph{Dynamic Graphs.}
Throughout, we consider a graph $G$ that undergoes an online sequence $\Sigma=(\sigma_1,\sigma_2,\ldots)$ of update operations. For now it may be convenient to think of the update operations being edge deletions, though we will consider additional update operations later. After each update operation (e.g. edge deletion), our algorithm will perform some updates to the data structure. 
We refer to different ``times'' during the algorithm's execution. We refer to time 0 as the time at which the data structures of the algorithm have been initialized, but no updates from $\Sigma$ have yet occurred. For each $\tau\geq 0$, we refer to ``time $\tau$ in the algorithm's execution'' as the time immediately after all updates to the data structures maintained by the algorithm following the $\tau$th update $\sigma_{\tau}\in \Sigma$ are completed. When we say that some property holds at every time in the algorithm's execution, we mean that the property holds at all times $\tau$ of the algorithm's execution, but it may not hold, for example, during the procedure that updates the data structures maintained by the algorithm, following some input update operation $\sigma_{\tau}\in \Sigma$.
For $\tau\geq 0$, we denote by $G\attime$ the graph $G$ at time $\tau$; that is, $G^0$ is the original graph, and for $\tau\geq 0$, $G^{\tau}$ is the graph obtained from $G$ after the first $\tau$ update operations $\sigma_1,\ldots,\sigma_{\tau}$. Lastly, the \emph{time horizon} $\tset=\set{0,1,\ldots,|\Sigma|}$ is the time interval from the beginning of the algorithm, and until all updates in $\Sigma$ have been processed.



\paragraph{Other Dynamic Objects}
Consider an algorithm that is applied to some dynamic graph $G$, with time horizon $\tset$. Suppose we define a dynamic set $S\subseteq V(G)$ of vertices, that may change over time. We assume that the set $S$ of vertices is initialized at some time $\tau\in \tset$, and undergoes changes afterwards, during which vertices may be added to or removed from $S$. We say that the set $S$ of vertices is \emph{decremental}, if, once the set $S$ of vertices is initialized at time $\tau$, vertices may leave it, but no new vertices may join it. We say that the set $S$ of vertices is \emph{incremental}, if, once $S$ is initialized at time $\tau$, vertices may join it, but they may not leave it. We may also consider other dynamic collections of objects, for which the notion of decremental or incremental collection is defined similarly.



\paragraph{Even-Shiloach Trees~\cite{EvenS,Dinitz,HenzingerKing}.}
Suppose we are given a graph $G=(V,E)$ with integral lengths $\ell(e)\geq 1$ on its edges $e\in E$, a source $s$, and a distance bound $D\geq 1$. Even-Shiloach Tree (\EST) algorithm maintains, for every vertex $v$ with $\dist_G(s,v)\leq D$, the distance $\dist_G(s,v)$, under the deletion of edges from $G$. Moreover, it maintains a shortest-path tree $\tau$ rooted at vertex $s$, that includes all vertices $v$ with $\dist_G(s,v)\leq D$. We denote the corresponding data structure by $\EST(G,s,D)$. %When the distance bound $D$ is unbounded (that is, $D=nL$, where $L=\max_{e\in E}\set{\ell(e)}$), then we denote the data structure by $\EST(G,s)$.
The total running time of the algorithm, including the initialization and all edge deletions, is $O(m\cdot D\log n)$, where $m$ is the initial number of edges in $G$ and $n=|V|$. Throughout this paper, we refer to the corresponding data structure as \emph{basic \EST}. We later define a slight generalization of this data structure that allows us to handle some additional update operations. This more general data structure will be referred to as \emph{generalized \EST}.

\paragraph{Cuts, Sparsity and Expanders.}
Given a graph $G$, a \emph{cut} in $G$ is a bipartition $(A,B)$ of the set $V(G)$ of its vertices, with $A,B\neq \emptyset$. The \emph{sparsity} of the cut $(A,B)$ is $\phi_G(A,B)=\frac{|E_G(A,B)|}{\min \set{|A|,|B|}}$. We denote by $\Phi(G)$ the smallest sparsity of any cut in $G$, and we refer to $\Phi(G)$ as the \emph{expansion} of $G$.

\begin{definition}[Expander]
	We say that a graph $G$ is a $\phi$-expander iff $\Phi(G)\geq \phi$.
\end{definition}

We will repeatedly use the following standard observation, whose proof is included in Section \ref{subsec: short paths in expanders} of Appendix for completeness.
\begin{observation}\label{obs: short paths in exp}
	Let $G$ be an $n$-vertex $\phi$-expander with maximum vertex degree at most $\Delta$. Then for any pair $u,v$ of vertices of $G$, there is a path connecting $u$ to $v$ that contains at most $\frac{8\Delta \log n}{\phi}$ edges.
\end{observation}



\paragraph{Expander Pruning.}

We use an algorithm for expander pruning by \cite{expander-pruning}. We slightly rephrase it so it is defined in terms of graph expansion, instead of conductance that was used in the original paper. For completeness, we include the proof in Section \ref{subsec: expander pruning} of Appendix.





\begin{theorem}[Adaptation of Theorem 1.3 in~\cite{expander-pruning}]\label{thm: expander pruning}
	There is a deterministic algorithm, that, given an access to the adjacency list of a graph $G=(V,E)$ that is a $\phi$-expander, for some parameter $0<\phi<1$, such that the maximum vertex degree in $G$ is at most $\Delta$, and a sequence $\Sigma=(e_1,e_2,\ldots,e_k)$ of $ {k\leq \phi |E|/(10\Delta)}$ online edge deletions from $G$, maintains a vertex set $S\subseteq V$ with the following properties. Let $G^i$ denote the graph $G\setminus\set{e_1,\ldots,e_i}$; let $S_0=\emptyset$ be the set $S$ at the beginning of the algorithm, and for all $0<i\leq k$, let $S_i$ be the set $S$ after the deletion of the edges of $e_1,\ldots,e_i$ from graph $G$. Then, for all $1\leq i\leq k$:
	
	\begin{itemize}
		\item $S_{i-1}\subseteq S_i$;
		\item $ |S_i|\leq 8i\Delta/\phi$;
		\item $|E(S_i,V\setminus S_i)|\leq 4i$; and
		\item graph $G^i[V\setminus S_i]$ is a $\phi/(6\Delta)$-expander.
	\end{itemize}
	
	The total running time of the algorithm is $\Otilde(k\Delta^2/\phi^2)$.
\end{theorem}





==> arxiv-version-final/proccut.tex <==
\newpage

\subsubsection{Procedure \proccut}
\label{subsubsec: proccut}


Consider the current cluster $C$, and let $x$ be a regular vertex of $C$. 
The procedure runs Dijkstra's algorithm (or weighted BFS) from vertex $x$ in graph $C$, up to a certain depth $D^*$, that will be determined later. 

Recall that Dijkstra's algorithm maintains a set $S$ of ``discovered'' vertices of $C$, where at the beginning $S=\set{x}$. Throughout the algorithm, for every vertex $y\in S$, we maintain the distance $\dist_C(x,y)$, and a neighbor vertex $a_y$ of $y$ that does not lie in $S$, and minimizes the length of the edge $(y,a_y)$. In every iteration, we select a vertex $y\in S$, for which $\dist_C(x,y)+\ell(y,a_y)$ is minimized, and add vertex $a_y$ to $S$. We are then guaranteed that $\dist_C(x,a_y)=\dist_C(x,y)+\ell(y,a_y)$. 
Assume that we are given, for every vertex $y\in V(C)$, a list $\lambda(y)$ of its neighbors $a$, sorted according to the length $\ell(a,y)$ of the corresponding edge, from smallest to largest. Then Dijkstra's algorithm can be implemented so that, if $S_i$ is the set $S$ after the $i$th iteration, then the total running time of the algorithm up to and including iteration $i$ is $O(E(S_i))$. In order to do so, we maintain, for every vertex $y\in V(G)$, a pointer $p_y$ to the vertex $a_y$ on the list $\lambda(y)$. We also maintain a heap of vertices in set $\set{a_y\mid y\in S}$, whose key is $\dist_G(x,y)+\ell(y,a_y)$. In every iteration, we select a vertex $a=a_y$ from the top of the heap, add it to $S$, and then advance the pointer $p_y$ until the first vertex that does not lie in $S$ is encountered (if vertex $a$ that was added to $S$ serves as vertex $a_y$ for several vertices $y\in S$, we advance the pointer $p_y$ for each such vertex $y$). We also initialize pointer $p_a$. 

For all $z\geq 0$, we denote by $L_z$ the set of all vertices of $C$ that lie at distance $2(z-1)D+1$ to $2zD$ from $x$ in $C$. In other words:

\[L_z=B_C(x,2zD)\setminus B_C(x,2(z-1)D).   \]

We refer to the vertices of $L_j$ as \emph{layer $i$ of the BFS}. We denote by $W_z$ the total number of regular vertices in $L_0\cup L_1\cup\cdots\cup L_z$, and by $m_z$ the total number of edges $e\in E(C)$, such that both endpoints of $e$ lie in $L_0\cup L_1\cup\cdots\cup L_z$. The following definition is crucial for the description of Procedure \proccut.

\begin{definition}[Eligible Layer]
	Let $z>1$ be an integer, and let $i\geq 0$ be an integer for which $N^{1-1/2^i}\leq N_z<N^{1-1/2^{i+1}}$ holds. For all $q'<i\leq q$, and $0\leq j\leq r+2$, let $W^{i,j}_z$ be the total number of regular vertices $x\in T^i_j$ that lie in  $L_0\cup L_1\cup\cdots\cup L_z$, and similarly, let $W^{i,j}_{z+1}$ be the total number of regular vertices $x\in T^i_j$ that lie in  $L_0\cup L_1\cup\cdots\cup L_{z-1}$ . We say that layer $L_z$ of the BFS is \emph{eligible}, if the following conditions hold:
	
	\begin{properties}{C}
		\item $i>q'$;  \label{cut condition 1: not too small}
		\item $m_z\leq m_{z-1}\cdot \hat W^{\eps}$; and
		\item for all $0\leq j\leq r+2$, $W^{i,j}_z\leq W^{i,j}_{z-1}\cdot N^{\eps\cdot 2^{i-4}}$.
	\end{properties}
\end{definition}



We need the following claim, whose proof uses standard arguments and appears in Section \ref{subsec: proof of proccut eligible layer} of Appendix.
\begin{claim}\label{claim: eligible layer}
	If the total number of regula vertices in $B_C (x, ??\cdot D )$ is at most $N/2^{q'}$, then there is some eligible layer $L_z$ with $1<i<  ??$.
\end{claim}


We are now ready to describe the algorithm for \proccut.
The input to the procedure is a cluster $C\in \cset$, a vertex $x\in V(C)$, and a distance threshold $D>0$. We assume that we are given, for every vertex $y\in V(C)$, a list $\lambda(y)$ of its neighbors $a$ in $C$, sorted according to the length $\ell(a,y)$ of the corresponding edge, from smallest to largest.
The procedure runs Dijkstra's algorithm from the input vertex $x$ in graph $C$, until it encounters the first layer $L_i$, such that either $\sum_{i'\leq i}\tW_{i'}> \tW(C)/2$, or $L_i$ is an eligible layer. In the former case, the algorithm outputs FAIL. In the latter case, it computes two new clusters: cluster $C'$ is the subgraph of $H$ induced by vertex set $L_1\cup\cdots\cup L_{i}$. Cluster $C''$ is obtained from cluster $C$ by deleting all vertices in $L_1\cup \cdots L_{i-1}$ from it. 
The algorithm outputs cluster $C'$ explicitly, by listing all its vertics and edges, and it outputs cluster $C''$ implicitly, by listing the edges and the vertices of $C\setminus C''$.
Notice that vertices of $L_i$, and edges that connect them, belong to both $C'$ and $C''$.
The following observation immediately follows from Claim \ref{claim: eligible layer} and the definition of a layer.

\begin{observation}\label{obs: diam of cut off cluster}
	If Procedure $\proccut(C,x,D)$ does not return FAIL, then it produces two clusters $C',C''$, with $W(C')\leq W(C)/2$, and $\diam(C')\leq 512D\log^4W$. Moreover, $V(C')\subseteq B_C(x,256D\log^4W)$.
\end{observation}

Next, we establish that the two new clusters $C',C''$ contain a $D$-neighborhood every vertex of $C$ in the following claim, whose proof appears in Section \ref{subsec: proof of maintain neighborhood cover} of Appendix.

\begin{claim}\label{claim: cut gives valid neighborhood cover}
	Assume that Procedure $\proccut(C,x,D)$ produces two clusters $C'$ and $C''$. Then for every vertex $y\in V(C)$, either $B_C(y,D)\subseteq V(C')$ or $B_C(y,D)\subseteq V(C'')$ must hold.
\end{claim} 

We view Procedure \proccut as creating a new cluster $C'$ that is split off of the cluster $C$; recall that $\tW(C')\leq \tW(C)/2$ must hold. We then update the cluster $C$, by setting $C= C''$.
Notice that the running time of the procedure is $O(|E(C')|)\leq O(W(C')\mu)$. %This is since for every regular vertex $v$, the total number of edges that belonged to $H$ over the course of the algorithm and were incident to $v$ is bounded by $w(v)\cdot \mu$.  We note that Procedure \proccut does not compute the cluster $C''$ explicitly, and instead it produces a set of edges and vertices that need to be deleted from $C$ to ensure that $C=C''$ holds.
%We will apply Procedure \proccut to clusters $C$ that lie in the current cluster set $\cset$. If the outcome of the procedure is two clusters $C'$ and $C''$, then we add $C'$ to $\cset$, and we update the cluster $C$ in $\cset$ by deleting edges and vertices from it so that $C=C''$ holds.

Lastly, we prove the following lemma, that is central to bounding the number of clusters that a regular vertex may belong to.
The proof appears in \Cref{subsec: proving bound on budgets} of Appendix.

\begin{lemma}\label{lem: change in budget after proccut}
	Assume that Procedure $\proccut(C,x,D)$, when applied to a cluster $C\in \cset$, produced two clusters $C'$, $C''$, and assume that cluster set $\cset$ was updated accordingly. Denote by $\beta$ and $\beta'$ the total budget of all vertices in $V(H)$ at the beginning and at the end of the procedure, respectively. For all $1\leq j\leq r$, let $\beta_{\geq j}$ and $\beta'_{\geq j}$ denote the total budget of all vertices in $S_{\geq j}$ at the beginning and at the end of the procedure, respectively, and let $\tW'_j$ be the total weight of new regular vertices that join class $S_j$ at the end of the procedure. Then $\beta'\leq \beta$, and moreover, for all $1\leq j\leq r$, $\beta_{\geq j}'\leq \beta_{\geq j}+2^{j}(1+1/\log W) \tW'_j$.
\end{lemma}

==> arxiv-version-final/pseudocut-DS.tex <==
\newpage
\subsubsection{Data Structures}

We now describe the data structures that our algorithm maintains.


\paragraph{Graph $\tilde H$.}
As described already, our algorithm maintains the graph $\tilde H$. Once the graph is initialized at the beginning of the algorithm, it undergoes a sequence $\tilde \Sigma$ of online valid update operations, that coresponds to the sequence $\Sigma$ of valid update operations that input graph $H$ undergoes. We call all updates in $\tilde \Sigma$ \emph{primary} updates. Additionally, whenever the algorithm is asked to process query \maxrouting, the algorithm that responds to the query may delete a collection of at most $\frac{|T|(\mu+D^*)}{\eta}$ edges. Once the query is processed, all edges that were deleted while processing the query, are inserted back into graph $\tilde H$. We view these edge-deletion and edge-insertion operations as part of the update sequence for graph $\tilde H$, but we refer to them as \emph{secondary} updates. Note that edge-insertion (which is not a valid update operation) is allowed as a secondary update.


\paragraph{Graphs $C\in \cset$ and Emulators}
Consider now the graphs $C\in \cset$. As graph $\tH$ undergoes the sequence $\tilde \Sigma$ of valid update operations, we update every cluster $C\in \cset$ accordingly. Specifically, if an edge $e$ is deleted from $\tH$ via $\tilde \Sigma$, then for every cluster $C\in \cset$ containing edge $e$, we delete $e$ from $C$ as well. If an isolated vertex $x$ is deleted from graph $\tH$, then, for every cluster $C\in \cset$ containing $x$, we delete $x$ from $C$ as well. Lastly, assume that a supernode-splitting operation was applied to supernode $u$ in graph $\tH$ with the set $E'$ of edges. We consider every cluster $C\in \cset$ containing supernode $u$. If at least one edge of $E'$ belongs to $C$, then we perform a supernode-splitting operation in cluster $C$, with supernode $u$, and the set $E'\cap E(C)$ of edges. 

We ignore for now the secondary update operations that graph $\tilde H$ undergoes, and assume that it only undergoes the sequence $\tilde \Sigma$ of valid update operations (primary updates). We need the following simple observation.

\begin{observation}\label{obs: containment of balls overtime}
	For every time $\tau$ during the time horizon, for every regular vertex $v$ of $\tH\attime$, there is a cluster $C\in \cset$, with $B_{\tH\attime}(x,D^*)\subseteq V(C\attime)$.
\end{observation}
\begin{proof}
	Let $v$ be any regular vertex that belongs to graph $\tH$ at the beginning of the algorithm (recall that regular vertices may not be inserted into $\tH$). From \Cref{claim: cutting tilde H}, there is some cluster $C\in \cset$, with $B_{\tH\attime[0]}(v,D^*)\subseteq V(C^0)$. We denote by $G$ the dynamic graph, that is the subgraph of $\tilde H$, induced by $B_{\tH}(v,D^*)$. 
	We also denote by $\tilde G$ the dynamic graph, that is the subgraph of $C$, induced by $B_{C}(v,D^*)$.
	Since $C$ is a vertex-induced subgraph of $\tH$, $G\attime[0]= \tilde G\attime[0]$ holds. From our definition of updates to clusters of $\cset$, it is easy to verify that, whenever graph $G$ undergoes any update, graph $\tilde G$ undergoes an identical update, and vice versa. Therefore, at all times $\tau$, $G\attime=\tilde G\attime$ holds, and $B_{\tH\attime}(x,D^*)\subseteq V(C\attime)$.
\end{proof}

Consider now some cluster $C\in \cset$.  We denote by $N^0(C)$ the number of regular vertices that lie in cluster $C$ at the beginning of the algorithm. From \Cref{claim: cutting tilde H},   $N^0(C)\leq \frac{W^{1-2\eps}}{64\mu}$. Cluster $C$ then undergoes a sequence of valid update operations that we denote by $\Sigma(C)$, whose dynamic degree bound is at most $\mu$ (since the dynamic degree bound of $(\tilde H,\tilde \Sigma)$ is at most $\mu$. Therefore, the total number of vertices that are ever present in cluster $C$ is at most $2N^0(C)\mu$, and the total number of edges that are ever present in $C$ is at most $N^0(C)\cdot \mu$. From \Cref{lem: vertex splitting to fully dynamic}, by using a collection of spare vertices, we can maintain a cluster $\tilde C$, that is identical to $C$, except that it may contain additional isolated vertices. Once cluster $\tilde C$ is initialized, it only undergoes edge-deletion and edge-insertion updates. The number of vertices in $\tilde C$ is at most  $2N^0(C)\mu$, and the number of edges that are ever present in $\tilde C$ is at most $N^0(C)\mu$. We denote the update sequence for $\tilde C$ by $\tilde \Sigma(C)$, and we denote $m(C)=3N^0(C)\mu$. From our discussion,
$|V(\tilde C)|+|E(\tilde C\attime[0])|+|\tilde \Sigma(C)|\leq m(C)$, and $m(C)\leq \frac{W^{1-2\eps}}{64}$.

Intuitively, we would like to apply the algorithm from \Cref{cor: T-emulator} to graph $\tilde C$, together with the set $F(C)=V(C)\cap F$ of terminals, in order to maintain an $F(C)$-emulator for graph $C$. However, this may be wasteful, since the running time of the algorithm may be as high as roughly $\Omega(W)$, while it is possible that $N^0(C)\ll W$. As an example, it is possible that set $\cset$ contains a very large number of clusters, each of which contains very few regular vertices, and so we cannot afford spending time $\Omega(W)$ on maintaining an emulator for each such cluster. In order to overcome this difficulty, we will group these clusters into larger graphs, in which the number of regular vertices is close to $W$, by simply taking a disjoint union of small clusters. The resulting collection of graphs will be relatively small, and we will be able to apply the algorithm from \Cref{cor: T-emulator} to each such graph.

Specifically, at the beginning of the algorithm, we construct a new collection $\gset$ of graphs, as follows. We start with $\gset=\set{\tilde C\mid C\in \cset}$, and then iterate. While there is a pair $G,G'\in \gset$ of graphs, with $m(G)+m(G')\leq \frac{W^{1-2\eps}}{64}$, We delete graphs $G$ and $G'$ from $\gset$, and instead we add a new graph $G''$, that is a disjoint union of $G$ and $G'$. We then set $m(G'')=m(G)+m(G')$. We note that it is possible that, for some vertex $x\in V(\tilde H)$, graphs $G$ and $G'$ both contain a copy of this vertex. We view these different copies of $x$ as different vertices. Notice that, when the algorithm terminates, we are guaranteed that for every graph $G\in \gset$, $m(G)\leq \frac{W^{1-2\eps}}{64}$ holds, and there is at most one graph $G\in \gset$ with $m(G)\leq \frac{W^{1-2\eps}}{128}$.

Recall that, from \Cref{claim: cutting tilde H},  $\sum_{C\in \cset}N^0(C)\leq (W'\cdot \mu)^{1+\eps}$. Therefore: 


\[\begin{split}
\sum_{C\in \cset}m(C)&=\sum_{C\in \cset}3N^0(C)\cdot \mu\\
&\leq 3(W')^{1+\eps}\mu^{2+\eps}\\
&\leq \frac{3\left(\rho\cdot W^{1-2\eps}\right )^{1+\eps}\cdot \mu^{2+\eps}}{(128\mu)^{1+\eps}} \\
&\leq W^{1-\eps}\mu\rho^{1+\eps}.
\end{split}
\]

(we have used the fact that 
$\frac{W'}{\rho}\leq \frac{W^{1-2\eps}}{128\mu}$).


Altogether, we get that:

\[
\begin{split}
|\gset|& \leq \frac{\sum_{C\in \cset}m(C)}{W^{1-2\eps}/64}\\
&\leq \frac{64W^{1-\eps}\mu\rho^{1+\eps}}{W^{1-2\eps}}\\
&\leq 64W^{\eps}\mu\rho^2.
\end{split}\]


Consider now any graph $G\in \gset$. From our construction, there is some subset $\cset_G\subseteq \cset$ of clusters, such that graph $G$ is a disjoint union of all clusters in set $\tilde \cset(G)=\set{\tilde C\mid C\in \cset_G}$. Recall that every cluster $\tilde C\in \tilde \cset_G$ undergoes an online sequence $\tilde \Sigma(C)$ of edge insertions and deletions. Whenever any such update is applied to any cluster $\tilde C\in\tilde \cset_G$,  we update graph $G$ accordingly. We denote by $\Sigma(G)$ the resulting online sequence of edge-insertions and edge-deletions that graph $G$ undergoes. Observe that:

\[|V(G)|+|E(G\attime[0])|+|\Sigma(G)|=\sum_{\tilde C\in \tilde \cset_G}\left(|V(\tilde C)|+|E(\tilde C\attime[0])|+|\tilde \Sigma(C)|\right )=\sum_{\tilde C\in \tilde \cset_G} m(C)=m(G)\leq \frac{W^{1-2\eps}}{64}. \]




As mentioned already, whenever a \maxrouting query arrives, the algorithm for responding to the query may delete a collection $E'$ of up to $\frac{|T| D^*\alpha'}{\eta}$ edges from graph $\tilde H$. Once the query is answered, all edges of $E'$ are inserted back into $\tilde H$. Recall that we have called such updates to graph $\tilde H$ \emph{secondary}. Whenever an edge $e$ is deleted from graph $\tilde H$ via a secondary update, for every cluster $C\in \cset$ with $e\in E( C)$, we delete edge $e$ from cluster $C$ and from $\tilde C$. Similarly, when such an edge $e$ is inserted back into $\tilde H$, we insert it back into $C$ and into $\tilde C$. 
If $G\in \gset$ is a graph that contains $\tilde C$, then graph $G$ is updated similarly. Notice that, from \Cref{claim: cutting tilde H}, every regular vertex $v\in V(\tH\attime[0])$ belongs to at most $\frac{4\cdot(W'\mu)^{2\eps}}{\eps}$ graphs in $\cset$. Therefore, for every edge $e\in E(\tilde H)$, at most $\frac{4\cdot(W'\mu)^{2\eps}}{\eps}$ copies of $e$ may exist in the clusters of $\cset$. Therefore, for a fixed graph $G\in \gset$, over the course of the procedure that responds to a single \maxrouting query, in total, the total number of edges that may be deleted from $G$ is bounded by: 

\[\frac{4|T|\cdot D^*\cdot\alpha'\cdot(W'\mu)^{2\eps}}{\eta\eps}\leq \frac{4|T|\cdot D^*\alpha'\cdot W^{2\eps}\cdot \rho^{2\eps}}{\eta\eps}\]


(since $\frac{W'}{\rho}\leq \frac{W^{1-2\eps}}{128\mu}$)


may allow up to $\frac{W^{1-2\eps}}{64}$ edge deletions. Single query: 
$\frac{4|T|\cdot D^*\alpha'\cdot W^{2\eps}\cdot \rho^{2\eps}}{\eta\eps}$ edge deletions. So number of queries bounded by:

\[ \frac{W^{1-4\eps}\eta\eps}{256|T|\cdot D^*\alpha'\cdot  \rho^{2\eps} }\]


\mynote{figure out how much $\eta$ is? that depends on how many edges we are allowed to delete when trying to improve the pseudocut. (fix the $\alpha'$ parameter, the constant in it?). Then assume that $\mu\leq W^{\eps}$. Not clear if we can assume anything on $\rho$? But maybe for sure $\rho\leq W$, so we can get rid of stuff like $\rho^{2\eps}$. Do we want to assume that $W^{\eps}<1/\eps$? does it follow from $\eps>1/(\log W)^{1/4}$? or should we make a stronger assumption? Restricted emulator: parameter $D^*$ will need to be replaced with $\alpha'\cdot D^*$, because we need to ensure that when we can't route anymore, the distance is at least $D^*$. Does this mean that we need a gap of $\alpha'$ between $D^*$ and $\hat D$? maybe replace one direction with $2^{1/\eps}$?}




To get a distancing, we need either congestion >$D^*$, or route less than $1/D^*$-fraction of guys. Latter is forbidden in the distanced-matching game. So congestion $>D^*$. Want roughly $\frac{W^{1-2\eps}}{128|T|\mu D^*}$ iterations.


We denote by $\tilde \Sigma'(C)$ the update sequence to cluster $\tilde C$ that includes both primary and secondary updates, and we denote $m(C)=|V(\tilde C)|+|E(\tilde C\attime[0])|+|\tilde \Sigma'(C)|$. From the above discussion, $m\leq \frac{W^{1-2\eps}}{16}$ holds, and so particular, $m^{1+2\eps}<\frac{W}{8}$. 
We let $W(C)\leq W$ be the smallest integer for which 
Denote $F(C)=V(C)\cap F$. Since  $\frac{1}{(\log W)^{1/4}}<\eps<1$, and $D^*$ is an integral power of $2$, we have now received a valid input to the $W$-bounded \maintainemulator problem, where the set of terminals associated with the problem is $F(C)$ (see \Cref{dec: maintainemulator problem}). Since we have made Assumption \ref{assumption: alg for recdynnc}, we can now apply the algorithm from \Cref{cor: T-emulator} for the \maintainemulator problem on this input. Recall that the algorithm achives stretch $\alpha'=(\alpha(W))^{O(1/\eps)}$, and has total update time at most $O\left (W^{1+O(\delta)+O(\eps)}\cdot (\Delta(W)\cdot\log W)^{O(1/\eps^2)}\right )$, where $\delta$ is the parameter from \Cref{assumption: alg for recdynnc}. We denote the $F(C)$-emulator that the algorithm maintains by $R_C$.

The algorithm also ensures that, at all times, $|V(R_C)|\leq |F(C)|\cdot \left(\Delta(W)\log W\right )^{O(1/\eps)}$ holds.
Recall that the emulator graph $R_C$, after it is initialized, undergoes a sequence of edge-deletion, edge-insertion, isolated vertex-deletion and vertex-splitting updates. Moreover, if $\tset'$ is any time interval during which update sequence $\tilde \Sigma'(C)$ to graph $\tilde C$ is decremental, then, during $\tset'$, graph $R_C$ may only undergo edge-deletion, isolated vertex-deletion, and vertex-splitting updates. Furthermore, the total number of edges that are ever present in $H$ during $\tset'$ is at most $|F(C)|\cdot \left(\Delta(W)\log W\right )^{O(1/\eps)}$. This will be useful for us since, during the procedure that responds to a \maxrouting query, we only perform edge-deletions in graph $C$ and hence $\tilde C$. Therefore, throughout the duration of the procedure, the emulator $R_C$ may only undergo edge-deletion, edge-insertion, isolated vertex-deletion and vertex-splitting updates. This will allow us to use modified \EST data structure in order to respond to \maxrouting query.

This completes the definition of all data structures that our algorithm maintains. We now bound the total update time of these data structures. Consider some cluster $C\in \cset$. As noted already, the total update time of the algorithm from \Cref{cor: T-emulator} for maintaining the emulator $R_C$ for $\tilde C$ is bounded by $|F(C)|\cdot \left(\Delta(W)\log W\right )^{O(1/\eps)}$. The time that is required in order to compute the update sequence $\tilde \Sigma(C)$ given update sequence $\tilde \Sigma$ for graph $\tilde H$ is asymptotically bound by this running time. Therefore, the total update time required to maintain all clusters $C\in\cset$ and the corresponding emulators $R_C$ is bounded by:

\[\sum_{C\in \cset}|F(C)|\cdot \left(\Delta(W)\log W\right )^{O(1/\eps)}.\]

Recall that the total number of fake terminals in graph $\tilde H$ is $|F|\leq |T|\cdot \mu$. Moreover, from \Cref{claim: cutting tilde H}, every fake terminal $\tilde t$ may belong to at most $\frac{4(W'\mu)^{2\eps}}{\eps}$ clusters of $\cset$ at the beginning of the algorithm. 
	
	

==> arxiv-version-final/pseudocut-case1.tex <==

\subsubsection{Special Case: $|T|\geq W^{1-2\eps}/64\mu^2$}




From now on we assume that $|T|<\frac{W^{1-2\eps}}{128\mu^2}$. 
Let $\tset$ be the time horizon that is associated with the update sequence $\Sigma$ for $H$. We now provide a high-level overview of the algorithm.
We start by defining a modified graph $\tH$, that will be more convenient for us to use. Intuitively, graph $\tH$ is obtained from graph $H$ by ``splitting'' every terminal $t\in T$ into a number of ``fake terminals'', that we refer to as \emph{copies of $T$}. We will ensure that, for every pair $t,t'\in T$ of terminals, if there is a short path $P$ connecting $t$ to $t'$ in $H$, such that no inner vertices of $P$ are terminals, then there is a path $P'$ connecting a copy of $t$ ot a copy of $t'$ in $\tH$, of a similar length. However, graph $\tH$ will have one additional useful property: for every regular vertex $v$ of $\tH$, the ball of radius $\tilde D$ around $v$ in $\tH$ only contains a relatively small number of regular vertices (from the definition of a pseudocut, this property holds for graph $H\setminus T$, but it does not necessarily hold for graph $H$). This property will allow us to construct a collection $\hset$ of vertex-induced subgraphs of $\tH$, each of which is relatively small, such that, for every fake terminal $\tilde t$, there is some graph $H'\in \hset$, with $B_{\tH}(\tilde t,  D)$ contained in $H'$. While the graphs in $\hset$ are not necessarily disjoint, we will ensure that their total size is comparable to the size of $\tH$. Since the size of each graph $H'\in \hset$ is sufficiently small, we can now maintain an approximate $F(H')$-emulator of $H'$, where $F(H')$ is the set of fake terminals lying in $H'$, using the algorithm from \Cref{cor: T-emulator}. These are the only data structures that our algorithm maintains. In order to respond to a \maxrouting query between a pair $A,B$ of subsets of the terminals, we combine all resulting emulators into a single graph, whose size is comparable to $|T|$, construct an \EST data structure in the resulting graph, and then use standard path peeling: we iteratively construct a short path connecting a pair $a\in A,b\in B$ of vertices, and then delete from $\tH$ and all graphs in $\hset$ all edges that participate in $\eta$ of the paths that we have constructed so far. Once an approximate maximal routing is computed, all edges that were deleted from graph $\tH$ and the graphs of $\hset$ over the course of the procedure are inserted back into them. We now describe our algorithm formally, starting with the definition of the modified graph $\tH$.



==> arxiv-version-final/pseudocut-embed-inner.tex <==
\newpage






\newpage
\subsection{Proof of \Cref{thm: support maxrouting queries}}
For convenience, we will refer to vertices of $T$ as \emph{terminals}.

\input{pseudocut-case1}
\input{pseudocut-modified}
\input{pseudocut-cutting}
\input{pseudocut-DS}




\newpage





\begin{definition}[$W$-bounded \maintainemulator problem]
	The input to the $W$-bounded \newline \maintainemulator problem is the same as the input to the $W$-bounded \APSP problem: a graph $G$ with integral lengths $\ell(e)\geq 1$ for its edges $e\in E(G)$,
	that undergoes an online sequence $\Sigma$ of edge deletions and insertions,  a precision parameter $\frac{1}{(\log W)^{1/4}}<\eps<1$, and a distance parameter $0<D^*<W$ that is an integral power of $2$, such that, if we denote $|V(G)|+|E(G\attime[0])|+|\Sigma|=m$, then $m^{1+2\eps}<W/8$ holds. Additionally, we are given a subset $T\subseteq V(G)$ of vertices of $G$ called terminals. The goal is to maintain  a $D^*$-restricted $T$-emulator $H$ for graph $G$, with a strech $\alpha'$. Specifically, the algorithm for the $W$-bounded \maintainemulator problem, after initializing the graph $H$, must produce a sequence of online updates to $H$, that only consists of edge-deletion, edge-insertion, isolated vertex-deletion, and vertex-splitting operations. 
	%Further, we require that,  if $\tset'$ is any time interval during which the update sequence $\Sigma$ for $G$ is decremental, then, during $\tset'$, graph $H$ may only undergo edge-deletion, isolated vertex-deletion, and vertex-splitting updates. 
	Lastly, the algorithm must support $\transformpath$ queries: given a path $P$ of length $D$ in graph $H$, that connects a pair $t,t'\in T$ of terminals, it must return a path  $P'$ in graph $G$, connecting $t$ to $t'$, whose length is at most $\alpha'\cdot D$. The query time must be bounded by $O(|E(P)|+|E(P')|)$, where $P$ is the path that the algorithm is given as input, and $P'$ is the path that the algorithm returns.
\end{definition}


\begin{corollary}\label{cor: T-emulator}
	Suppose \Cref{assumption: alg for recdynnc} holds for some parameter $W>0$. Then there is a deterministic algorithm, that we call \algemulator for the $W$-bounded \maintainemulator problem, that achieves stretch $\alpha'=(\alpha(W))^{O(1/\eps)}$, and has total update time at most $O\left (W^{1+O(\delta)+O(\eps)}\cdot (\Delta(W)\cdot\log W)^{O(1/\eps^2)}\right )$, where $\delta$ is the parameter from \Cref{assumption: alg for recdynnc}. The algorithm also ensures that, at all times, $|V(H)|\leq |T|\cdot \left(\Delta(W)\log W\right )^{O(1/\eps)}$ holds, where $H$ is the $T$-emulator that it maintains. Lastly, the algorithm ensures that, if $\tset'$ is any time interval during which the update sequence $\Sigma$ for $G$ is decremental, then, during $\tset'$, graph $H$ may only undergo edge-deletion, isolated vertex-deletion, and vertex-splitting updates. Furthermore, the total number of edges that are ever present in $H$ during $\tset'$ is at most $|T|\cdot \left(\Delta(W)\log W\right )^{O(1/\eps)}$.
\end{corollary}

==> arxiv-version-final/recdynnc-to-maintain-cluster.tex <==
\newpage

\section{Reduction from \recdynnc to \maintaincluster}
\label{sec: reduction from recdynnc to maintain cluster}

The goal of this section is to provide a reduction from the \recdynnc problem to the \maintaincluster problem, that is summarized in the following theorem.


\begin{theorem}\label{thm: recdynnc to maintain cluster}
	Assume that for some parameter $\hat W$, there exists a deterministic algorithm for the \maintaincluster problem, that we denote by \algmaintaincluster. The algorithm, given a valid input structure $\iset=\left(C,\set{\ell(e)}_{e\in E(C)},D \right )$, that undergoes a sequence of valid update operations with dynamic degree bound $\mu$, the number of regular vertices in $C$ at the beginning of the algorithm is at most $\hat W$, achieves approximation factor $\alpha(\hat W)$, and  has total update time $T(N^0(C),\mu,D,\hat W)$. Then there is a deterministic algorithm for the \recdynnc problem, that, given a valid input structure  $\iset=\left(H=(V,U,E),\set{\ell(e)}_{e\in E},D \right )$ undergoing a sequence of valid update operations with dynamic degree bound $\mu$, such that the number of regular vertices in $H$ at the beginning of the algorithm is at most $\hat W$, and a parameter $0<\eps<1$, achieves approximation factor $\alpha(\hat W,\eps)$, and  has total update time $??$. The algorithm also ensures that, for every regular vertex $v\in V$, the total number of clusters in the neighborhood cover $\cset$ that the algorithm maintains, to which vertex $v$ ever belongs over the course of the algorithm, is bounded by $\hat W^{O(\eps)}$.
\end{theorem}

The remainder of this section is dedicated to the proof of \Cref{thm: recdynnc to maintain cluster}. The main tool that we use is an algorithm for managing a single cluster, that we refer to as \algmanagecluster. Whenever a new cluster $C$ is added to the neighborhood cover $\cset$ that we maintain, we initialize the algorithm \algmaintaincluster on $C$. The purpose of the algorithm is to support queries $\spquery(C,v,v')$ between pairs of regular vertices of $C$. Whenever the diameter of cluster $C$ becomes too large (and the queries cannot be supported), the algorithm must split cluster $C$ into two clusters: the algorithm must compute two new clusters $C',C''\subseteq C$, so that $N(C')\leq N(C'')$, and, for every regular vertex $v\in V(C)$, either $B_C(v,D)\subseteq C'$, or $B_C(v,D)\subseteq C''$ holds. Cluster $C'$ is then added to the set $\cset$ of clusers that our algorithm maintains, and Algorithm \algmanagecluster is initialized on $C'$. We also delete vertices and edges from $C$, so that $C=C''$ holds. We say that cluster $C'$ is a \emph{child-cluster} of $C$. In order to ensure that every regular vertex of the input graph $H$ lies in a small number of clusters of $\cset$, we need to ensure that every regular vertex of $C$ lies in a relatively small number of child-clusters of $C$. More specifically, we partition all child-clusters of $C$ into classes, according to the number of regular vertices in each such cluster. We then ensure that for every regular vertex of $C$ belongs to a relatively small number of clusters from each class, where the threshold for each class is chosen appropriately.

In order to implement algorithm \algmanagecluster, we apply the algorithm for the \maintaincluster problem, whose existence is assumed in the statement of \Cref{thm: recdynnc to maintain cluster}, to cluster $C$. Whenever that algorithm raises a flag $F$, providing a pair $v,v'$ of regular vertices of $C$ with $\dist_C(v,v')\geq \Delta(\hat W)\cdot D$, our algorithm must compute a pair $C',C''\subseteq C$ of clusters to be used for cluster-splitting. We then feed to algorithm \algmaintaincluster a sequence of valid update operations (flag lowering sequence), containing all edges of $E(C)\setminus E(C'')$, and all vertices of $V(C)\setminus V(C'')$. From the definition of the \maintaincluster problem, it is enough to ensure that either $B_C(v,\Delta(\hat W)\cdot D/2)\subseteq C''$, or $B_C(v',\Delta(\hat W)\cdot D/2)\subseteq C''$ holds. In the former cases, we are then guaranteed that none of the edges and vertices of $B_C(v,\Delta(\hat W)\cdot D/2)$ are deleted from $C$ as part of the flag-lowering sequence, while int he latter case the same guarantee holds for $B_C(v',\Delta(\hat W)\cdot D/2)$. As mentioned already, the main challenge is to implement the algorithm for cluster-splitting, so that every regular vertex of $C$ lies in a relatively small number of child-clusters of $C$.

We now describe Algorithm \algmanagecluster more formally, and analyze its properties.

\input{manage-cluster}
\input{proccut}

==> arxiv-version-final/stretch-transform-path.tex <==
\subsubsection{Bounding the Stretch, and Supporting $\transformpath$ Queries}
\label{subsubsection: stretch transform path}

In this subsection we complete the proof of \Cref{cor: T-emulator}, by showing that the graph $H$ that our algorithm maintains is indeed a $D^*$-restricted $T$-emulator, and by providing an algorithm to support $\transformpath$ queries. Recall that we denoted by $\alpha=\alpha(W)$ the parameter from \Cref{assumption: alg for recdynnc}. 
We start with the following claim.

\begin{claim}\label{claim: distances preserved in emulator}
	At all times $\tau\in \tset$,  for every pair $x,y\in T$ of terminals, if $\dist_{G\attime}(x,y)\leq D^*$, then  $ \dist_{H\attime}(x,y)\leq \alpha^{O(1/\eps)}\cdot \dist_{G\attime}(x,y)$ holds.
\end{claim}

\begin{proof}
	The proof of the claim uses the following observation, whose proof is deferred to Section \ref{subsec: covering chain importance} of Appendix.
	
\begin{observation}\label{obs: coverning chain importance}
	Let $\tau \in \tset$ be any time during the time horizon, let $x\in V(G)$ be a vertex, and let $J=((L_1,i_1,C_1,x_1),\ldots,(L_r,i_r,C_r,x_r))$  be a valid covering chain for vertex $x$ at time $\tau$. Then for all $1\leq r'<r$, supernode $u^{L_{r'+1}}(C_{r'})$ lies in graph $H^{L_{r'+1}}$, and moreover, it is marked as an important supernode for cluster $C_{r'+1}$.
\end{observation}
	
Consider now some time $\tau\in \tset$, and a pair  $x,y\in T$ of terminals, for which $\dist_{G\attime}(x,y)\leq D^*$ holds. In the remainder of the proof, whenever we refer to dynamic objects or data structures, we refer to them at time $\tau$, unless stated otherwise. Let $P$ be the shortest path connecting $x$ to $y$ in graph $G$. Let $L$ be the level of path $P$, and let $D\leq D^*$ be its length, so $\dist_G(x,y)=D$. Let $i\leq \log D^*$ be the smallest integer, for which $D_i\geq D$ holds, so $D_i\leq 2D$. 
Then from \Cref{claim: short path existence}, at time $\tau$, $R^L_i(x),R^L_i(y)\neq \emptyset$, and there is a path $P'$ in graph $H^L$, connecting a vertex $v^L(x')$, with $x'\in R_i^L(x)$ to a vertex $v^L(y')$, with $y'\in R_i^L(y)$, whose length is at most $2^{10L+4}\cdot D_i$.

From the definition of the set $R_i^L(x)$ of vertices, there is a covering chain: \newline $J=((L_1,i_1,C_1,x_1),\ldots,(L_r,i_r,C_r,x_r))\in \jset^L_i(x)$, such that $x'=x_r$. Recall that $L_r=L$, $L_1=0$, $i_1=i$, and $x_1=x$ must hold. From the definition of a covering quadruple, $C_1=\coveringcluster^0_{i}(x)$ holds, and so, in particular, $v^0(x)\in V(C_1)$. Therefore, vertex $z(C_1)$ lies in graph $H$, and edge $(x,z(C_1))$ of length $2^{\scale(C_1)}=2^i$ also belongs to graph $H$. We now claim that, for all $1< r'\leq r$, vertex $z(C_{r'})$ lies in graph $H$, and it is connected with an edge of length $2^{i_{r'}}$ to vertex $z(C_{r'-1})$.

We have shown already that vertex $z(C_1)$ lies in graph $H$. Assume that for some $1<r'\leq r$, we have shown that vertex $z(C_{r'-1})$ lies in graph $H$. Then, from \Cref{obs: coverning chain importance}, 
supernode $u^{L_{r'}}(C_{r'-1})$ lies in graph $H^{L_{r'}}$, and  it is marked as an important supernode for cluster $C_{r'}$. From the definition of graph $H$, vertex $z(C_{r'})$ must lie in $H$, and it is connected with an edge of length $2^{i_{r'}}$ to vertex $v(C_{r'-1})$.

We have now obtained a path $P_1=(x,z(C_1),z(C_2),\ldots,z(C_{r}))$ in graph $H$, whose length is bounded by $2\cdot 2^{i_r}\leq D_i\cdot 2^{10L+10}$.


Similarly, from the definition of the set $R_i^L(y)$ of vertices, there is a covering chain: \newline $J'=((L'_1,i'_1,C'_1,x'_1),\ldots,(L'_{\hat r},i'_{\hat r},C'_{\hat r},x'_{\hat r}))\in \jset^L_i(y)$, such that $y'=x'_{\hat r}$. Using the same argument as before, there is a path $P_2=(y,z(C'_1),z(C'_2),\ldots,z(C'_{\hat r}))$ in graph $H$, whose length is bounded by $D_i\cdot 2^{10L+10}$. We delete the last vertex from this path, and we denote $C'=C'_{\hat r-1}$, so that the last vertex on path $P_2$ is now $z(C')$. Note that $\scale(C')=i+10(L_{\hat r-1}+10)\leq i+10L$. For convenience, we denote $C=C_r$, $i'=\scale(C_r)=i+10(L+10)$, and $i''=\scale(C')\leq i+10L$.
Recall that vertex $u^L(C')$ lies in graph $H^L$. We will use the following observation in order to complete the proof.

\begin{observation}\label{obs: another important supernode}
	At time $\tau$, supernode $u^L(C')$ is marked as an important supernode for cluster $C$.
\end{observation}

The proof of the observation is deferred to Section \ref{subsec: obs: another important supernode} of Appendix. It is now immediate to complete the proof of \Cref{claim: distances preserved in emulator} using it. Indeed, if, at time $\tau$, supernode $u^L(C')$ is marked as an important supernode for cluster $C$, then edge $e=(z(C'),z(C))$ of length $2^{\scale(C)}=2^{i+10L+10}$ belongs to graph $H$. By concatenating path $P_1$, edge $e$, and path $P_2$ (in reverse), we obtain the desired path $P$ in graph $H$, that connects $x$ to $y$. The length of the path is bounded by $3\cdot 2^{i+10L+10}\leq D_i\cdot 2^{O(1/\eps)}\leq D\cdot \alpha^{O(1/\eps)}$, since $\alpha=\alpha(W)\geq 2$.
\end{proof}





Next, we provide an algorithm to respond to $\transformpath$ queries in the following claim.

\begin{claim}\label{claim: alg to transform paths}
	There is a deterministic algorithm that supports $\transformpath$ queries in graph $H$:  given a path $P$ of length $D$ in graph $H$, that connects a pair $t,t'\in T$ of terminals, the algorithm computes a path  $P'$ in graph $G$, connecting $t$ to $t'$, whose length is at most $D\cdot \alpha^{O(1/\eps)}$. The query time must be bounded by $O(|E(P)|+|E(P')|)$, where $P$ is the path that the algorithm is given as input, and $P'$ is the path that the algorithm returns.
\end{claim}
\begin{proof}
	Consider first an edge $e=(z(C),z(C'))$ in graph $H$, connecting a pair of non-terminal vertices. Assume that $C\in A_L,C'\in A_{L'}$, and assume w.l.o.g. that $L<L'$ holds. Then supernode $u^{L'}(C)$ currently lies in graph $H^{L'}$, and it is marked as an important supernode for cluster $C'$. From Rule \ref{rule for importance}, $\scale(C)\leq \scale(C')$ must hold, and, from definition of graph $H$, the length of $e$ in $H$ is $\ell_H(e)=2^{\scale(C')}$. In particular, $\ell_H(e)\leq \max\set{2^{\scale(C)},2^{\scale(C')}}$. Using data structure $\DS$, we can also compute, in time $O(1)$, a vertex $a\in V(G)$ with $a\in V^F(C)\cap V^F(C')$. Indeed, since $u^{L'}(C)$ is a supernode in graph $H^{L'}$, and it is marked as important for cluster $C'$, it may not be an isolated vertex in $H^{L'}$. Let $v^L(a)$ be any neighbor vertex of $u^{L'}(C)$. Then $a\in V^F(C)$ must hold from the definition of graph $H^L$, and, since supernode $u^L(C)$ is important for cluster $C'$, $a\in V^F(C')$ must also hold.
	
	Consider now the given path $P$ of length $D$ in graph $H$, that connects a pair $t,t'\in T$ of terminals. We can assume w.l.o.g. that the path does not contain any terminals as inner vertices, since otherwise we can decompose the path into a sequence of subpaths, each of which has two terminals as its endpoints, and contains no terminals as inner vertices. By applying the claim to each of the subpaths and then concatenating the resulting paths, we  obtain the desired path connecting $t$ to $t'$ in $G$. From now on we assume that path $P$ contains no terminals as inner vertices, and we denote $P=(t,z(C_1),z(C_2),\ldots,z(C_r),t')$. From the above discussion, the length of path $P$ in $H$ is at least $\sum_{j=1}^r2^{\scale(C_j)}$.
	
	From the definition of graph $H$ and the flattened sets of vertices, $t\in V^F(C_1)$ and $t'\in V^F(C_r)$ must hold. For all $1\leq j< r$, we use the algorithm that we described above to compute, in time $O(1)$, a vertex $a_j\in V(G)$, such that $a_j\in V^F(C_j)$ and $a_j\in V^F(C_{j+1})$ holds. For convenience, we also denote $a_0=t$ and $a_r=t'$.
	
	Next, we consider clusters $C_1,\ldots,C_r$ one by one. Let $C_j$ be any such cluster. We have now defined a pair $a_{j-1},a_j$ of vertices of $G$, both of which lie in $V^F(C_j)$. We use the algorithm from \Cref{claim: short paths flat sets}, in order to compute a path $Q_j$ in graph $G$, connecting $a_{j-1}$ to $a_j$, whose length is at most  $(\tilde c\alpha)^{q+1}\cdot 2^{\scale(C_j)}$ (if $a_{j-1}=a_j$, then we let path $Q_j$ consist of a single vertex -- vertex $a_j$). The time required to compute the path is at most $O(|E(Q_j)|+1)$.
	Lastly, we obtain a path $P'$ in graph $G$, by concatenating the paths  $Q_1,\ldots,Q_r$. The resulting path connects $t$ to $t'$, and its length is bounded by:
	
	\[\sum_{j=1}^r  (\tilde c\alpha)^{q+1}\cdot 2^{\scale(C_j)}\leq \alpha^{O(1/\eps)}\cdot \sum_{j=1}^r2^{\scale(C_j)}\leq D\cdot \alpha^{O(1/\eps)}\].
	
It is easy to verify that the running time of the algorithm is bounded by $O|E(P')|+|E(P)|)$.
\end{proof}

We now complete the proof that $H$ is a valid $D^*$-restricted $T$-emulator with stretch $\alpha^{O(1/\eps)}$.
Clearly, from the definition of graph $H$, $T\subseteq V(H)$ always holds. From  \Cref{claim: distances preserved in emulator}
at all times $\tau\in \tset$,  for every pair $x,y\in T$ of terminals, if $\dist_{G\attime}(x,y)\leq D^*$, then  $ \dist_{H\attime}(x,y)\leq \alpha'\cdot \dist_{G\attime}(x,y)$ holds. 


It now remains to show that, for a large enough consant $c$,  at all times $\tau\in \tset$, for every pair $x,y\in T$ of terminals, if $\dist_{G\attime}(x,y)\leq D^*$, then  $\dist_{H\attime}(x,y)>\frac{\dist_{G\attime}(x,y)}{\alpha^c}$ holds. Assume for contradiction that this is not the case, so at some time $\tau \in \tset$, there is a pair $x,y\in T$ of terminals, for which  $\dist_{H\attime}(x,y)\leq \frac{\dist_{G\attime}(x,y)}{\alpha^c}$ holds. Let $P$ be a path connecting $x$ to $y$ in $H\attime$, whose length is at most $D=\frac{\dist_{G\attime}(x,y)}{\alpha^c}$.
But then, from 
\Cref{claim: alg to transform paths}, ther eis a path $P'$ in graph $G$, connecting $x$ to $y$, whose length is at most $D\cdot \alpha^{O(1/\eps)}$. By letting $c$ be a large enough constant, we conclude that the length of $P'$ is less than $\dist_{G\attime}(x,y)$, which is impossible.

==> arxiv-version-final/temp.tex <==

\begin{theorem}\label{thm: maintain cluster algorithm2}
	There is a deterministic algorithm for the \maintaincluster problem, that,  on input $\iset=\left(C,\set{\ell(e)}_{e\in E(C)},D \right )$, that undergoes a sequence $\Sigma$ of valid update operations with dynamic degree bound $\mu\geq (N^0(C))^{1/10}$, where $N^0(C)$ is the number of regular vertices in $C$ at the beginning of the algorithm, achieves approximation factor $1$, and  has total update time: $O(N\cdot \mu^{22}\cdot D^*)$.
\end{theorem}




\begin{theorem}\label{recdynnc simple}
	There is a deterministic algorithm for the \recdynnc problem, that,  on input $\iset=\left(H,\set{\ell(e)}_{e\in E(H)},D \right )$, that undergoes a sequence $\Sigma$ of valid update operations with dynamic degree bound $\mu$, such that $\mu\geq N^{1/10}$ holds, where $N$ is the number of regular vertices in $H$ at the beginning of the algorithm, and a precision parameter $\frac{1}{(\log N)^{1/24}}\leq \eps\leq 1/400$, such that $1/\eps$ is an integer, achieves approximation factor
	$\alpha^*=2^{O(1/\eps^6)}\cdot \log\log N$.
	The algorithm ensures that, for every regular vertex $v$ of $H$, the total number of clusters to which $v$ ever belongs over the course of the algorithm is bounded by $N^{4\eps}$.
	The algorithm has total update time: $ O\left( N^{1+8\eps}\cdot \mu^{22}\cdot D^* \right )$.
\end{theorem}	


\begin{lemma}\label{lemma: inductive}
	Let $N>0$, and $1/(\log N)^{1/50}\leq \eps<1/400$ be parameters, such that $1/\eps$ is an integer, and let $q=\ceil{1/\eps}$. For all $3\leq i\leq q$, there is a deterministic algorithm for the \recdynnc problem, that, given a valid input structure $\iset=\left(H,\set{\ell(e)}_{e\in E},D \right )$ undergoing a sequence of valid update operations with dynamic degree bound $\mu$, such that, if we denote by $N^0(H)$ the number of regular vertices in $H$ at the beginning of the algorithm, then $N^0(H)\leq N^{i\eps}$, achieves approximation factor $\alpha_i=(\log\log (N\mu))^{\tilde c\cdot 2^{2i}/\eps^{18}}$, and has total update time:
	
	
	\[\begin{split}
	N^0(H)\cdot \hat W^{\tilde c\eps+\tilde ci\eps^2}\cdot \mu^{\tilde c i} \cdot D^{3},
	\end{split}
	\]
	
	where $\tilde c$ is a fixed large enough constant.
	The algorithm also ensures that, for every regular vertex $v$ of $H$, there are at most $\Delta_i$ clusters that ever contain $v$ over the course of the algorithm, where $\Delta_3=\hat W^{3\eps}$, and, for all $i>3$, $\Delta_i=\hat W^{4\eps^4}$.
\end{lemma}

